Study of the doubly charmed tetraquark $T_{cc}^+$

An exotic narrow state in the $D^0D^0\pi^+$ mass spectrum just below the $D^{*+}D^0$ mass threshold is studied using a data set corresponding to an integrated luminosity of 9 fb$^{-1}$ acquired with the LHCb detector in proton-proton collisions at centre-of-mass energies of 7, 8 and 13 TeV. The state is consistent with the ground isoscalar $T^+_{cc}$ tetraquark with a quark content of $cc\bar{u}\bar{d}$ and spin-parity quantum numbers $\mathrm{J}^{\mathrm{P}}=1^+$. Study of the $DD$ mass spectra disfavours interpretation of the resonance as the isovector state. The decay structure via intermediate off-shell $D^{*+}$ mesons is confirmed by the $D^0\pi^+$ mass distribution. The mass of the resonance and its coupling to the $D^{*}D$ system are analysed. Resonance parameters including the pole position, scattering length, effective range and compositeness are measured to reveal important information about the nature of the $T^+_{cc}$ state. In addition, an unexpected dependence of the production rate on track multiplicity is observed.

==> Authorship_LHCb-PAPER-2021-031.tex <==
% LHCb collaboration author list
% Data extracted on July 8th, 2021 at 8:38pm for paper reference LHCb-PAPER-2021-031
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{32}$,
A.S.W.~Abdelmotteleb$^{56}$,
C.~Abell{\'a}n~Beteta$^{50}$,
F.J.~Abudinen~Gallego$^{56}$,
T.~Ackernley$^{60}$,
B.~Adeva$^{46}$,
M.~Adinolfi$^{54}$,
H.~Afsharnia$^{9}$,
C.~Agapopoulou$^{13}$,
C.A.~Aidala$^{87}$,
S.~Aiola$^{25}$,
Z.~Ajaltouni$^{9}$,
S.~Akar$^{65}$,
J.~Albrecht$^{15}$,
F.~Alessio$^{48}$,
M.~Alexander$^{59}$,
A.~Alfonso~Albero$^{45}$,
Z.~Aliouche$^{62}$,
G.~Alkhazov$^{38}$,
P.~Alvarez~Cartelle$^{55}$,
S.~Amato$^{2}$,
J.L.~Amey$^{54}$,
Y.~Amhis$^{11}$,
L.~An$^{48}$,
L.~Anderlini$^{22}$,
A.~Andreianov$^{38}$,
M.~Andreotti$^{21}$,
F.~Archilli$^{17}$,
A.~Artamonov$^{44}$,
M.~Artuso$^{68}$,
K.~Arzymatov$^{42}$,
E.~Aslanides$^{10}$,
M.~Atzeni$^{50}$,
B.~Audurier$^{12}$,
S.~Bachmann$^{17}$,
M.~Bachmayer$^{49}$,
J.J.~Back$^{56}$,
P.~Baladron~Rodriguez$^{46}$,
V.~Balagura$^{12}$,
W.~Baldini$^{21}$,
J.~Baptista~Leite$^{1}$,
M.~Barbetti$^{22,g}$,
R.J.~Barlow$^{62}$,
S.~Barsuk$^{11}$,
W.~Barter$^{61}$,
M.~Bartolini$^{24,h}$,
F.~Baryshnikov$^{83}$,
J.M.~Basels$^{14}$,
S.~Bashir$^{34}$,
G.~Bassi$^{29}$,
B.~Batsukh$^{68}$,
A.~Battig$^{15}$,
A.~Bay$^{49}$,
A.~Beck$^{56}$,
M.~Becker$^{15}$,
F.~Bedeschi$^{29}$,
I.~Bediaga$^{1}$,
A.~Beiter$^{68}$,
V.~Belavin$^{42}$,
S.~Belin$^{27}$,
V.~Bellee$^{50}$,
K.~Belous$^{44}$,
I.~Belov$^{40}$,
I.~Belyaev$^{41}$,
G.~Bencivenni$^{23}$,
E.~Ben-Haim$^{13}$,
A.~Berezhnoy$^{40}$,
R.~Bernet$^{50}$,
D.~Berninghoff$^{17}$,
H.C.~Bernstein$^{68}$,
C.~Bertella$^{48}$,
A.~Bertolin$^{28}$,
C.~Betancourt$^{50}$,
F.~Betti$^{48}$,
Ia.~Bezshyiko$^{50}$,
S.~Bhasin$^{54}$,
J.~Bhom$^{35}$,
L.~Bian$^{73}$,
M.S.~Bieker$^{15}$,
S.~Bifani$^{53}$,
P.~Billoir$^{13}$,
M.~Birch$^{61}$,
F.C.R.~Bishop$^{55}$,
A.~Bitadze$^{62}$,
A.~Bizzeti$^{22,k}$,
M.~Bj{\o}rn$^{63}$,
M.P.~Blago$^{48}$,
T.~Blake$^{56}$,
F.~Blanc$^{49}$,
S.~Blusk$^{68}$,
D.~Bobulska$^{59}$,
J.A.~Boelhauve$^{15}$,
O.~Boente~Garcia$^{46}$,
T.~Boettcher$^{65}$,
A.~Boldyrev$^{82}$,
A.~Bondar$^{43}$,
N.~Bondar$^{38,48}$,
S.~Borghi$^{62}$,
M.~Borisyak$^{42}$,
M.~Borsato$^{17}$,
J.T.~Borsuk$^{35}$,
S.A.~Bouchiba$^{49}$,
T.J.V.~Bowcock$^{60}$,
A.~Boyer$^{48}$,
C.~Bozzi$^{21}$,
M.J.~Bradley$^{61}$,
S.~Braun$^{66}$,
A.~Brea~Rodriguez$^{46}$,
J.~Brodzicka$^{35}$,
A.~Brossa~Gonzalo$^{56}$,
D.~Brundu$^{27}$,
A.~Buonaura$^{50}$,
L.~Buonincontri$^{28}$,
A.T.~Burke$^{62}$,
C.~Burr$^{48}$,
A.~Bursche$^{72}$,
A.~Butkevich$^{39}$,
J.S.~Butter$^{32}$,
J.~Buytaert$^{48}$,
W.~Byczynski$^{48}$,
S.~Cadeddu$^{27}$,
H.~Cai$^{73}$,
R.~Calabrese$^{21,f}$,
L.~Calefice$^{15,13}$,
L.~Calero~Diaz$^{23}$,
S.~Cali$^{23}$,
R.~Calladine$^{53}$,
M.~Calvi$^{26,j}$,
M.~Calvo~Gomez$^{85}$,
P.~Camargo~Magalhaes$^{54}$,
P.~Campana$^{23}$,
A.F.~Campoverde~Quezada$^{6}$,
S.~Capelli$^{26,j}$,
L.~Capriotti$^{20,d}$,
A.~Carbone$^{20,d}$,
G.~Carboni$^{31}$,
R.~Cardinale$^{24,h}$,
A.~Cardini$^{27}$,
I.~Carli$^{4}$,
P.~Carniti$^{26,j}$,
L.~Carus$^{14}$,
K.~Carvalho~Akiba$^{32}$,
A.~Casais~Vidal$^{46}$,
G.~Casse$^{60}$,
M.~Cattaneo$^{48}$,
G.~Cavallero$^{48}$,
S.~Celani$^{49}$,
J.~Cerasoli$^{10}$,
D.~Cervenkov$^{63}$,
A.J.~Chadwick$^{60}$,
M.G.~Chapman$^{54}$,
M.~Charles$^{13}$,
Ph.~Charpentier$^{48}$,
G.~Chatzikonstantinidis$^{53}$,
C.A.~Chavez~Barajas$^{60}$,
M.~Chefdeville$^{8}$,
C.~Chen$^{3}$,
S.~Chen$^{4}$,
A.~Chernov$^{35}$,
V.~Chobanova$^{46}$,
S.~Cholak$^{49}$,
M.~Chrzaszcz$^{35}$,
A.~Chubykin$^{38}$,
V.~Chulikov$^{38}$,
P.~Ciambrone$^{23}$,
M.F.~Cicala$^{56}$,
X.~Cid~Vidal$^{46}$,
G.~Ciezarek$^{48}$,
P.E.L.~Clarke$^{58}$,
M.~Clemencic$^{48}$,
H.V.~Cliff$^{55}$,
J.~Closier$^{48}$,
J.L.~Cobbledick$^{62}$,
V.~Coco$^{48}$,
J.A.B.~Coelho$^{11}$,
J.~Cogan$^{10}$,
E.~Cogneras$^{9}$,
L.~Cojocariu$^{37}$,
P.~Collins$^{48}$,
T.~Colombo$^{48}$,
L.~Congedo$^{19,c}$,
A.~Contu$^{27}$,
N.~Cooke$^{53}$,
G.~Coombs$^{59}$,
I.~Corredoira~$^{46}$,
G.~Corti$^{48}$,
C.M.~Costa~Sobral$^{56}$,
B.~Couturier$^{48}$,
D.C.~Craik$^{64}$,
J.~Crkovsk\'{a}$^{67}$,
M.~Cruz~Torres$^{1}$,
R.~Currie$^{58}$,
C.L.~Da~Silva$^{67}$,
S.~Dadabaev$^{83}$,
L.~Dai$^{71}$,
E.~Dall'Occo$^{15}$,
J.~Dalseno$^{46}$,
C.~D'Ambrosio$^{48}$,
A.~Danilina$^{41}$,
P.~d'Argent$^{48}$,
J.E.~Davies$^{62}$,
A.~Davis$^{62}$,
O.~De~Aguiar~Francisco$^{62}$,
K.~De~Bruyn$^{79}$,
S.~De~Capua$^{62}$,
M.~De~Cian$^{49}$,
J.M.~De~Miranda$^{1}$,
L.~De~Paula$^{2}$,
M.~De~Serio$^{19,c}$,
D.~De~Simone$^{50}$,
P.~De~Simone$^{23}$,
F.~De~Vellis$^{15}$,
J.A.~de~Vries$^{80}$,
C.T.~Dean$^{67}$,
F.~Debernardis$^{19,c}$,
D.~Decamp$^{8}$,
V.~Dedu$^{10}$,
L.~Del~Buono$^{13}$,
B.~Delaney$^{55}$,
H.-P.~Dembinski$^{15}$,
A.~Dendek$^{34}$,
V.~Denysenko$^{50}$,
D.~Derkach$^{82}$,
O.~Deschamps$^{9}$,
F.~Desse$^{11}$,
F.~Dettori$^{27,e}$,
B.~Dey$^{77}$,
A.~Di~Cicco$^{23}$,
P.~Di~Nezza$^{23}$,
S.~Didenko$^{83}$,
L.~Dieste~Maronas$^{46}$,
H.~Dijkstra$^{48}$,
V.~Dobishuk$^{52}$,
C.~Dong$^{3}$,
A.M.~Donohoe$^{18}$,
F.~Dordei$^{27}$,
A.C.~dos~Reis$^{1}$,
L.~Douglas$^{59}$,
A.~Dovbnya$^{51}$,
A.G.~Downes$^{8}$,
M.W.~Dudek$^{35}$,
L.~Dufour$^{48}$,
V.~Duk$^{78}$,
P.~Durante$^{48}$,
J.M.~Durham$^{67}$,
D.~Dutta$^{62}$,
A.~Dziurda$^{35}$,
A.~Dzyuba$^{38}$,
S.~Easo$^{57}$,
U.~Egede$^{69}$,
V.~Egorychev$^{41}$,
S.~Eidelman$^{43,u,\dagger}$,
S.~Eisenhardt$^{58}$,
S.~Ek-In$^{49}$,
L.~Eklund$^{59,86}$,
S.~Ely$^{68}$,
A.~Ene$^{37}$,
E.~Epple$^{67}$,
S.~Escher$^{14}$,
J.~Eschle$^{50}$,
S.~Esen$^{13}$,
T.~Evans$^{48}$,
A.~Falabella$^{20}$,
J.~Fan$^{3}$,
Y.~Fan$^{6}$,
B.~Fang$^{73}$,
S.~Farry$^{60}$,
D.~Fazzini$^{26,j}$,
M.~F{\'e}o$^{48}$,
A.~Fernandez~Prieto$^{46}$,
A.D.~Fernez$^{66}$,
F.~Ferrari$^{20,d}$,
L.~Ferreira~Lopes$^{49}$,
F.~Ferreira~Rodrigues$^{2}$,
S.~Ferreres~Sole$^{32}$,
M.~Ferrillo$^{50}$,
M.~Ferro-Luzzi$^{48}$,
S.~Filippov$^{39}$,
R.A.~Fini$^{19}$,
M.~Fiorini$^{21,f}$,
M.~Firlej$^{34}$,
K.M.~Fischer$^{63}$,
D.S.~Fitzgerald$^{87}$,
C.~Fitzpatrick$^{62}$,
T.~Fiutowski$^{34}$,
A.~Fkiaras$^{48}$,
F.~Fleuret$^{12}$,
M.~Fontana$^{13}$,
F.~Fontanelli$^{24,h}$,
R.~Forty$^{48}$,
D.~Foulds-Holt$^{55}$,
V.~Franco~Lima$^{60}$,
M.~Franco~Sevilla$^{66}$,
M.~Frank$^{48}$,
E.~Franzoso$^{21}$,
G.~Frau$^{17}$,
C.~Frei$^{48}$,
D.A.~Friday$^{59}$,
J.~Fu$^{6}$,
Q.~Fuehring$^{15}$,
E.~Gabriel$^{32}$,
G.~Galati$^{19,c}$,
A.~Gallas~Torreira$^{46}$,
D.~Galli$^{20,d}$,
S.~Gambetta$^{58,48}$,
Y.~Gan$^{3}$,
M.~Gandelman$^{2}$,
P.~Gandini$^{25}$,
Y.~Gao$^{5}$,
M.~Garau$^{27}$,
L.M.~Garcia~Martin$^{56}$,
P.~Garcia~Moreno$^{45}$,
J.~Garc{\'\i}a~Pardi{\~n}as$^{26,j}$,
B.~Garcia~Plana$^{46}$,
F.A.~Garcia~Rosales$^{12}$,
L.~Garrido$^{45}$,
C.~Gaspar$^{48}$,
R.E.~Geertsema$^{32}$,
D.~Gerick$^{17}$,
L.L.~Gerken$^{15}$,
E.~Gersabeck$^{62}$,
M.~Gersabeck$^{62}$,
T.~Gershon$^{56}$,
D.~Gerstel$^{10}$,
L.~Giambastiani$^{28}$,
V.~Gibson$^{55}$,
H.K.~Giemza$^{36}$,
A.L.~Gilman$^{63}$,
M.~Giovannetti$^{23,p}$,
A.~Giovent{\`u}$^{46}$,
P.~Gironella~Gironell$^{45}$,
L.~Giubega$^{37}$,
C.~Giugliano$^{21,f,48}$,
K.~Gizdov$^{58}$,
E.L.~Gkougkousis$^{48}$,
V.V.~Gligorov$^{13}$,
C.~G{\"o}bel$^{70}$,
E.~Golobardes$^{85}$,
D.~Golubkov$^{41}$,
A.~Golutvin$^{61,83}$,
A.~Gomes$^{1,a}$,
S.~Gomez~Fernandez$^{45}$,
F.~Goncalves~Abrantes$^{63}$,
M.~Goncerz$^{35}$,
G.~Gong$^{3}$,
P.~Gorbounov$^{41}$,
I.V.~Gorelov$^{40}$,
C.~Gotti$^{26}$,
E.~Govorkova$^{48}$,
J.P.~Grabowski$^{17}$,
T.~Grammatico$^{13}$,
L.A.~Granado~Cardoso$^{48}$,
E.~Graug{\'e}s$^{45}$,
E.~Graverini$^{49}$,
G.~Graziani$^{22}$,
A.~Grecu$^{37}$,
L.M.~Greeven$^{32}$,
N.A.~Grieser$^{4}$,
L.~Grillo$^{62}$,
S.~Gromov$^{83}$,
B.R.~Gruberg~Cazon$^{63}$,
C.~Gu$^{3}$,
M.~Guarise$^{21}$,
M.~Guittiere$^{11}$,
P. A.~G{\"u}nther$^{17}$,
E.~Gushchin$^{39}$,
A.~Guth$^{14}$,
Y.~Guz$^{44}$,
T.~Gys$^{48}$,
T.~Hadavizadeh$^{69}$,
G.~Haefeli$^{49}$,
C.~Haen$^{48}$,
J.~Haimberger$^{48}$,
T.~Halewood-leagas$^{60}$,
P.M.~Hamilton$^{66}$,
J.P.~Hammerich$^{60}$,
Q.~Han$^{7}$,
X.~Han$^{17}$,
T.H.~Hancock$^{63}$,
E.B.~Hansen$^{62}$,
S.~Hansmann-Menzemer$^{17}$,
N.~Harnew$^{63}$,
T.~Harrison$^{60}$,
C.~Hasse$^{48}$,
M.~Hatch$^{48}$,
J.~He$^{6,b}$,
M.~Hecker$^{61}$,
K.~Heijhoff$^{32}$,
K.~Heinicke$^{15}$,
A.M.~Hennequin$^{48}$,
K.~Hennessy$^{60}$,
L.~Henry$^{48}$,
J.~Heuel$^{14}$,
A.~Hicheur$^{2}$,
D.~Hill$^{49}$,
M.~Hilton$^{62}$,
S.E.~Hollitt$^{15}$,
R.~Hou$^{7}$,
Y.~Hou$^{8}$,
J.~Hu$^{17}$,
J.~Hu$^{72}$,
W.~Hu$^{7}$,
X.~Hu$^{3}$,
W.~Huang$^{6}$,
X.~Huang$^{73}$,
W.~Hulsbergen$^{32}$,
R.J.~Hunter$^{56}$,
M.~Hushchyn$^{82}$,
D.~Hutchcroft$^{60}$,
D.~Hynds$^{32}$,
P.~Ibis$^{15}$,
M.~Idzik$^{34}$,
D.~Ilin$^{38}$,
P.~Ilten$^{65}$,
A.~Inglessi$^{38}$,
A.~Ishteev$^{83}$,
K.~Ivshin$^{38}$,
R.~Jacobsson$^{48}$,
H.~Jage$^{14}$,
S.~Jakobsen$^{48}$,
E.~Jans$^{32}$,
B.K.~Jashal$^{47}$,
A.~Jawahery$^{66}$,
V.~Jevtic$^{15}$,
F.~Jiang$^{3}$,
M.~John$^{63}$,
D.~Johnson$^{48}$,
C.R.~Jones$^{55}$,
T.P.~Jones$^{56}$,
B.~Jost$^{48}$,
N.~Jurik$^{48}$,
S.H.~Kalavan~Kadavath$^{34}$,
S.~Kandybei$^{51}$,
Y.~Kang$^{3}$,
M.~Karacson$^{48}$,
M.~Karpov$^{82}$,
F.~Keizer$^{48}$,
D.M.~Keller$^{68}$,
M.~Kenzie$^{56}$,
T.~Ketel$^{33}$,
B.~Khanji$^{15}$,
A.~Kharisova$^{84}$,
S.~Kholodenko$^{44}$,
T.~Kirn$^{14}$,
V.S.~Kirsebom$^{49}$,
O.~Kitouni$^{64}$,
S.~Klaver$^{32}$,
N.~Kleijne$^{29}$,
K.~Klimaszewski$^{36}$,
M.R.~Kmiec$^{36}$,
S.~Koliiev$^{52}$,
A.~Kondybayeva$^{83}$,
A.~Konoplyannikov$^{41}$,
P.~Kopciewicz$^{34}$,
R.~Kopecna$^{17}$,
P.~Koppenburg$^{32}$,
M.~Korolev$^{40}$,
I.~Kostiuk$^{32,52}$,
O.~Kot$^{52}$,
S.~Kotriakhova$^{21,38}$,
P.~Kravchenko$^{38}$,
L.~Kravchuk$^{39}$,
R.D.~Krawczyk$^{48}$,
M.~Kreps$^{56}$,
F.~Kress$^{61}$,
S.~Kretzschmar$^{14}$,
P.~Krokovny$^{43,u}$,
W.~Krupa$^{34}$,
W.~Krzemien$^{36}$,
M.~Kucharczyk$^{35}$,
V.~Kudryavtsev$^{43,u}$,
H.S.~Kuindersma$^{32,33}$,
G.J.~Kunde$^{67}$,
T.~Kvaratskheliya$^{41}$,
D.~Lacarrere$^{48}$,
G.~Lafferty$^{62}$,
A.~Lai$^{27}$,
A.~Lampis$^{27}$,
D.~Lancierini$^{50}$,
J.J.~Lane$^{62}$,
R.~Lane$^{54}$,
G.~Lanfranchi$^{23}$,
C.~Langenbruch$^{14}$,
J.~Langer$^{15}$,
O.~Lantwin$^{83}$,
T.~Latham$^{56}$,
F.~Lazzari$^{29,q}$,
R.~Le~Gac$^{10}$,
S.H.~Lee$^{87}$,
R.~Lef{\`e}vre$^{9}$,
A.~Leflat$^{40}$,
S.~Legotin$^{83}$,
O.~Leroy$^{10}$,
T.~Lesiak$^{35}$,
B.~Leverington$^{17}$,
H.~Li$^{72}$,
P.~Li$^{17}$,
S.~Li$^{7}$,
Y.~Li$^{4}$,
Y.~Li$^{4}$,
Z.~Li$^{68}$,
X.~Liang$^{68}$,
T.~Lin$^{61}$,
R.~Lindner$^{48}$,
V.~Lisovskyi$^{15}$,
R.~Litvinov$^{27}$,
G.~Liu$^{72}$,
H.~Liu$^{6}$,
Q.~Liu$^{6}$,
S.~Liu$^{4}$,
A.~Lobo~Salvia$^{45}$,
A.~Loi$^{27}$,
J.~Lomba~Castro$^{46}$,
I.~Longstaff$^{59}$,
J.H.~Lopes$^{2}$,
S.~Lopez~Solino$^{46}$,
G.H.~Lovell$^{55}$,
Y.~Lu$^{4}$,
C.~Lucarelli$^{22,g}$,
D.~Lucchesi$^{28,l}$,
S.~Luchuk$^{39}$,
M.~Lucio~Martinez$^{32}$,
V.~Lukashenko$^{32,52}$,
Y.~Luo$^{3}$,
A.~Lupato$^{62}$,
E.~Luppi$^{21,f}$,
O.~Lupton$^{56}$,
A.~Lusiani$^{29,m}$,
X.~Lyu$^{6}$,
L.~Ma$^{4}$,
R.~Ma$^{6}$,
S.~Maccolini$^{20,d}$,
F.~Machefert$^{11}$,
F.~Maciuc$^{37}$,
V.~Macko$^{49}$,
P.~Mackowiak$^{15}$,
S.~Maddrell-Mander$^{54}$,
O.~Madejczyk$^{34}$,
L.R.~Madhan~Mohan$^{54}$,
O.~Maev$^{38}$,
A.~Maevskiy$^{82}$,
D.~Maisuzenko$^{38}$,
M.W.~Majewski$^{34}$,
J.J.~Malczewski$^{35}$,
S.~Malde$^{63}$,
B.~Malecki$^{48}$,
A.~Malinin$^{81}$,
T.~Maltsev$^{43,u}$,
H.~Malygina$^{17}$,
G.~Manca$^{27,e}$,
G.~Mancinelli$^{10}$,
D.~Manuzzi$^{20,d}$,
D.~Marangotto$^{25,i}$,
J.~Maratas$^{9,s}$,
J.F.~Marchand$^{8}$,
U.~Marconi$^{20}$,
S.~Mariani$^{22,g}$,
C.~Marin~Benito$^{48}$,
M.~Marinangeli$^{49}$,
J.~Marks$^{17}$,
A.M.~Marshall$^{54}$,
P.J.~Marshall$^{60}$,
G.~Martelli$^{78}$,
G.~Martellotti$^{30}$,
L.~Martinazzoli$^{48,j}$,
M.~Martinelli$^{26,j}$,
D.~Martinez~Santos$^{46}$,
F.~Martinez~Vidal$^{47}$,
A.~Massafferri$^{1}$,
M.~Materok$^{14}$,
R.~Matev$^{48}$,
A.~Mathad$^{50}$,
V.~Matiunin$^{41}$,
C.~Matteuzzi$^{26}$,
K.R.~Mattioli$^{87}$,
A.~Mauri$^{32}$,
E.~Maurice$^{12}$,
J.~Mauricio$^{45}$,
M.~Mazurek$^{48}$,
M.~McCann$^{61}$,
L.~Mcconnell$^{18}$,
T.H.~Mcgrath$^{62}$,
N.T.~Mchugh$^{59}$,
A.~McNab$^{62}$,
R.~McNulty$^{18}$,
J.V.~Mead$^{60}$,
B.~Meadows$^{65}$,
G.~Meier$^{15}$,
N.~Meinert$^{76}$,
D.~Melnychuk$^{36}$,
S.~Meloni$^{26,j}$,
M.~Merk$^{32,80}$,
A.~Merli$^{25}$,
L.~Meyer~Garcia$^{2}$,
M.~Mikhasenko$^{48}$,
D.A.~Milanes$^{74}$,
E.~Millard$^{56}$,
M.~Milovanovic$^{48}$,
M.-N.~Minard$^{8}$,
A.~Minotti$^{26,j}$,
L.~Minzoni$^{21,f}$,
S.E.~Mitchell$^{58}$,
B.~Mitreska$^{62}$,
D.S.~Mitzel$^{15}$,
A.~M{\"o}dden~$^{15}$,
R.A.~Mohammed$^{63}$,
R.D.~Moise$^{61}$,
S.~Mokhnenko$^{82}$,
T.~Momb{\"a}cher$^{46}$,
I.A.~Monroy$^{74}$,
S.~Monteil$^{9}$,
M.~Morandin$^{28}$,
G.~Morello$^{23}$,
M.J.~Morello$^{29,m}$,
J.~Moron$^{34}$,
A.B.~Morris$^{75}$,
A.G.~Morris$^{56}$,
R.~Mountain$^{68}$,
H.~Mu$^{3}$,
F.~Muheim$^{58,48}$,
M.~Mulder$^{48}$,
D.~M{\"u}ller$^{48}$,
K.~M{\"u}ller$^{50}$,
C.H.~Murphy$^{63}$,
D.~Murray$^{62}$,
P.~Muzzetto$^{27,48}$,
P.~Naik$^{54}$,
T.~Nakada$^{49}$,
R.~Nandakumar$^{57}$,
T.~Nanut$^{49}$,
I.~Nasteva$^{2}$,
M.~Needham$^{58}$,
I.~Neri$^{21}$,
N.~Neri$^{25,i}$,
S.~Neubert$^{75}$,
N.~Neufeld$^{48}$,
R.~Newcombe$^{61}$,
E.M.~Niel$^{11}$,
S.~Nieswand$^{14}$,
N.~Nikitin$^{40}$,
N.S.~Nolte$^{64}$,
C.~Normand$^{8}$,
C.~Nunez$^{87}$,
A.~Oblakowska-Mucha$^{34}$,
V.~Obraztsov$^{44}$,
T.~Oeser$^{14}$,
D.P.~O'Hanlon$^{54}$,
S.~Okamura$^{21}$,
R.~Oldeman$^{27,e}$,
F.~Oliva$^{58}$,
M.E.~Olivares$^{68}$,
C.J.G.~Onderwater$^{79}$,
R.H.~O'neil$^{58}$,
J.M.~Otalora~Goicochea$^{2}$,
T.~Ovsiannikova$^{41}$,
P.~Owen$^{50}$,
A.~Oyanguren$^{47}$,
K.O.~Padeken$^{75}$,
B.~Pagare$^{56}$,
P.R.~Pais$^{48}$,
T.~Pajero$^{63}$,
A.~Palano$^{19}$,
M.~Palutan$^{23}$,
Y.~Pan$^{62}$,
G.~Panshin$^{84}$,
A.~Papanestis$^{57}$,
M.~Pappagallo$^{19,c}$,
L.L.~Pappalardo$^{21,f}$,
C.~Pappenheimer$^{65}$,
W.~Parker$^{66}$,
C.~Parkes$^{62}$,
B.~Passalacqua$^{21}$,
G.~Passaleva$^{22}$,
A.~Pastore$^{19}$,
M.~Patel$^{61}$,
C.~Patrignani$^{20,d}$,
C.J.~Pawley$^{80}$,
A.~Pearce$^{48}$,
A.~Pellegrino$^{32}$,
M.~Pepe~Altarelli$^{48}$,
S.~Perazzini$^{20}$,
D.~Pereima$^{41}$,
A.~Pereiro~Castro$^{46}$,
P.~Perret$^{9}$,
M.~Petric$^{59,48}$,
K.~Petridis$^{54}$,
A.~Petrolini$^{24,h}$,
A.~Petrov$^{81}$,
S.~Petrucci$^{58}$,
M.~Petruzzo$^{25}$,
T.T.H.~Pham$^{68}$,
L.~Pica$^{29,m}$,
M.~Piccini$^{78}$,
B.~Pietrzyk$^{8}$,
G.~Pietrzyk$^{49}$,
M.~Pili$^{63}$,
D.~Pinci$^{30}$,
F.~Pisani$^{48}$,
M.~Pizzichemi$^{26,48,j}$,
Resmi ~P.K$^{10}$,
V.~Placinta$^{37}$,
J.~Plews$^{53}$,
M.~Plo~Casasus$^{46}$,
F.~Polci$^{13}$,
M.~Poli~Lener$^{23}$,
M.~Poliakova$^{68}$,
A.~Poluektov$^{10}$,
N.~Polukhina$^{83,t}$,
I.~Polyakov$^{68}$,
E.~Polycarpo$^{2}$,
S.~Ponce$^{48}$,
D.~Popov$^{6,48}$,
S.~Popov$^{42}$,
S.~Poslavskii$^{44}$,
K.~Prasanth$^{35}$,
L.~Promberger$^{48}$,
C.~Prouve$^{46}$,
V.~Pugatch$^{52}$,
V.~Puill$^{11}$,
H.~Pullen$^{63}$,
G.~Punzi$^{29,n}$,
H.~Qi$^{3}$,
W.~Qian$^{6}$,
J.~Qin$^{6}$,
N.~Qin$^{3}$,
R.~Quagliani$^{49}$,
B.~Quintana$^{8}$,
N.V.~Raab$^{18}$,
R.I.~Rabadan~Trejo$^{6}$,
B.~Rachwal$^{34}$,
J.H.~Rademacker$^{54}$,
M.~Rama$^{29}$,
M.~Ramos~Pernas$^{56}$,
M.S.~Rangel$^{2}$,
F.~Ratnikov$^{42,82}$,
G.~Raven$^{33}$,
M.~Reboud$^{8}$,
F.~Redi$^{49}$,
F.~Reiss$^{62}$,
C.~Remon~Alepuz$^{47}$,
Z.~Ren$^{3}$,
V.~Renaudin$^{63}$,
R.~Ribatti$^{29}$,
S.~Ricciardi$^{57}$,
K.~Rinnert$^{60}$,
P.~Robbe$^{11}$,
G.~Robertson$^{58}$,
A.B.~Rodrigues$^{49}$,
E.~Rodrigues$^{60}$,
J.A.~Rodriguez~Lopez$^{74}$,
E.R.R.~Rodriguez~Rodriguez$^{46}$,
A.~Rollings$^{63}$,
P.~Roloff$^{48}$,
V.~Romanovskiy$^{44}$,
M.~Romero~Lamas$^{46}$,
A.~Romero~Vidal$^{46}$,
J.D.~Roth$^{87}$,
M.~Rotondo$^{23}$,
M.S.~Rudolph$^{68}$,
T.~Ruf$^{48}$,
R.A.~Ruiz~Fernandez$^{46}$,
J.~Ruiz~Vidal$^{47}$,
A.~Ryzhikov$^{82}$,
J.~Ryzka$^{34}$,
J.J.~Saborido~Silva$^{46}$,
N.~Sagidova$^{38}$,
N.~Sahoo$^{56}$,
B.~Saitta$^{27,e}$,
M.~Salomoni$^{48}$,
C.~Sanchez~Gras$^{32}$,
R.~Santacesaria$^{30}$,
C.~Santamarina~Rios$^{46}$,
M.~Santimaria$^{23}$,
E.~Santovetti$^{31,p}$,
D.~Saranin$^{83}$,
G.~Sarpis$^{14}$,
M.~Sarpis$^{75}$,
A.~Sarti$^{30}$,
C.~Satriano$^{30,o}$,
A.~Satta$^{31}$,
M.~Saur$^{15}$,
D.~Savrina$^{41,40}$,
H.~Sazak$^{9}$,
L.G.~Scantlebury~Smead$^{63}$,
A.~Scarabotto$^{13}$,
S.~Schael$^{14}$,
S.~Scherl$^{60}$,
M.~Schiller$^{59}$,
H.~Schindler$^{48}$,
M.~Schmelling$^{16}$,
B.~Schmidt$^{48}$,
S.~Schmitt$^{14}$,
O.~Schneider$^{49}$,
A.~Schopper$^{48}$,
M.~Schubiger$^{32}$,
S.~Schulte$^{49}$,
M.H.~Schune$^{11}$,
R.~Schwemmer$^{48}$,
B.~Sciascia$^{23,48}$,
S.~Sellam$^{46}$,
A.~Semennikov$^{41}$,
M.~Senghi~Soares$^{33}$,
A.~Sergi$^{24,h}$,
N.~Serra$^{50}$,
L.~Sestini$^{28}$,
A.~Seuthe$^{15}$,
Y.~Shang$^{5}$,
D.M.~Shangase$^{87}$,
M.~Shapkin$^{44}$,
I.~Shchemerov$^{83}$,
L.~Shchutska$^{49}$,
T.~Shears$^{60}$,
L.~Shekhtman$^{43,u}$,
Z.~Shen$^{5}$,
V.~Shevchenko$^{81}$,
E.B.~Shields$^{26,j}$,
Y.~Shimizu$^{11}$,
E.~Shmanin$^{83}$,
J.D.~Shupperd$^{68}$,
B.G.~Siddi$^{21}$,
R.~Silva~Coutinho$^{50}$,
G.~Simi$^{28}$,
S.~Simone$^{19,c}$,
N.~Skidmore$^{62}$,
T.~Skwarnicki$^{68}$,
M.W.~Slater$^{53}$,
I.~Slazyk$^{21,f}$,
J.C.~Smallwood$^{63}$,
J.G.~Smeaton$^{55}$,
A.~Smetkina$^{41}$,
E.~Smith$^{50}$,
M.~Smith$^{61}$,
A.~Snoch$^{32}$,
M.~Soares$^{20}$,
L.~Soares~Lavra$^{9}$,
M.D.~Sokoloff$^{65}$,
F.J.P.~Soler$^{59}$,
A.~Solovev$^{38}$,
I.~Solovyev$^{38}$,
F.L.~Souza~De~Almeida$^{2}$,
B.~Souza~De~Paula$^{2}$,
B.~Spaan$^{15}$,
E.~Spadaro~Norella$^{25}$,
P.~Spradlin$^{59}$,
F.~Stagni$^{48}$,
M.~Stahl$^{65}$,
S.~Stahl$^{48}$,
S.~Stanislaus$^{63}$,
O.~Steinkamp$^{50,83}$,
O.~Stenyakin$^{44}$,
H.~Stevens$^{15}$,
S.~Stone$^{68}$,
M.~Straticiuc$^{37}$,
D.~Strekalina$^{83}$,
F.~Suljik$^{63}$,
J.~Sun$^{27}$,
L.~Sun$^{73}$,
Y.~Sun$^{66}$,
P.~Svihra$^{62}$,
P.N.~Swallow$^{53}$,
K.~Swientek$^{34}$,
A.~Szabelski$^{36}$,
T.~Szumlak$^{34}$,
M.~Szymanski$^{48}$,
S.~Taneja$^{62}$,
A.R.~Tanner$^{54}$,
M.D.~Tat$^{63}$,
A.~Terentev$^{83}$,
F.~Teubert$^{48}$,
E.~Thomas$^{48}$,
D.J.D.~Thompson$^{53}$,
K.A.~Thomson$^{60}$,
V.~Tisserand$^{9}$,
S.~T'Jampens$^{8}$,
M.~Tobin$^{4}$,
L.~Tomassetti$^{21,f}$,
X.~Tong$^{5}$,
D.~Torres~Machado$^{1}$,
D.Y.~Tou$^{13}$,
E.~Trifonova$^{83}$,
C.~Trippl$^{49}$,
G.~Tuci$^{6}$,
A.~Tully$^{49}$,
N.~Tuning$^{32,48}$,
A.~Ukleja$^{36}$,
D.J.~Unverzagt$^{17}$,
E.~Ursov$^{83}$,
A.~Usachov$^{32}$,
A.~Ustyuzhanin$^{42,82}$,
U.~Uwer$^{17}$,
A.~Vagner$^{84}$,
V.~Vagnoni$^{20}$,
A.~Valassi$^{48}$,
G.~Valenti$^{20}$,
N.~Valls~Canudas$^{85}$,
M.~van~Beuzekom$^{32}$,
M.~Van~Dijk$^{49}$,
E.~van~Herwijnen$^{83}$,
C.B.~Van~Hulse$^{18}$,
M.~van~Veghel$^{79}$,
R.~Vazquez~Gomez$^{45}$,
P.~Vazquez~Regueiro$^{46}$,
C.~V{\'a}zquez~Sierra$^{48}$,
S.~Vecchi$^{21}$,
J.J.~Velthuis$^{54}$,
M.~Veltri$^{22,r}$,
A.~Venkateswaran$^{68}$,
M.~Veronesi$^{32}$,
M.~Vesterinen$^{56}$,
D.~~Vieira$^{65}$,
M.~Vieites~Diaz$^{49}$,
H.~Viemann$^{76}$,
X.~Vilasis-Cardona$^{85}$,
E.~Vilella~Figueras$^{60}$,
A.~Villa$^{20}$,
P.~Vincent$^{13}$,
F.C.~Volle$^{11}$,
D.~Vom~Bruch$^{10}$,
A.~Vorobyev$^{38}$,
V.~Vorobyev$^{43,u}$,
N.~Voropaev$^{38}$,
K.~Vos$^{80}$,
R.~Waldi$^{17}$,
J.~Walsh$^{29}$,
C.~Wang$^{17}$,
J.~Wang$^{5}$,
J.~Wang$^{4}$,
J.~Wang$^{3}$,
J.~Wang$^{73}$,
M.~Wang$^{3}$,
R.~Wang$^{54}$,
Y.~Wang$^{7}$,
Z.~Wang$^{50}$,
Z.~Wang$^{3}$,
Z.~Wang$^{6}$,
J.A.~Ward$^{56}$,
N.K.~Watson$^{53}$,
S.G.~Weber$^{13}$,
D.~Websdale$^{61}$,
C.~Weisser$^{64}$,
B.D.C.~Westhenry$^{54}$,
D.J.~White$^{62}$,
M.~Whitehead$^{54}$,
A.R.~Wiederhold$^{56}$,
D.~Wiedner$^{15}$,
G.~Wilkinson$^{63}$,
M.~Wilkinson$^{68}$,
I.~Williams$^{55}$,
M.~Williams$^{64}$,
M.R.J.~Williams$^{58}$,
F.F.~Wilson$^{57}$,
W.~Wislicki$^{36}$,
M.~Witek$^{35}$,
L.~Witola$^{17}$,
G.~Wormser$^{11}$,
S.A.~Wotton$^{55}$,
H.~Wu$^{68}$,
K.~Wyllie$^{48}$,
Z.~Xiang$^{6}$,
D.~Xiao$^{7}$,
Y.~Xie$^{7}$,
A.~Xu$^{5}$,
J.~Xu$^{6}$,
L.~Xu$^{3}$,
M.~Xu$^{7}$,
Q.~Xu$^{6}$,
Z.~Xu$^{5}$,
Z.~Xu$^{6}$,
D.~Yang$^{3}$,
S.~Yang$^{6}$,
Y.~Yang$^{6}$,
Z.~Yang$^{5}$,
Z.~Yang$^{66}$,
Y.~Yao$^{68}$,
L.E.~Yeomans$^{60}$,
H.~Yin$^{7}$,
J.~Yu$^{71}$,
X.~Yuan$^{68}$,
O.~Yushchenko$^{44}$,
E.~Zaffaroni$^{49}$,
M.~Zavertyaev$^{16,t}$,
M.~Zdybal$^{35}$,
O.~Zenaiev$^{48}$,
M.~Zeng$^{3}$,
D.~Zhang$^{7}$,
L.~Zhang$^{3}$,
S.~Zhang$^{71}$,
S.~Zhang$^{5}$,
Y.~Zhang$^{5}$,
Y.~Zhang$^{63}$,
A.~Zharkova$^{83}$,
A.~Zhelezov$^{17}$,
Y.~Zheng$^{6}$,
T.~Zhou$^{5}$,
X.~Zhou$^{6}$,
Y.~Zhou$^{6}$,
V.~Zhovkovska$^{11}$,
X.~Zhu$^{3}$,
X.~Zhu$^{7}$,
Z.~Zhu$^{6}$,
V.~Zhukov$^{14,40}$,
J.B.~Zonneveld$^{58}$,
Q.~Zou$^{4}$,
S.~Zucchelli$^{20,d}$,
D.~Zuliani$^{28}$,
G.~Zunica$^{62}$.\bigskip

{\footnotesize \it

$^{1}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$^{4}$Institute Of High Energy Physics (IHEP), Beijing, China\\
$^{5}$School of Physics State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China\\
$^{6}$University of Chinese Academy of Sciences, Beijing, China\\
$^{7}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China\\
$^{8}$Univ. Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$^{9}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$^{10}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$^{11}$Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\\
$^{12}$Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, Institut Polytechnique de Paris, Palaiseau, France\\
$^{13}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$^{14}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$^{15}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{16}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$^{17}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$^{18}$School of Physics, University College Dublin, Dublin, Ireland\\
$^{19}$INFN Sezione di Bari, Bari, Italy\\
$^{20}$INFN Sezione di Bologna, Bologna, Italy\\
$^{21}$INFN Sezione di Ferrara, Ferrara, Italy\\
$^{22}$INFN Sezione di Firenze, Firenze, Italy\\
$^{23}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{24}$INFN Sezione di Genova, Genova, Italy\\
$^{25}$INFN Sezione di Milano, Milano, Italy\\
$^{26}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$^{27}$INFN Sezione di Cagliari, Monserrato, Italy\\
$^{28}$Universita degli Studi di Padova, Universita e INFN, Padova, Padova, Italy\\
$^{29}$INFN Sezione di Pisa, Pisa, Italy\\
$^{30}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$^{31}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$^{32}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$^{33}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$^{34}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$^{35}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$^{36}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$^{37}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$^{38}$Petersburg Nuclear Physics Institute NRC Kurchatov Institute (PNPI NRC KI), Gatchina, Russia\\
$^{39}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), Moscow, Russia\\
$^{40}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia\\
$^{41}$Institute of Theoretical and Experimental Physics NRC Kurchatov Institute (ITEP NRC KI), Moscow, Russia\\
$^{42}$Yandex School of Data Analysis, Moscow, Russia\\
$^{43}$Budker Institute of Nuclear Physics (SB RAS), Novosibirsk, Russia\\
$^{44}$Institute for High Energy Physics NRC Kurchatov Institute (IHEP NRC KI), Protvino, Russia, Protvino, Russia\\
$^{45}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$^{46}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$^{47}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain\\
$^{48}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{49}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{50}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$^{51}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$^{52}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$^{53}$University of Birmingham, Birmingham, United Kingdom\\
$^{54}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$^{55}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{56}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{57}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{58}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{59}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{60}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{61}$Imperial College London, London, United Kingdom\\
$^{62}$Department of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{63}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$^{64}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$^{65}$University of Cincinnati, Cincinnati, OH, United States\\
$^{66}$University of Maryland, College Park, MD, United States\\
$^{67}$Los Alamos National Laboratory (LANL), Los Alamos, United States\\
$^{68}$Syracuse University, Syracuse, NY, United States\\
$^{69}$School of Physics and Astronomy, Monash University, Melbourne, Australia, associated to $^{56}$\\
$^{70}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$^{71}$Physics and Micro Electronic College, Hunan University, Changsha City, China, associated to $^{7}$\\
$^{72}$Guangdong Provincial Key Laboratory of Nuclear Science, Guangdong-Hong Kong Joint Laboratory of Quantum Matter, Institute of Quantum Matter, South China Normal University, Guangzhou, China, associated to $^{3}$\\
$^{73}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{3}$\\
$^{74}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{13}$\\
$^{75}$Universit{\"a}t Bonn - Helmholtz-Institut f{\"u}r Strahlen und Kernphysik, Bonn, Germany, associated to $^{17}$\\
$^{76}$Institut f{\"u}r Physik, Universit{\"a}t Rostock, Rostock, Germany, associated to $^{17}$\\
$^{77}$Eotvos Lorand University, Budapest, Hungary, associated to $^{48}$\\
$^{78}$INFN Sezione di Perugia, Perugia, Italy, associated to $^{21}$\\
$^{79}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{32}$\\
$^{80}$Universiteit Maastricht, Maastricht, Netherlands, associated to $^{32}$\\
$^{81}$National Research Centre Kurchatov Institute, Moscow, Russia, associated to $^{41}$\\
$^{82}$National Research University Higher School of Economics, Moscow, Russia, associated to $^{42}$\\
$^{83}$National University of Science and Technology ``MISIS'', Moscow, Russia, associated to $^{41}$\\
$^{84}$National Research Tomsk Polytechnic University, Tomsk, Russia, associated to $^{41}$\\
$^{85}$DS4DS, La Salle, Universitat Ramon Llull, Barcelona, Spain, associated to $^{45}$\\
$^{86}$Department of Physics and Astronomy, Uppsala University, Uppsala, Sweden, associated to $^{59}$\\
$^{87}$University of Michigan, Ann Arbor, United States, associated to $^{68}$\\
\bigskip
$^{a}$Universidade Federal do Tri{\^a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$^{b}$Hangzhou Institute for Advanced Study, UCAS, Hangzhou, China\\
$^{c}$Universit{\`a} di Bari, Bari, Italy\\
$^{d}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{e}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{f}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{g}$Universit{\`a} di Firenze, Firenze, Italy\\
$^{h}$Universit{\`a} di Genova, Genova, Italy\\
$^{i}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{j}$Universit{\`a} di Milano Bicocca, Milano, Italy\\
$^{k}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$^{l}$Universit{\`a} di Padova, Padova, Italy\\
$^{m}$Scuola Normale Superiore, Pisa, Italy\\
$^{n}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{o}$Universit{\`a} della Basilicata, Potenza, Italy\\
$^{p}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{q}$Universit{\`a} di Siena, Siena, Italy\\
$^{r}$Universit{\`a} di Urbino, Urbino, Italy\\
$^{s}$MSU - Iligan Institute of Technology (MSU-IIT), Iligan, Philippines\\
$^{t}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$^{u}$Novosibirsk State University, Novosibirsk, Russia\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}

==> Authorship_LHCb-PAPER-2021-032.tex <==
% LHCb collaboration author list
% Data extracted on July 8th, 2021 at 8:41pm for paper reference LHCb-PAPER-2021-032
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{32}$,
A.S.W.~Abdelmotteleb$^{56}$,
C.~Abell{\'a}n~Beteta$^{50}$,
F.J.~Abudinen~Gallego$^{56}$,
T.~Ackernley$^{60}$,
B.~Adeva$^{46}$,
M.~Adinolfi$^{54}$,
H.~Afsharnia$^{9}$,
C.~Agapopoulou$^{13}$,
C.A.~Aidala$^{87}$,
S.~Aiola$^{25}$,
Z.~Ajaltouni$^{9}$,
S.~Akar$^{65}$,
J.~Albrecht$^{15}$,
F.~Alessio$^{48}$,
M.~Alexander$^{59}$,
A.~Alfonso~Albero$^{45}$,
Z.~Aliouche$^{62}$,
G.~Alkhazov$^{38}$,
P.~Alvarez~Cartelle$^{55}$,
S.~Amato$^{2}$,
J.L.~Amey$^{54}$,
Y.~Amhis$^{11}$,
L.~An$^{48}$,
L.~Anderlini$^{22}$,
A.~Andreianov$^{38}$,
M.~Andreotti$^{21}$,
F.~Archilli$^{17}$,
A.~Artamonov$^{44}$,
M.~Artuso$^{68}$,
K.~Arzymatov$^{42}$,
E.~Aslanides$^{10}$,
M.~Atzeni$^{50}$,
B.~Audurier$^{12}$,
S.~Bachmann$^{17}$,
M.~Bachmayer$^{49}$,
J.J.~Back$^{56}$,
P.~Baladron~Rodriguez$^{46}$,
V.~Balagura$^{12}$,
W.~Baldini$^{21}$,
J.~Baptista~Leite$^{1}$,
M.~Barbetti$^{22,g}$,
R.J.~Barlow$^{62}$,
S.~Barsuk$^{11}$,
W.~Barter$^{61}$,
M.~Bartolini$^{24,h}$,
F.~Baryshnikov$^{83}$,
J.M.~Basels$^{14}$,
S.~Bashir$^{34}$,
G.~Bassi$^{29}$,
B.~Batsukh$^{68}$,
A.~Battig$^{15}$,
A.~Bay$^{49}$,
A.~Beck$^{56}$,
M.~Becker$^{15}$,
F.~Bedeschi$^{29}$,
I.~Bediaga$^{1}$,
A.~Beiter$^{68}$,
V.~Belavin$^{42}$,
S.~Belin$^{27}$,
V.~Bellee$^{50}$,
K.~Belous$^{44}$,
I.~Belov$^{40}$,
I.~Belyaev$^{41}$,
G.~Bencivenni$^{23}$,
E.~Ben-Haim$^{13}$,
A.~Berezhnoy$^{40}$,
R.~Bernet$^{50}$,
D.~Berninghoff$^{17}$,
H.C.~Bernstein$^{68}$,
C.~Bertella$^{48}$,
A.~Bertolin$^{28}$,
C.~Betancourt$^{50}$,
F.~Betti$^{48}$,
Ia.~Bezshyiko$^{50}$,
S.~Bhasin$^{54}$,
J.~Bhom$^{35}$,
L.~Bian$^{73}$,
M.S.~Bieker$^{15}$,
S.~Bifani$^{53}$,
P.~Billoir$^{13}$,
M.~Birch$^{61}$,
F.C.R.~Bishop$^{55}$,
A.~Bitadze$^{62}$,
A.~Bizzeti$^{22,k}$,
M.~Bj{\o}rn$^{63}$,
M.P.~Blago$^{48}$,
T.~Blake$^{56}$,
F.~Blanc$^{49}$,
S.~Blusk$^{68}$,
D.~Bobulska$^{59}$,
J.A.~Boelhauve$^{15}$,
O.~Boente~Garcia$^{46}$,
T.~Boettcher$^{65}$,
A.~Boldyrev$^{82}$,
A.~Bondar$^{43}$,
N.~Bondar$^{38,48}$,
S.~Borghi$^{62}$,
M.~Borisyak$^{42}$,
M.~Borsato$^{17}$,
J.T.~Borsuk$^{35}$,
S.A.~Bouchiba$^{49}$,
T.J.V.~Bowcock$^{60}$,
A.~Boyer$^{48}$,
C.~Bozzi$^{21}$,
M.J.~Bradley$^{61}$,
S.~Braun$^{66}$,
A.~Brea~Rodriguez$^{46}$,
J.~Brodzicka$^{35}$,
A.~Brossa~Gonzalo$^{56}$,
D.~Brundu$^{27}$,
A.~Buonaura$^{50}$,
L.~Buonincontri$^{28}$,
A.T.~Burke$^{62}$,
C.~Burr$^{48}$,
A.~Bursche$^{72}$,
A.~Butkevich$^{39}$,
J.S.~Butter$^{32}$,
J.~Buytaert$^{48}$,
W.~Byczynski$^{48}$,
S.~Cadeddu$^{27}$,
H.~Cai$^{73}$,
R.~Calabrese$^{21,f}$,
L.~Calefice$^{15,13}$,
L.~Calero~Diaz$^{23}$,
S.~Cali$^{23}$,
R.~Calladine$^{53}$,
M.~Calvi$^{26,j}$,
M.~Calvo~Gomez$^{85}$,
P.~Camargo~Magalhaes$^{54}$,
P.~Campana$^{23}$,
A.F.~Campoverde~Quezada$^{6}$,
S.~Capelli$^{26,j}$,
L.~Capriotti$^{20,d}$,
A.~Carbone$^{20,d}$,
G.~Carboni$^{31}$,
R.~Cardinale$^{24,h}$,
A.~Cardini$^{27}$,
I.~Carli$^{4}$,
P.~Carniti$^{26,j}$,
L.~Carus$^{14}$,
K.~Carvalho~Akiba$^{32}$,
A.~Casais~Vidal$^{46}$,
G.~Casse$^{60}$,
M.~Cattaneo$^{48}$,
G.~Cavallero$^{48}$,
S.~Celani$^{49}$,
J.~Cerasoli$^{10}$,
D.~Cervenkov$^{63}$,
A.J.~Chadwick$^{60}$,
M.G.~Chapman$^{54}$,
M.~Charles$^{13}$,
Ph.~Charpentier$^{48}$,
G.~Chatzikonstantinidis$^{53}$,
C.A.~Chavez~Barajas$^{60}$,
M.~Chefdeville$^{8}$,
C.~Chen$^{3}$,
S.~Chen$^{4}$,
A.~Chernov$^{35}$,
V.~Chobanova$^{46}$,
S.~Cholak$^{49}$,
M.~Chrzaszcz$^{35}$,
A.~Chubykin$^{38}$,
V.~Chulikov$^{38}$,
P.~Ciambrone$^{23}$,
M.F.~Cicala$^{56}$,
X.~Cid~Vidal$^{46}$,
G.~Ciezarek$^{48}$,
P.E.L.~Clarke$^{58}$,
M.~Clemencic$^{48}$,
H.V.~Cliff$^{55}$,
J.~Closier$^{48}$,
J.L.~Cobbledick$^{62}$,
V.~Coco$^{48}$,
J.A.B.~Coelho$^{11}$,
J.~Cogan$^{10}$,
E.~Cogneras$^{9}$,
L.~Cojocariu$^{37}$,
P.~Collins$^{48}$,
T.~Colombo$^{48}$,
L.~Congedo$^{19,c}$,
A.~Contu$^{27}$,
N.~Cooke$^{53}$,
G.~Coombs$^{59}$,
I.~Corredoira~$^{46}$,
G.~Corti$^{48}$,
C.M.~Costa~Sobral$^{56}$,
B.~Couturier$^{48}$,
D.C.~Craik$^{64}$,
J.~Crkovsk\'{a}$^{67}$,
M.~Cruz~Torres$^{1}$,
R.~Currie$^{58}$,
C.L.~Da~Silva$^{67}$,
S.~Dadabaev$^{83}$,
L.~Dai$^{71}$,
E.~Dall'Occo$^{15}$,
J.~Dalseno$^{46}$,
C.~D'Ambrosio$^{48}$,
A.~Danilina$^{41}$,
P.~d'Argent$^{48}$,
J.E.~Davies$^{62}$,
A.~Davis$^{62}$,
O.~De~Aguiar~Francisco$^{62}$,
K.~De~Bruyn$^{79}$,
S.~De~Capua$^{62}$,
M.~De~Cian$^{49}$,
J.M.~De~Miranda$^{1}$,
L.~De~Paula$^{2}$,
M.~De~Serio$^{19,c}$,
D.~De~Simone$^{50}$,
P.~De~Simone$^{23}$,
F.~De~Vellis$^{15}$,
J.A.~de~Vries$^{80}$,
C.T.~Dean$^{67}$,
F.~Debernardis$^{19,c}$,
D.~Decamp$^{8}$,
V.~Dedu$^{10}$,
L.~Del~Buono$^{13}$,
B.~Delaney$^{55}$,
H.-P.~Dembinski$^{15}$,
A.~Dendek$^{34}$,
V.~Denysenko$^{50}$,
D.~Derkach$^{82}$,
O.~Deschamps$^{9}$,
F.~Desse$^{11}$,
F.~Dettori$^{27,e}$,
B.~Dey$^{77}$,
A.~Di~Cicco$^{23}$,
P.~Di~Nezza$^{23}$,
S.~Didenko$^{83}$,
L.~Dieste~Maronas$^{46}$,
H.~Dijkstra$^{48}$,
V.~Dobishuk$^{52}$,
C.~Dong$^{3}$,
A.M.~Donohoe$^{18}$,
F.~Dordei$^{27}$,
A.C.~dos~Reis$^{1}$,
L.~Douglas$^{59}$,
A.~Dovbnya$^{51}$,
A.G.~Downes$^{8}$,
M.W.~Dudek$^{35}$,
L.~Dufour$^{48}$,
V.~Duk$^{78}$,
P.~Durante$^{48}$,
J.M.~Durham$^{67}$,
D.~Dutta$^{62}$,
A.~Dziurda$^{35}$,
A.~Dzyuba$^{38}$,
S.~Easo$^{57}$,
U.~Egede$^{69}$,
V.~Egorychev$^{41}$,
S.~Eidelman$^{43,u,\dagger}$,
S.~Eisenhardt$^{58}$,
S.~Ek-In$^{49}$,
L.~Eklund$^{59,86}$,
S.~Ely$^{68}$,
A.~Ene$^{37}$,
E.~Epple$^{67}$,
S.~Escher$^{14}$,
J.~Eschle$^{50}$,
S.~Esen$^{13}$,
T.~Evans$^{48}$,
A.~Falabella$^{20}$,
J.~Fan$^{3}$,
Y.~Fan$^{6}$,
B.~Fang$^{73}$,
S.~Farry$^{60}$,
D.~Fazzini$^{26,j}$,
M.~F{\'e}o$^{48}$,
A.~Fernandez~Prieto$^{46}$,
A.D.~Fernez$^{66}$,
F.~Ferrari$^{20,d}$,
L.~Ferreira~Lopes$^{49}$,
F.~Ferreira~Rodrigues$^{2}$,
S.~Ferreres~Sole$^{32}$,
M.~Ferrillo$^{50}$,
M.~Ferro-Luzzi$^{48}$,
S.~Filippov$^{39}$,
R.A.~Fini$^{19}$,
M.~Fiorini$^{21,f}$,
M.~Firlej$^{34}$,
K.M.~Fischer$^{63}$,
D.S.~Fitzgerald$^{87}$,
C.~Fitzpatrick$^{62}$,
T.~Fiutowski$^{34}$,
A.~Fkiaras$^{48}$,
F.~Fleuret$^{12}$,
M.~Fontana$^{13}$,
F.~Fontanelli$^{24,h}$,
R.~Forty$^{48}$,
D.~Foulds-Holt$^{55}$,
V.~Franco~Lima$^{60}$,
M.~Franco~Sevilla$^{66}$,
M.~Frank$^{48}$,
E.~Franzoso$^{21}$,
G.~Frau$^{17}$,
C.~Frei$^{48}$,
D.A.~Friday$^{59}$,
J.~Fu$^{6}$,
Q.~Fuehring$^{15}$,
E.~Gabriel$^{32}$,
G.~Galati$^{19,c}$,
A.~Gallas~Torreira$^{46}$,
D.~Galli$^{20,d}$,
S.~Gambetta$^{58,48}$,
Y.~Gan$^{3}$,
M.~Gandelman$^{2}$,
P.~Gandini$^{25}$,
Y.~Gao$^{5}$,
M.~Garau$^{27}$,
L.M.~Garcia~Martin$^{56}$,
P.~Garcia~Moreno$^{45}$,
J.~Garc{\'\i}a~Pardi{\~n}as$^{26,j}$,
B.~Garcia~Plana$^{46}$,
F.A.~Garcia~Rosales$^{12}$,
L.~Garrido$^{45}$,
C.~Gaspar$^{48}$,
R.E.~Geertsema$^{32}$,
D.~Gerick$^{17}$,
L.L.~Gerken$^{15}$,
E.~Gersabeck$^{62}$,
M.~Gersabeck$^{62}$,
T.~Gershon$^{56}$,
D.~Gerstel$^{10}$,
L.~Giambastiani$^{28}$,
V.~Gibson$^{55}$,
H.K.~Giemza$^{36}$,
A.L.~Gilman$^{63}$,
M.~Giovannetti$^{23,p}$,
A.~Giovent{\`u}$^{46}$,
P.~Gironella~Gironell$^{45}$,
L.~Giubega$^{37}$,
C.~Giugliano$^{21,f,48}$,
K.~Gizdov$^{58}$,
E.L.~Gkougkousis$^{48}$,
V.V.~Gligorov$^{13}$,
C.~G{\"o}bel$^{70}$,
E.~Golobardes$^{85}$,
D.~Golubkov$^{41}$,
A.~Golutvin$^{61,83}$,
A.~Gomes$^{1,a}$,
S.~Gomez~Fernandez$^{45}$,
F.~Goncalves~Abrantes$^{63}$,
M.~Goncerz$^{35}$,
G.~Gong$^{3}$,
P.~Gorbounov$^{41}$,
I.V.~Gorelov$^{40}$,
C.~Gotti$^{26}$,
E.~Govorkova$^{48}$,
J.P.~Grabowski$^{17}$,
T.~Grammatico$^{13}$,
L.A.~Granado~Cardoso$^{48}$,
E.~Graug{\'e}s$^{45}$,
E.~Graverini$^{49}$,
G.~Graziani$^{22}$,
A.~Grecu$^{37}$,
L.M.~Greeven$^{32}$,
N.A.~Grieser$^{4}$,
L.~Grillo$^{62}$,
S.~Gromov$^{83}$,
B.R.~Gruberg~Cazon$^{63}$,
C.~Gu$^{3}$,
M.~Guarise$^{21}$,
M.~Guittiere$^{11}$,
P. A.~G{\"u}nther$^{17}$,
E.~Gushchin$^{39}$,
A.~Guth$^{14}$,
Y.~Guz$^{44}$,
T.~Gys$^{48}$,
T.~Hadavizadeh$^{69}$,
G.~Haefeli$^{49}$,
C.~Haen$^{48}$,
J.~Haimberger$^{48}$,
T.~Halewood-leagas$^{60}$,
P.M.~Hamilton$^{66}$,
J.P.~Hammerich$^{60}$,
Q.~Han$^{7}$,
X.~Han$^{17}$,
T.H.~Hancock$^{63}$,
E.B.~Hansen$^{62}$,
S.~Hansmann-Menzemer$^{17}$,
N.~Harnew$^{63}$,
T.~Harrison$^{60}$,
C.~Hasse$^{48}$,
M.~Hatch$^{48}$,
J.~He$^{6,b}$,
M.~Hecker$^{61}$,
K.~Heijhoff$^{32}$,
K.~Heinicke$^{15}$,
A.M.~Hennequin$^{48}$,
K.~Hennessy$^{60}$,
L.~Henry$^{48}$,
J.~Heuel$^{14}$,
A.~Hicheur$^{2}$,
D.~Hill$^{49}$,
M.~Hilton$^{62}$,
S.E.~Hollitt$^{15}$,
R.~Hou$^{7}$,
Y.~Hou$^{8}$,
J.~Hu$^{17}$,
J.~Hu$^{72}$,
W.~Hu$^{7}$,
X.~Hu$^{3}$,
W.~Huang$^{6}$,
X.~Huang$^{73}$,
W.~Hulsbergen$^{32}$,
R.J.~Hunter$^{56}$,
M.~Hushchyn$^{82}$,
D.~Hutchcroft$^{60}$,
D.~Hynds$^{32}$,
P.~Ibis$^{15}$,
M.~Idzik$^{34}$,
D.~Ilin$^{38}$,
P.~Ilten$^{65}$,
A.~Inglessi$^{38}$,
A.~Ishteev$^{83}$,
K.~Ivshin$^{38}$,
R.~Jacobsson$^{48}$,
H.~Jage$^{14}$,
S.~Jakobsen$^{48}$,
E.~Jans$^{32}$,
B.K.~Jashal$^{47}$,
A.~Jawahery$^{66}$,
V.~Jevtic$^{15}$,
F.~Jiang$^{3}$,
M.~John$^{63}$,
D.~Johnson$^{48}$,
C.R.~Jones$^{55}$,
T.P.~Jones$^{56}$,
B.~Jost$^{48}$,
N.~Jurik$^{48}$,
S.H.~Kalavan~Kadavath$^{34}$,
S.~Kandybei$^{51}$,
Y.~Kang$^{3}$,
M.~Karacson$^{48}$,
M.~Karpov$^{82}$,
F.~Keizer$^{48}$,
D.M.~Keller$^{68}$,
M.~Kenzie$^{56}$,
T.~Ketel$^{33}$,
B.~Khanji$^{15}$,
A.~Kharisova$^{84}$,
S.~Kholodenko$^{44}$,
T.~Kirn$^{14}$,
V.S.~Kirsebom$^{49}$,
O.~Kitouni$^{64}$,
S.~Klaver$^{32}$,
N.~Kleijne$^{29}$,
K.~Klimaszewski$^{36}$,
M.R.~Kmiec$^{36}$,
S.~Koliiev$^{52}$,
A.~Kondybayeva$^{83}$,
A.~Konoplyannikov$^{41}$,
P.~Kopciewicz$^{34}$,
R.~Kopecna$^{17}$,
P.~Koppenburg$^{32}$,
M.~Korolev$^{40}$,
I.~Kostiuk$^{32,52}$,
O.~Kot$^{52}$,
S.~Kotriakhova$^{21,38}$,
P.~Kravchenko$^{38}$,
L.~Kravchuk$^{39}$,
R.D.~Krawczyk$^{48}$,
M.~Kreps$^{56}$,
F.~Kress$^{61}$,
S.~Kretzschmar$^{14}$,
P.~Krokovny$^{43,u}$,
W.~Krupa$^{34}$,
W.~Krzemien$^{36}$,
M.~Kucharczyk$^{35}$,
V.~Kudryavtsev$^{43,u}$,
H.S.~Kuindersma$^{32,33}$,
G.J.~Kunde$^{67}$,
T.~Kvaratskheliya$^{41}$,
D.~Lacarrere$^{48}$,
G.~Lafferty$^{62}$,
A.~Lai$^{27}$,
A.~Lampis$^{27}$,
D.~Lancierini$^{50}$,
J.J.~Lane$^{62}$,
R.~Lane$^{54}$,
G.~Lanfranchi$^{23}$,
C.~Langenbruch$^{14}$,
J.~Langer$^{15}$,
O.~Lantwin$^{83}$,
T.~Latham$^{56}$,
F.~Lazzari$^{29,q}$,
R.~Le~Gac$^{10}$,
S.H.~Lee$^{87}$,
R.~Lef{\`e}vre$^{9}$,
A.~Leflat$^{40}$,
S.~Legotin$^{83}$,
O.~Leroy$^{10}$,
T.~Lesiak$^{35}$,
B.~Leverington$^{17}$,
H.~Li$^{72}$,
P.~Li$^{17}$,
S.~Li$^{7}$,
Y.~Li$^{4}$,
Y.~Li$^{4}$,
Z.~Li$^{68}$,
X.~Liang$^{68}$,
T.~Lin$^{61}$,
R.~Lindner$^{48}$,
V.~Lisovskyi$^{15}$,
R.~Litvinov$^{27}$,
G.~Liu$^{72}$,
H.~Liu$^{6}$,
Q.~Liu$^{6}$,
S.~Liu$^{4}$,
A.~Lobo~Salvia$^{45}$,
A.~Loi$^{27}$,
J.~Lomba~Castro$^{46}$,
I.~Longstaff$^{59}$,
J.H.~Lopes$^{2}$,
S.~Lopez~Solino$^{46}$,
G.H.~Lovell$^{55}$,
Y.~Lu$^{4}$,
C.~Lucarelli$^{22,g}$,
D.~Lucchesi$^{28,l}$,
S.~Luchuk$^{39}$,
M.~Lucio~Martinez$^{32}$,
V.~Lukashenko$^{32,52}$,
Y.~Luo$^{3}$,
A.~Lupato$^{62}$,
E.~Luppi$^{21,f}$,
O.~Lupton$^{56}$,
A.~Lusiani$^{29,m}$,
X.~Lyu$^{6}$,
L.~Ma$^{4}$,
R.~Ma$^{6}$,
S.~Maccolini$^{20,d}$,
F.~Machefert$^{11}$,
F.~Maciuc$^{37}$,
V.~Macko$^{49}$,
P.~Mackowiak$^{15}$,
S.~Maddrell-Mander$^{54}$,
O.~Madejczyk$^{34}$,
L.R.~Madhan~Mohan$^{54}$,
O.~Maev$^{38}$,
A.~Maevskiy$^{82}$,
D.~Maisuzenko$^{38}$,
M.W.~Majewski$^{34}$,
J.J.~Malczewski$^{35}$,
S.~Malde$^{63}$,
B.~Malecki$^{48}$,
A.~Malinin$^{81}$,
T.~Maltsev$^{43,u}$,
H.~Malygina$^{17}$,
G.~Manca$^{27,e}$,
G.~Mancinelli$^{10}$,
D.~Manuzzi$^{20,d}$,
D.~Marangotto$^{25,i}$,
J.~Maratas$^{9,s}$,
J.F.~Marchand$^{8}$,
U.~Marconi$^{20}$,
S.~Mariani$^{22,g}$,
C.~Marin~Benito$^{48}$,
M.~Marinangeli$^{49}$,
J.~Marks$^{17}$,
A.M.~Marshall$^{54}$,
P.J.~Marshall$^{60}$,
G.~Martelli$^{78}$,
G.~Martellotti$^{30}$,
L.~Martinazzoli$^{48,j}$,
M.~Martinelli$^{26,j}$,
D.~Martinez~Santos$^{46}$,
F.~Martinez~Vidal$^{47}$,
A.~Massafferri$^{1}$,
M.~Materok$^{14}$,
R.~Matev$^{48}$,
A.~Mathad$^{50}$,
V.~Matiunin$^{41}$,
C.~Matteuzzi$^{26}$,
K.R.~Mattioli$^{87}$,
A.~Mauri$^{32}$,
E.~Maurice$^{12}$,
J.~Mauricio$^{45}$,
M.~Mazurek$^{48}$,
M.~McCann$^{61}$,
L.~Mcconnell$^{18}$,
T.H.~Mcgrath$^{62}$,
N.T.~Mchugh$^{59}$,
A.~McNab$^{62}$,
R.~McNulty$^{18}$,
J.V.~Mead$^{60}$,
B.~Meadows$^{65}$,
G.~Meier$^{15}$,
N.~Meinert$^{76}$,
D.~Melnychuk$^{36}$,
S.~Meloni$^{26,j}$,
M.~Merk$^{32,80}$,
A.~Merli$^{25}$,
L.~Meyer~Garcia$^{2}$,
M.~Mikhasenko$^{48}$,
D.A.~Milanes$^{74}$,
E.~Millard$^{56}$,
M.~Milovanovic$^{48}$,
M.-N.~Minard$^{8}$,
A.~Minotti$^{26,j}$,
L.~Minzoni$^{21,f}$,
S.E.~Mitchell$^{58}$,
B.~Mitreska$^{62}$,
D.S.~Mitzel$^{15}$,
A.~M{\"o}dden~$^{15}$,
R.A.~Mohammed$^{63}$,
R.D.~Moise$^{61}$,
S.~Mokhnenko$^{82}$,
T.~Momb{\"a}cher$^{46}$,
I.A.~Monroy$^{74}$,
S.~Monteil$^{9}$,
M.~Morandin$^{28}$,
G.~Morello$^{23}$,
M.J.~Morello$^{29,m}$,
J.~Moron$^{34}$,
A.B.~Morris$^{75}$,
A.G.~Morris$^{56}$,
R.~Mountain$^{68}$,
H.~Mu$^{3}$,
F.~Muheim$^{58,48}$,
M.~Mulder$^{48}$,
D.~M{\"u}ller$^{48}$,
K.~M{\"u}ller$^{50}$,
C.H.~Murphy$^{63}$,
D.~Murray$^{62}$,
P.~Muzzetto$^{27,48}$,
P.~Naik$^{54}$,
T.~Nakada$^{49}$,
R.~Nandakumar$^{57}$,
T.~Nanut$^{49}$,
I.~Nasteva$^{2}$,
M.~Needham$^{58}$,
I.~Neri$^{21}$,
N.~Neri$^{25,i}$,
S.~Neubert$^{75}$,
N.~Neufeld$^{48}$,
R.~Newcombe$^{61}$,
E.M.~Niel$^{11}$,
S.~Nieswand$^{14}$,
N.~Nikitin$^{40}$,
N.S.~Nolte$^{64}$,
C.~Normand$^{8}$,
C.~Nunez$^{87}$,
A.~Oblakowska-Mucha$^{34}$,
V.~Obraztsov$^{44}$,
T.~Oeser$^{14}$,
D.P.~O'Hanlon$^{54}$,
S.~Okamura$^{21}$,
R.~Oldeman$^{27,e}$,
F.~Oliva$^{58}$,
M.E.~Olivares$^{68}$,
C.J.G.~Onderwater$^{79}$,
R.H.~O'neil$^{58}$,
J.M.~Otalora~Goicochea$^{2}$,
T.~Ovsiannikova$^{41}$,
P.~Owen$^{50}$,
A.~Oyanguren$^{47}$,
K.O.~Padeken$^{75}$,
B.~Pagare$^{56}$,
P.R.~Pais$^{48}$,
T.~Pajero$^{63}$,
A.~Palano$^{19}$,
M.~Palutan$^{23}$,
Y.~Pan$^{62}$,
G.~Panshin$^{84}$,
A.~Papanestis$^{57}$,
M.~Pappagallo$^{19,c}$,
L.L.~Pappalardo$^{21,f}$,
C.~Pappenheimer$^{65}$,
W.~Parker$^{66}$,
C.~Parkes$^{62}$,
B.~Passalacqua$^{21}$,
G.~Passaleva$^{22}$,
A.~Pastore$^{19}$,
M.~Patel$^{61}$,
C.~Patrignani$^{20,d}$,
C.J.~Pawley$^{80}$,
A.~Pearce$^{48}$,
A.~Pellegrino$^{32}$,
M.~Pepe~Altarelli$^{48}$,
S.~Perazzini$^{20}$,
D.~Pereima$^{41}$,
A.~Pereiro~Castro$^{46}$,
P.~Perret$^{9}$,
M.~Petric$^{59,48}$,
K.~Petridis$^{54}$,
A.~Petrolini$^{24,h}$,
A.~Petrov$^{81}$,
S.~Petrucci$^{58}$,
M.~Petruzzo$^{25}$,
T.T.H.~Pham$^{68}$,
L.~Pica$^{29,m}$,
M.~Piccini$^{78}$,
B.~Pietrzyk$^{8}$,
G.~Pietrzyk$^{49}$,
M.~Pili$^{63}$,
D.~Pinci$^{30}$,
F.~Pisani$^{48}$,
M.~Pizzichemi$^{26,48,j}$,
Resmi ~P.K$^{10}$,
V.~Placinta$^{37}$,
J.~Plews$^{53}$,
M.~Plo~Casasus$^{46}$,
F.~Polci$^{13}$,
M.~Poli~Lener$^{23}$,
M.~Poliakova$^{68}$,
A.~Poluektov$^{10}$,
N.~Polukhina$^{83,t}$,
I.~Polyakov$^{68}$,
E.~Polycarpo$^{2}$,
S.~Ponce$^{48}$,
D.~Popov$^{6,48}$,
S.~Popov$^{42}$,
S.~Poslavskii$^{44}$,
K.~Prasanth$^{35}$,
L.~Promberger$^{48}$,
C.~Prouve$^{46}$,
V.~Pugatch$^{52}$,
V.~Puill$^{11}$,
H.~Pullen$^{63}$,
G.~Punzi$^{29,n}$,
H.~Qi$^{3}$,
W.~Qian$^{6}$,
J.~Qin$^{6}$,
N.~Qin$^{3}$,
R.~Quagliani$^{49}$,
B.~Quintana$^{8}$,
N.V.~Raab$^{18}$,
R.I.~Rabadan~Trejo$^{6}$,
B.~Rachwal$^{34}$,
J.H.~Rademacker$^{54}$,
M.~Rama$^{29}$,
M.~Ramos~Pernas$^{56}$,
M.S.~Rangel$^{2}$,
F.~Ratnikov$^{42,82}$,
G.~Raven$^{33}$,
M.~Reboud$^{8}$,
F.~Redi$^{49}$,
F.~Reiss$^{62}$,
C.~Remon~Alepuz$^{47}$,
Z.~Ren$^{3}$,
V.~Renaudin$^{63}$,
R.~Ribatti$^{29}$,
S.~Ricciardi$^{57}$,
K.~Rinnert$^{60}$,
P.~Robbe$^{11}$,
G.~Robertson$^{58}$,
A.B.~Rodrigues$^{49}$,
E.~Rodrigues$^{60}$,
J.A.~Rodriguez~Lopez$^{74}$,
E.R.R.~Rodriguez~Rodriguez$^{46}$,
A.~Rollings$^{63}$,
P.~Roloff$^{48}$,
V.~Romanovskiy$^{44}$,
M.~Romero~Lamas$^{46}$,
A.~Romero~Vidal$^{46}$,
J.D.~Roth$^{87}$,
M.~Rotondo$^{23}$,
M.S.~Rudolph$^{68}$,
T.~Ruf$^{48}$,
R.A.~Ruiz~Fernandez$^{46}$,
J.~Ruiz~Vidal$^{47}$,
A.~Ryzhikov$^{82}$,
J.~Ryzka$^{34}$,
J.J.~Saborido~Silva$^{46}$,
N.~Sagidova$^{38}$,
N.~Sahoo$^{56}$,
B.~Saitta$^{27,e}$,
M.~Salomoni$^{48}$,
C.~Sanchez~Gras$^{32}$,
R.~Santacesaria$^{30}$,
C.~Santamarina~Rios$^{46}$,
M.~Santimaria$^{23}$,
E.~Santovetti$^{31,p}$,
D.~Saranin$^{83}$,
G.~Sarpis$^{14}$,
M.~Sarpis$^{75}$,
A.~Sarti$^{30}$,
C.~Satriano$^{30,o}$,
A.~Satta$^{31}$,
M.~Saur$^{15}$,
D.~Savrina$^{41,40}$,
H.~Sazak$^{9}$,
L.G.~Scantlebury~Smead$^{63}$,
A.~Scarabotto$^{13}$,
S.~Schael$^{14}$,
S.~Scherl$^{60}$,
M.~Schiller$^{59}$,
H.~Schindler$^{48}$,
M.~Schmelling$^{16}$,
B.~Schmidt$^{48}$,
S.~Schmitt$^{14}$,
O.~Schneider$^{49}$,
A.~Schopper$^{48}$,
M.~Schubiger$^{32}$,
S.~Schulte$^{49}$,
M.H.~Schune$^{11}$,
R.~Schwemmer$^{48}$,
B.~Sciascia$^{23,48}$,
S.~Sellam$^{46}$,
A.~Semennikov$^{41}$,
M.~Senghi~Soares$^{33}$,
A.~Sergi$^{24,h}$,
N.~Serra$^{50}$,
L.~Sestini$^{28}$,
A.~Seuthe$^{15}$,
Y.~Shang$^{5}$,
D.M.~Shangase$^{87}$,
M.~Shapkin$^{44}$,
I.~Shchemerov$^{83}$,
L.~Shchutska$^{49}$,
T.~Shears$^{60}$,
L.~Shekhtman$^{43,u}$,
Z.~Shen$^{5}$,
V.~Shevchenko$^{81}$,
E.B.~Shields$^{26,j}$,
Y.~Shimizu$^{11}$,
E.~Shmanin$^{83}$,
J.D.~Shupperd$^{68}$,
B.G.~Siddi$^{21}$,
R.~Silva~Coutinho$^{50}$,
G.~Simi$^{28}$,
S.~Simone$^{19,c}$,
N.~Skidmore$^{62}$,
T.~Skwarnicki$^{68}$,
M.W.~Slater$^{53}$,
I.~Slazyk$^{21,f}$,
J.C.~Smallwood$^{63}$,
J.G.~Smeaton$^{55}$,
A.~Smetkina$^{41}$,
E.~Smith$^{50}$,
M.~Smith$^{61}$,
A.~Snoch$^{32}$,
M.~Soares$^{20}$,
L.~Soares~Lavra$^{9}$,
M.D.~Sokoloff$^{65}$,
F.J.P.~Soler$^{59}$,
A.~Solovev$^{38}$,
I.~Solovyev$^{38}$,
F.L.~Souza~De~Almeida$^{2}$,
B.~Souza~De~Paula$^{2}$,
B.~Spaan$^{15}$,
E.~Spadaro~Norella$^{25}$,
P.~Spradlin$^{59}$,
F.~Stagni$^{48}$,
M.~Stahl$^{65}$,
S.~Stahl$^{48}$,
S.~Stanislaus$^{63}$,
O.~Steinkamp$^{50,83}$,
O.~Stenyakin$^{44}$,
H.~Stevens$^{15}$,
S.~Stone$^{68}$,
M.~Straticiuc$^{37}$,
D.~Strekalina$^{83}$,
F.~Suljik$^{63}$,
J.~Sun$^{27}$,
L.~Sun$^{73}$,
Y.~Sun$^{66}$,
P.~Svihra$^{62}$,
P.N.~Swallow$^{53}$,
K.~Swientek$^{34}$,
A.~Szabelski$^{36}$,
T.~Szumlak$^{34}$,
M.~Szymanski$^{48}$,
S.~Taneja$^{62}$,
A.R.~Tanner$^{54}$,
M.D.~Tat$^{63}$,
A.~Terentev$^{83}$,
F.~Teubert$^{48}$,
E.~Thomas$^{48}$,
D.J.D.~Thompson$^{53}$,
K.A.~Thomson$^{60}$,
V.~Tisserand$^{9}$,
S.~T'Jampens$^{8}$,
M.~Tobin$^{4}$,
L.~Tomassetti$^{21,f}$,
X.~Tong$^{5}$,
D.~Torres~Machado$^{1}$,
D.Y.~Tou$^{13}$,
E.~Trifonova$^{83}$,
C.~Trippl$^{49}$,
G.~Tuci$^{6}$,
A.~Tully$^{49}$,
N.~Tuning$^{32,48}$,
A.~Ukleja$^{36}$,
D.J.~Unverzagt$^{17}$,
E.~Ursov$^{83}$,
A.~Usachov$^{32}$,
A.~Ustyuzhanin$^{42,82}$,
U.~Uwer$^{17}$,
A.~Vagner$^{84}$,
V.~Vagnoni$^{20}$,
A.~Valassi$^{48}$,
G.~Valenti$^{20}$,
N.~Valls~Canudas$^{85}$,
M.~van~Beuzekom$^{32}$,
M.~Van~Dijk$^{49}$,
E.~van~Herwijnen$^{83}$,
C.B.~Van~Hulse$^{18}$,
M.~van~Veghel$^{79}$,
R.~Vazquez~Gomez$^{45}$,
P.~Vazquez~Regueiro$^{46}$,
C.~V{\'a}zquez~Sierra$^{48}$,
S.~Vecchi$^{21}$,
J.J.~Velthuis$^{54}$,
M.~Veltri$^{22,r}$,
A.~Venkateswaran$^{68}$,
M.~Veronesi$^{32}$,
M.~Vesterinen$^{56}$,
D.~~Vieira$^{65}$,
M.~Vieites~Diaz$^{49}$,
H.~Viemann$^{76}$,
X.~Vilasis-Cardona$^{85}$,
E.~Vilella~Figueras$^{60}$,
A.~Villa$^{20}$,
P.~Vincent$^{13}$,
F.C.~Volle$^{11}$,
D.~Vom~Bruch$^{10}$,
A.~Vorobyev$^{38}$,
V.~Vorobyev$^{43,u}$,
N.~Voropaev$^{38}$,
K.~Vos$^{80}$,
R.~Waldi$^{17}$,
J.~Walsh$^{29}$,
C.~Wang$^{17}$,
J.~Wang$^{5}$,
J.~Wang$^{4}$,
J.~Wang$^{3}$,
J.~Wang$^{73}$,
M.~Wang$^{3}$,
R.~Wang$^{54}$,
Y.~Wang$^{7}$,
Z.~Wang$^{50}$,
Z.~Wang$^{3}$,
Z.~Wang$^{6}$,
J.A.~Ward$^{56}$,
N.K.~Watson$^{53}$,
S.G.~Weber$^{13}$,
D.~Websdale$^{61}$,
C.~Weisser$^{64}$,
B.D.C.~Westhenry$^{54}$,
D.J.~White$^{62}$,
M.~Whitehead$^{54}$,
A.R.~Wiederhold$^{56}$,
D.~Wiedner$^{15}$,
G.~Wilkinson$^{63}$,
M.~Wilkinson$^{68}$,
I.~Williams$^{55}$,
M.~Williams$^{64}$,
M.R.J.~Williams$^{58}$,
F.F.~Wilson$^{57}$,
W.~Wislicki$^{36}$,
M.~Witek$^{35}$,
L.~Witola$^{17}$,
G.~Wormser$^{11}$,
S.A.~Wotton$^{55}$,
H.~Wu$^{68}$,
K.~Wyllie$^{48}$,
Z.~Xiang$^{6}$,
D.~Xiao$^{7}$,
Y.~Xie$^{7}$,
A.~Xu$^{5}$,
J.~Xu$^{6}$,
L.~Xu$^{3}$,
M.~Xu$^{7}$,
Q.~Xu$^{6}$,
Z.~Xu$^{5}$,
Z.~Xu$^{6}$,
D.~Yang$^{3}$,
S.~Yang$^{6}$,
Y.~Yang$^{6}$,
Z.~Yang$^{5}$,
Z.~Yang$^{66}$,
Y.~Yao$^{68}$,
L.E.~Yeomans$^{60}$,
H.~Yin$^{7}$,
J.~Yu$^{71}$,
X.~Yuan$^{68}$,
O.~Yushchenko$^{44}$,
E.~Zaffaroni$^{49}$,
M.~Zavertyaev$^{16,t}$,
M.~Zdybal$^{35}$,
O.~Zenaiev$^{48}$,
M.~Zeng$^{3}$,
D.~Zhang$^{7}$,
L.~Zhang$^{3}$,
S.~Zhang$^{71}$,
S.~Zhang$^{5}$,
Y.~Zhang$^{5}$,
Y.~Zhang$^{63}$,
A.~Zharkova$^{83}$,
A.~Zhelezov$^{17}$,
Y.~Zheng$^{6}$,
T.~Zhou$^{5}$,
X.~Zhou$^{6}$,
Y.~Zhou$^{6}$,
V.~Zhovkovska$^{11}$,
X.~Zhu$^{3}$,
X.~Zhu$^{7}$,
Z.~Zhu$^{6}$,
V.~Zhukov$^{14,40}$,
J.B.~Zonneveld$^{58}$,
Q.~Zou$^{4}$,
S.~Zucchelli$^{20,d}$,
D.~Zuliani$^{28}$,
G.~Zunica$^{62}$.\bigskip

{\footnotesize \it

$^{1}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$^{4}$Institute Of High Energy Physics (IHEP), Beijing, China\\
$^{5}$School of Physics State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China\\
$^{6}$University of Chinese Academy of Sciences, Beijing, China\\
$^{7}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China\\
$^{8}$Univ. Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$^{9}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$^{10}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$^{11}$Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\\
$^{12}$Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, Institut Polytechnique de Paris, Palaiseau, France\\
$^{13}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$^{14}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$^{15}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{16}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$^{17}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$^{18}$School of Physics, University College Dublin, Dublin, Ireland\\
$^{19}$INFN Sezione di Bari, Bari, Italy\\
$^{20}$INFN Sezione di Bologna, Bologna, Italy\\
$^{21}$INFN Sezione di Ferrara, Ferrara, Italy\\
$^{22}$INFN Sezione di Firenze, Firenze, Italy\\
$^{23}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{24}$INFN Sezione di Genova, Genova, Italy\\
$^{25}$INFN Sezione di Milano, Milano, Italy\\
$^{26}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$^{27}$INFN Sezione di Cagliari, Monserrato, Italy\\
$^{28}$Universita degli Studi di Padova, Universita e INFN, Padova, Padova, Italy\\
$^{29}$INFN Sezione di Pisa, Pisa, Italy\\
$^{30}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$^{31}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$^{32}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$^{33}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$^{34}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$^{35}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$^{36}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$^{37}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$^{38}$Petersburg Nuclear Physics Institute NRC Kurchatov Institute (PNPI NRC KI), Gatchina, Russia\\
$^{39}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), Moscow, Russia\\
$^{40}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia\\
$^{41}$Institute of Theoretical and Experimental Physics NRC Kurchatov Institute (ITEP NRC KI), Moscow, Russia\\
$^{42}$Yandex School of Data Analysis, Moscow, Russia\\
$^{43}$Budker Institute of Nuclear Physics (SB RAS), Novosibirsk, Russia\\
$^{44}$Institute for High Energy Physics NRC Kurchatov Institute (IHEP NRC KI), Protvino, Russia, Protvino, Russia\\
$^{45}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$^{46}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$^{47}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain\\
$^{48}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{49}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{50}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$^{51}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$^{52}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$^{53}$University of Birmingham, Birmingham, United Kingdom\\
$^{54}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$^{55}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{56}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{57}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{58}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{59}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{60}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{61}$Imperial College London, London, United Kingdom\\
$^{62}$Department of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{63}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$^{64}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$^{65}$University of Cincinnati, Cincinnati, OH, United States\\
$^{66}$University of Maryland, College Park, MD, United States\\
$^{67}$Los Alamos National Laboratory (LANL), Los Alamos, United States\\
$^{68}$Syracuse University, Syracuse, NY, United States\\
$^{69}$School of Physics and Astronomy, Monash University, Melbourne, Australia, associated to $^{56}$\\
$^{70}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$^{71}$Physics and Micro Electronic College, Hunan University, Changsha City, China, associated to $^{7}$\\
$^{72}$Guangdong Provincial Key Laboratory of Nuclear Science, Guangdong-Hong Kong Joint Laboratory of Quantum Matter, Institute of Quantum Matter, South China Normal University, Guangzhou, China, associated to $^{3}$\\
$^{73}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{3}$\\
$^{74}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{13}$\\
$^{75}$Universit{\"a}t Bonn - Helmholtz-Institut f{\"u}r Strahlen und Kernphysik, Bonn, Germany, associated to $^{17}$\\
$^{76}$Institut f{\"u}r Physik, Universit{\"a}t Rostock, Rostock, Germany, associated to $^{17}$\\
$^{77}$Eotvos Lorand University, Budapest, Hungary, associated to $^{48}$\\
$^{78}$INFN Sezione di Perugia, Perugia, Italy, associated to $^{21}$\\
$^{79}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{32}$\\
$^{80}$Universiteit Maastricht, Maastricht, Netherlands, associated to $^{32}$\\
$^{81}$National Research Centre Kurchatov Institute, Moscow, Russia, associated to $^{41}$\\
$^{82}$National Research University Higher School of Economics, Moscow, Russia, associated to $^{42}$\\
$^{83}$National University of Science and Technology ``MISIS'', Moscow, Russia, associated to $^{41}$\\
$^{84}$National Research Tomsk Polytechnic University, Tomsk, Russia, associated to $^{41}$\\
$^{85}$DS4DS, La Salle, Universitat Ramon Llull, Barcelona, Spain, associated to $^{45}$\\
$^{86}$Department of Physics and Astronomy, Uppsala University, Uppsala, Sweden, associated to $^{59}$\\
$^{87}$University of Michigan, Ann Arbor, United States, associated to $^{68}$\\
\bigskip
$^{a}$Universidade Federal do Tri{\^a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$^{b}$Hangzhou Institute for Advanced Study, UCAS, Hangzhou, China\\
$^{c}$Universit{\`a} di Bari, Bari, Italy\\
$^{d}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{e}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{f}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{g}$Universit{\`a} di Firenze, Firenze, Italy\\
$^{h}$Universit{\`a} di Genova, Genova, Italy\\
$^{i}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{j}$Universit{\`a} di Milano Bicocca, Milano, Italy\\
$^{k}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$^{l}$Universit{\`a} di Padova, Padova, Italy\\
$^{m}$Scuola Normale Superiore, Pisa, Italy\\
$^{n}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{o}$Universit{\`a} della Basilicata, Potenza, Italy\\
$^{p}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{q}$Universit{\`a} di Siena, Siena, Italy\\
$^{r}$Universit{\`a} di Urbino, Urbino, Italy\\
$^{s}$MSU - Iligan Institute of Technology (MSU-IIT), Iligan, Philippines\\
$^{t}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$^{u}$Novosibirsk State University, Novosibirsk, Russia\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}

==> LHCb_Authorship_DD-MMM-20YY.tex <==
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}




==> captions.tex <==
%% figure captions 

\subsection*{Figure Legends/Captions (for main text figures)}


Figure 1: {\bf Distribution of \Dz\Dz\pip~mass}.
    Distribution of \Dz\Dz\pip~mass where 
   the~contribution of the~non\protect\nobreakdash-$\Dz$ 
   background has been statistically subtracted.
   The~result of the~fit described in the~text is overlaid. 
   %% 
   %% {\color{red}{
   Uncertainties on the~data points are statistical
 only and represent one standard deviation, 
 calculated as a~sum in quadrature of the~assigned weights from 
 the~background\protect\nobreakdash-subtraction procedure.
 %% }}
 

Figure~2: {\bf Likelihood profile for the~$\left|g\right|$~parameter.} 
  Likelihood profile for the~absolute value of 
  the~coupling constant $g$
  from the~fit to the~background\protect\nobreakdash-subtracted 
  $\Dz\Dz\pip$~mass spectrum with a~model based 
  on the~$\mathfrak{F}^{\mathrm{U}}$~signal profile.
  

 Figure~3: {\bf Mass distribution for \Dz\pip~pairs. }
  Mass distribution for \Dz\pip~pairs
  from  selected $\Dz\Dz\pip$~candidates 
  with a~mass below the $\Dstarp\Dz$~mass threshold
  with  non\protect\nobreakdash-\Dz~background subtracted. 
  %% 
  The~overlaid fit result
  is described in the~text. 
  %%
  %% {\color{red}{
  The~background component vanishes in the~fit.
  %% }} 
  %% 
   %% {\color{red}{
   Uncertainties on the~data points are statistical
 only and represent one standard deviation, 
 calculated as a~sum in quadrature of the~assigned weights from 
 the~background\protect\nobreakdash-subtraction procedure.
 %% }}
 
 
Figure~4: {\bf
  Mass distributions for selected 
  $\Dz\Dz$, 
  $\Dp\Dz$
  $\Dp\Dp$ and $\Dp\Dz\pip$~combinations.
  }
  (Top) \D\D~and $\D\D\pip$~mass distributions
  for
  selected 
  (left)~\Dz\Dz
  and (right)~\Dp\Dz~candidates 
  with the~non\protect\nobreakdash-\D~background subtracted. 
  %%
  The~overlaid fit results
  are described in the~text.
  %%
  For~visibility
  the~\mbox{$\decay{\Tcc}{\Dp\Dz\piz}$}
  is stacked
  on top of the~\mbox{$\decay{\Tcc}{\Dp\Dz\g}$}~component.
  %%
  (Bottom) 
  Mass distributions 
  for
  selected 
  (left)~\Dp\Dp
  and (right)~\Dp\Dz\pip~candidates 
  with the
  non\protect\nobreakdash-\D~background subtracted. 
  %% 
  The~vertical coloured band indicates 
  the~expected mass
  for  the~hypothetical
  $\hat{\PT}^{++}_{\cquark\cquark}$~state. 
  The~overlaid fit results
  with background\protect\nobreakdash-only 
  functions
  are described in the~text. 
  %%
  %% {\color{red}{
  Uncertainties on the~data points are statistical
 only and represent one standard deviation, 
 calculated as a~sum in quadrature of the~assigned weights from 
 the~background\protect\nobreakdash-subtraction procedure.
 %%}}
 
  

  
Figure~5: {\bf
  Complex plane of 
  the~$\updelta \sqrt{s}$ 
  variable.
  }
  Complex plane of 
  the~$\updelta \sqrt{s}$~variable.
  The~dashed red line shows the~allowed region
  for large $\left| g\right|$~values.
  The~filled red circle indicates 
  the~best estimate for 
  the~pole location and the filled regions show 
  $1\upsigma$ and $2\upsigma$~confidence regions. 
  Open blue and green circles show 
  the~branch points corresponding 
  to the~$\Dstarp\Dz$ and 
  $\Dstarz\Dp$~channels, respectively, and 
  the corresponding blue and green lines 
  indicate branch cuts.  
  Three other branch points at 
  $\sqrt{s}$ of \mbox{$m_{\Dz}+m_{\Dp}$},
  \mbox{$m_{\Dz}+m_{\Dp}+m_{\piz}$} 
  and \mbox{$2m_{\Dz}+m_{\pip}$},
  corresponding to the~openings of 
  the~$\Dz\Dp\gamma$, $\Dz\Dp\piz$
  and $\Dz\Dz\pip$~decay channels, 
  are outside of the~displayed region. 
  
  
  Figure~6:
  {\bf Track multiplicity and transverse momentum distributions.}
  (left)~Background\protect\nobreakdash-subtracted distributions
  for the~multiplicity of tracks 
  reconstructed 
  in the~vertex detector 
  for (red circles)~\mbox{$\decay{\Tcc}{\Dz\Dz\pip}$}~signal,
  low\protect\nobreakdash-mass~(blue open squares) $\Dz\Dzb$~and (green filled diamonds)
  $\Dz\Dz$~pairs.
  The~binning scheme is chosen to have 
  an~approximately uniform 
  distribution for \Dz\Dzb~pairs.
  The~distributions for 
  the~$\Dz\Dzb$~and 
  $\Dz\Dz$~pairs are 
  normalised to the~same yields 
  as the~$\decay{\Tcc}{\Dz\Dz\pip}$~signal.
  %%
  (right)~Background-subtracted
  transverse momentum spectra 
  for (red circles)~\mbox{$\decay{\Tcc}
  {\Dz\Dz\pip}$}~signal,
  (blue open squares)~low-mass $\Dz\Dzb$
  and (green filled diamonds)
  $\Dz\Dz$~pairs.
  The binning scheme is chosen to have 
  an approximately uniform distribution for \Dz\Dzb~pairs.
  The distributions for 
  the~$\Dz\Dzb$~and 
  $\Dz\Dz$~pairs are 
  normalised to the~same yields 
  as $\decay{\Tcc}{\Dz\Dz\pip}$~signal.
  For~better visualisation, the
  points are slightly displaced from 
  the~bin centres. 
  %% 
  For~better visualisation, 
  the~points are slightly 
  displaced from the~bin centres.
  %%
  %% {\color{red}{
  Uncertainties on the~data points are statistical
 only and represent one standard deviation, 
 %% }}

 
 
  
Figure~7:
  {\bf Mass distributions for \Dz\Dz and \Dz\Dzb~candidates.}
  Background\protect\nobreakdash-subtracted 
  \Dz\Dz and \Dz\Dzb~mass distributions.
  The~near\protect\nobreakdash-threshold enhancement in 
   the $\Dz\Dz$ channel corresponds to partially reconstructed 
   ${\Tcc\to\Dz\Dz\pip}$ decays, while in the~$\Dz\Dzb$ channel 
   the~threshold enhancement
   corresponds to partially reconstructed 
   $\chicone(3872)\to\Dz\Dzb\piz$ decays.
   %%
   %% {\color{red}{
   The~$\Dz\Dzb$~mass distribution
   is zero\protect\nobreakdash-suppressed for better visualisation. 
   %% }}
   %% 
   %% {\color{red}{
   Uncertainties on the~data points are statistical
 only and represent one standard deviation, 
 calculated as a~sum in quadrature of the~assigned weights from 
 the~background\protect\nobreakdash-subtraction procedure.
   %% }}
   %%

==> detector.tex <==
\subsection*{Experimental setup}\label{sec:detector}

The \lhcb detector~\cite{LHCb-DP-2008-001,LHCb-DP-2014-002} is a single-arm forward
spectrometer covering the~pseudorapidity range $2<\eta <5$,
designed for the study of particles containing \bquark or \cquark
quarks. The detector includes a high-precision tracking system
consisting of a~silicon\nobreakdash-strip vertex detector surrounding 
the~$\proton\proton$~interaction region,
%%~\cite{LHCb-DP-2014-001}\verb!*!, 
a~large-area silicon-strip detector located
upstream of a~dipole magnet with a~bending power of about
$4{\mathrm{\,Tm}}$, and three stations of silicon\nobreakdash-strip detectors and straw
drift tubes
%%
placed downstream of the magnet.
The~tracking system provides a measurement of the momentum, \ptot, 
of charged particles with
a~relative uncertainty that varies from 0.5\% at low momentum to 1.0\% at 200\gevc.
The minimum distance of a track to 
a~primary $\proton\proton$~collision vertex\,(PV), 
the~impact parameter\,(IP), 
is measured with a resolution of $(15+29/\pt)\mum$,
where \pt is the component of the momentum transverse to the beam, in\,\gevc.
Different types of charged hadrons are distinguished using information
from two ring-imaging Cherenkov detectors~\cite{LHCb-DP-2012-003}. 
Photons, electrons and hadrons are identified by 
a~calorimeter system consisting of
scintillating-pad and preshower detectors, an electromagnetic
% calorimeter
and a hadronic calorimeter. 
Muons are identified by a~system composed of 
alternating layers of iron and multiwire
proportional chambers.
%% ~\cite{LHCb-DP-2012-002}\verb!*!.
%% 
The~online event selection is performed by 
a~trigger, 
%% ~\cite{LHCb-DP-2012-004}, 
which consists of a~hardware stage, based on information from 
the~calorimeter and muon systems, 
followed by a~software stage, which applies a full event
reconstruction.

\subsection*{Simulation}
Simulation is required to model 
the~effects of the~detector acceptance, 
resolution, 
and the~efficiency of 
the~imposed selection requirements.
In~the~simulation, $\proton\proton$~collisions 
are generated using
  \pythia~\cite{Sjostrand:2007gs}%% ,*Sjostrand:2006za} 
  with a~specific 
  \lhcb configuration~\cite{LHCb-PROC-2010-056}.
  Decays of unstable particles
  are described by \evtgen~\cite{Lange:2001uf}, 
  in which final-state
  radiation is generated 
  using \photos~\cite{davidson2015photos}.
  The~interaction of the~generated particles 
  with the~detector, and its response,
  are implemented using the~\geant
  toolkit~\cite{Allison:2006ve, 
  *Agostinelli:2002hh} as described in
  Ref.~\cite{LHCb-PROC-2011-006}. 




==> extended.tex <==
\renewcommand{\figurename}{\bf Extended Data Fig.}

\section*{Extended Data}

\begin{figure}[htb]  
  \centering
  \includegraphics[width=\textwidth]{Fig_ED1.pdf}
  \caption {\small
  {\bf{Two-dimensional mass distributions for  selected $\Dz\Dz\pip$, 
  $\Dz\Dz$ and $\Dz\Dp$~combinations.}}
  %%
  Two\protect\nobreakdash-dimensional mass distributions 
  for $\Dz$ and $\Dp$~candidates
  from selected (a)~$\Dz\Dz\pip$, 
  (b)~$\Dz\Dz$ and (c)~$\Dz\Dp$~combinations.
  $\kaon_{1/2}$ and $\pion_{1/2}$ correspond 
  to daughters of the~first/second \Dz candidate 
  in $\Dz\Dz$ and $\Dz\Dz\pip$ final states.
  }
  \label{fig:DATA_2D}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth]{Fig_ED2.pdf}
  \caption { \small
    {\bf Mass distributions for $\Dz\Dz\pip$~combinations 
with fake \Dz~candidates.}
  Mass distributions for $\Dz\Dz\pip$~combinations 
with (a)~one true and one fake \Dz~candidate, 
(b)~two fake $\Dz$~candidates
and (c)~at least one fake $\Dz$~candidate.
Results of the~fits with 
background\protect\nobreakdash-only
functions are overlaid.
  }
  \label{fig:SIDEBANDS}
\end{figure}



\begin{figure}[htb]
  %%
  \centering
  \includegraphics[width=\textwidth]{Fig_ED3.pdf}
  \caption {\small
  {\bf{Mass distributions for \Dz\Dz\pip and \Dz\Dzb\pim~candidates.}}
  %%
   Background\protect\nobreakdash-subtracted 
  \Dz\Dz\pip and \Dz\Dzb\pim~mass distributions.
  }
  \label{fig:D0D0piOS}
\end{figure}






\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth]{Fig_ED4.pdf}
  \caption {\small
   {\bf{Mass distributions for \Dz\Dp and \Dz\Dm~candidates.}}
   %%
   Background\protect\nobreakdash-subtracted 
  \Dz\Dp and \Dz\Dm~mass distributions.
  }
  \label{fig:D0DpOS}
\end{figure}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth]{Fig_ED5.pdf}
  \caption { \small
   {\bf{Three\protect\nobreakdash-body phase\protect\nobreakdash-space functions  
   $\varrho_f(s)$.}}
  %%
   Three\protect\nobreakdash-body phase\protect\nobreakdash-space functions  
   $\varrho_f(s)$ with (left) linear and (right) logarithmic 
   vertical-axis scale:
   (red)~\mbox{$\decay{\Tcc}{\Dz\Dz\pip }$},
   (blue)~\mbox{$\decay{\Tcc}{\Dp\Dz\piz}$} and 
   (green)~\mbox{$\decay{\Tcc}{\Dp\Dz\g}$}.
   The~sum, $\varrho_{\mathrm{tot}}(s)$,  
   is shown with a~black line. 
   The~two\protect\nobreakdash-body $\Dstar\D$~phase-space shapes 
   are shown by the~dashed lines and are different 
   from the~$\varrho_f(s)$~functions only 
   in the~vicinity 
   of the~thresholds or below them. 
   Vertical dash-dotted line indicates 
   $\sqrt{s^*}=3.9\gev$.
  }
  \label{fig:RHOS}
\end{figure}

\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth]{Fig_ED6.pdf}
  \caption { \small
  {\bf{Function $\xi(s)$.}} 
  %% 
  Function $\xi(s)$ 
  with (left) linear and (right) logarithmic vertical-axis scale
  is shown with 
  a~red line.
  The~three\protect\nobreakdash-body phase-space function
   $\varrho_{\mathrm{tot}}(s)$ 
   is shown for comparison with a~dashed line. 
  }
  \label{fig:xi}
\end{figure}

\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth]{Fig_ED7.pdf}
  \caption { \small
  {\bf{Scaling behaviour of the~$\mathfrak{F}^{\mathrm{U}}$~profile.}}
  %%
  %% Scaling behaviour of the~$\mathfrak{F}^{\mathrm{U}}$~profile.
  The~full width at half maximum $\mathfrak{w}$ as a~function
  of the~$\left|g\right|$~parameter for
  a~fixed value of the~$\updelta m_{\mathrm{U}}$~parameter
  \mbox{$\updelta m_{\mathrm{U}}=-359\kevcc$}.
  The~horizontal dashed blue line indicates 
  the~value of $\mathfrak{w}$ corresponding 
  to the~best fit parameters.
  }
  \label{fig:SCALING}
\end{figure}

\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth]{Fig_ED8.pdf}
  \caption { \small
  {\bf{Unitarised three-body Breit\protect\nobreakdash--Wigner 
  function %% $\mathfrak{F}^{\mathrm{U}}_{\decay{\Tcc}{\Dz\Dz\pip}}$.}}
  $\mathfrak{F}^{\mathrm{U}}$.}}
  %%
  Unitarised three\protect\nobreakdash-body Breit\protect\nobreakdash--Wigner 
  function $\mathfrak{F}^{\mathrm{U}}$ for 
  ${\decay{\Tcc}{\Dz\Dz\pip}}$~decays\,(red line)
  for a~large value of the~$\left|g\right|$~parameter
  and $\updelta m_{\mathrm{U}}=-359\kevcc$,
  normalized to unity for $\updelta m_{\Dz\Dz\pip}=\updelta m_{\mathrm{U}}$.
  Top inset shows a~zoomed region with 
  overlaid (blue dashed line)
  {\em{single\protect\nobreakdash-pole}} profile 
  with $\sqrt{\hat{s}}=\mathfrak{m}-\tfrac{i}{2}\mathfrak{w}$,
  and (thin green line)~three\protect\nobreakdash-body Breit\protect\nobreakdash--Wigner
  profile with $\left|g\right|=5.1\gev$.
  %%
  Bottom inset shows the~$\mathfrak{F}^{\mathrm{U}}$~profile 
  in log-scale. Vertical dashed lines indicate 
  (left\protect\nobreakdash-to\protect\nobreakdash-right) 
  $\Dstarp\Dz$ and $\Dstarz\Dp$~mass thresholds. 
  }
  \label{fig:BWU_shape}
\end{figure}




\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth]{Fig_ED9.pdf}
  \caption { \small
  {\bf{Comparison of the~$\mathcal{A}_{\mathrm{U}}$
   and $\mathcal{A}_{\mathrm{NR}}$~amplitudes.}} 
  The~real and imaginary
  parts of the inverse $\mathcal{A}_{\mathrm{U}}$
   and $\mathcal{A}_{\mathrm{NR}}$~amplitudes.
   The yellow band correspond to the~pole position
   and vertical dashed lines show the
   $\Dstarp\Dz$ and $\Dstarz\Dp$~mass thresholds.
  }
  \label{fig:MATCHING}
\end{figure}



\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth]{Fig_ED10.pdf}
  \caption { \small
  {\bf{Two-dimensional $\Dz\pip$ mass distribution.}}
  %%
  Background\protect\nobreakdash-sub\-tracted 
  two\protect\nobreakdash-dimensional $\Dz\pip$ mass distribution
  %{\em{Dalitz-like}} plot 
  for the~$\Dz\Dz\pip$~events with $\updelta m_{\Dz\Dz\pip}\le0$. 
  Dashed vertical and horizontal lines indicate the~known $\Dstarp$~mass.
  Red and dashed blue lines show  the~boundary 
  %of the Dalitz plot 
  corresponding to 
  \mbox{$\updelta m_{\Dz\Dz\pip}=0$}
  and \mbox{$\updelta m_{\Dz\Dz\pip}=-359\kevcc$}, respectively.
  }
  \label{fig:DALITZ}
\end{figure}


==> letter.tex <==
%% \section{Introduction}


Quantum chromodynamics\,(QCD), 
the~theory of the~strong force, 
describes 
interactions of coloured quarks and gluons
and the~formation of hadronic matter, 
the~so-called mesons and baryons. 
%%
While QCD makes precise 
predictions at high energies, 
the theory has difficulties
describing 
the~interactions of  quarks
in hadrons 
from first principles 
%% 
due to the~highly 
non\nobreakdash-perturbative 
regime at the~corresponding energy scale.
Hence, the~field of hadron spectroscopy is
driven by
experimental discoveries
that sometimes are unexpected, 
which could lead to changes 
in the~research landscape. 
%% 
Along with 
conventional mesons and baryons, 
made of 
a~quark-antiquark 
pair\,(\mbox{$\quark_1\quarkbar_2$})
and  three 
quarks\,(\mbox{$\quark_1\quark_2\quark_3$}),
respectively, 
particles with 
an~alternative quark content,
%% 
known as exotic states, 
have been actively discussed 
since the~birth of the~constituent quark 
model~\cite{GellMann:1964nj,
Zweig:352337,Zweig:570209, 
Jaffe:1976ig,
Jaffe:1976ih,
Rossi:1977cy,
Jaffe:1977cv, 
Lipkin:1987sk}.
%%
The~discussion has been revived 
by recent observations of 
numerous 
tetraquark $\quark_1\quark_2\quarkbar_3\quarkbar_4$ 
and pentaquark 
$\quark_1\quark_2\quark_3\quark_4\quarkbar_5$ 
candidates~\cite{
%% Brambilla:2019esw,
%% PDG2021}.
%% \cite{
Choi:2003ue,
 Choi:2007wga,
 Belle:2008qeq,
  Aaltonen:2009tz,
 Belle:2011aa, 
  Ablikim:2013mio,
  BESIII:2013ouc,
  BESIII:2013mhi,
  Abazov:2013xda,
  Chatrchyan:2013dma,
   Chilikin:2013tch,
   Belle:2013yex, %% ADDED! 
   Chilikin:2014bkk, 
  LHCb-PAPER-2014-014,
   LHCb-PAPER-2015-029, 
  LHCb-PAPER-2015-038,
  %%
  LHCb-PAPER-2016-018, 
  LHCb-PAPER-2016-019, 
  LHCb-PAPER-2018-034,
  LHCb-PAPER-2019-014,
  %% 
  LHCb-PAPER-2020-011, 
  LHCb-PAPER-2020-024,
  LHCb-PAPER-2020-025, 
  % 
  LHCb-PAPER-2020-035,
  LHCb-PAPER-2020-039,
  LHCb-PAPER-2020-044,
   %% 
   Ablikim_2021,
% LHCb-PAPER-2019-009
  LHCb-PAPER-2021-018}. %% IN PREPARATION!!! 
%%
Due~to the~closeness of their masses 
to known particle\nobreakdash-pair 
thresholds~\cite{
Brambilla:2019esw,
PDG2021}, 
many of these 
states are likely to be 
%% predominantly 
hadronic molecules~\cite{Oset:2019upy,
Richard_2016,Guo:2017jvc, 
MartinezTorres:2020hus}
where colour\nobreakdash-singlet hadrons are bound by 
%% {\color{red}
 residual nuclear forces
similar to the~electromagnetic 
%% van\nobreakdash-der\nobreakdash-Waals 
van der Waals 
forces attracting 
electrically neutral atoms and molecules.
An~ordinary 
example of 
a~hadronic molecule is the~deuteron 
formed by a~proton and a~neutron.
%%
On~the~other hand, an~interpretation of exotic states
as compact multiquark structures 
is also possible~\cite{Ali:2019roi}.

All exotic hadrons observed so far 
%% {\color{red}{
predominantly
%% }} 
decay via 
the~strong interaction and 
their decay widths vary from a~few to a~few hundred~\mev.
A~discovery of a~long\nobreakdash-lived exotic 
state, stable 
with respect to the~strong interaction,
would be intriguing.
% 
A~hadron with two heavy quarks~$\PQ$ and 
two light antiquarks~$\quarkbar$, \ie
\mbox{$\PQ_1\PQ_2\quarkbar_1\quarkbar_2$}, 
is a~prime candidate to form such 
a~state~\cite{Ader:1981db,
Ballot:1983iv,
Zouzou:1986qh,
Lipkin:1986dw,
Heller:1986bt,
Manohar:1992nd}.
In~the~limit of a~large heavy-quark mass
%% ,$m_{\PQ}\to+\infty$,
the~two heavy 
quarks $\PQ_1\PQ_2$ form a~point\nobreakdash-like 
heavy colour\nobreakdash-antitriplet object,
%% \ie  analogous to an~antiquark, 
that behaves similarly to an~antiquark,  
and the~corresponding state should be bound.
%% 
It is expected that the~$\bquark$ quark 
is heavy enough to sustain
%% 
the~existence of a~stable 
\mbox{$\bquark\bquark\uquarkbar\dquarkbar$}~state 
with its binding energy of
%% about $215\mev$~\cite{Karliner:2017qjm} 
about $200\mev$
with
respect to 
% {\color{red} % threshold % given by the
the~sum of masses of the~pseudoscalar, 
%% {\color{red}{
$\Bm$ or $\Bzb$,
%% }}   
and vector, 
%% {\color{red}{
$\B^{*-}$ or $\Bbar{}^{*0}$,
%% }}
beauty mesons
that defines the~minimal mass 
for the~strong decay to be allowed.
% }
% a~sum of masses of the~\B and $\B^*$~mesons.
%%
%% 
In~the~case of 
the~\mbox{$\bquark\cquark\uquarkbar\dquarkbar$}
and~\mbox{$\cquark\cquark\uquarkbar\dquarkbar$}~systems,
there is currently 
no consensus  as to 
whether such states exist and are narrow 
enough to be detected experimentally.
%%
The~similarity of 
the~\cquark\cquark\uquarkbar\dquarkbar~tetraquark state 
and the~\Xiccpp~baryon
containing two \cquark~quarks 
and a~\uquark~quark, 
leads to a~relationship between 
the~properties of the~two states.
In~particular, the~measured mass of 
the~\Xiccpp~baryon
with quark content $\cquark\cquark\uquark$~\cite{
LHCb-PAPER-2017-018,
LHCb-PAPER-2018-026,
LHCb-PAPER-2019-037}
% is translated into the conclusion that
implies that the~mass 
of the~$\cquark\cquark\uquarkbar\dquarkbar$
tetraquark is close to the
%% to the~$\Dstarp\Dz$~mass threshold
sum of masses of \Dz and \Dstarp~mesons 
with quark content of 
$\cquark\uquarkbar$ and $\cquark\dquarkbar$,
respectively, 
as suggested in Ref.~\cite{Karliner:2017qjm}.
%%
Theoretical predictions for 
the~mass of  
the~$\mbox{\cquark\cquark\uquarkbar\dquarkbar}$~ground~state
with 
spin\nobreakdash-parity quantum 
numbers $\mathrm{J^P=1^+}$ and 
isospin $\mathrm{I}=0$,
denoted hereafter as \Tcc, 
relative to the~$\Dstarp\Dz$~mass threshold
%%
\ifthenelse{\boolean{wordcount}}{}{%%
\begin{equation}\label{eq:delta_prime}
 \updelta m  \equiv 
 m_{\Tcc} - \left( m_{\Dstarp} + m_{\Dz}\right) \,,
\end{equation}%%
}
%%
lie in the~range 
\mbox{$-300< \updelta m < 300\mevcc$}~\cite{
Carlson:1987hh,
SilvestreBrac:1993ss,
Semay:1994ht,
Moinester:1995fk,
Pepin:1996id,
GELMAN2003296,
Vijande:2003ki,
Janc:2004qn,
Navarra:2007yw,
Vijande,
Ebert:2007rn,
Lee:2009rt,
Yang2009,
Li:2012ss,
Feng:2013kea,
Luo:2017eub,
Karliner:2017qjm,
Eichten:2017ffp,
Wang:2017uld,
Park:2018wjk,
Junnarkar:2018twb,
Deng:2018kly,
Liu:2019stu,
Maiani:2019lpu,
Yang:2019itm,
Tan:2020ldi,
Lu:2020rog,
Braaten:2020nwp,
Gao:2020ogo,
Cheng:2020wxa,
Noh:2021lqs,
Faustov:2021hjs},
where $m_{\Dstarp}$ and $m_{\Dz}$ denote 
the~known masses of the~$\Dstarp$ and $\Dz$~mesons~\cite{PDG2021}.
Lattice QCD calculations also do not provide 
a~definite conclusion on the~existence 
of the~\Tcc~state 
and its~binding energy~\cite{
Ikeda:2013vwa,
Cheung:2017tnt,
Francis:2018jyb,
Junnarkar:2018twb}.
%%
The~observation of 
the~$\Xiccpp$ baryon~\cite{LHCb-PAPER-2017-018,
LHCb-PAPER-2018-026}
and of a~new exotic resonance decaying to
a~pair of \jpsi~mesons~\cite{LHCb-PAPER-2020-011}
by the \lhcb experiment,
% ,
%at \lhcb 
motivates the~search for the~\Tcc state.
% 

In this Letter, the~observation of a~narrow state 
in the~\Dz\Dz\pip~mass 
spectrum %% \footnote{Throughout this Letter, 
%% charge conjugate decays are implied.} 
near the $\Dstarp\Dz$~mass threshold 
compatible with 
being a~$\Tcc$~tetraquark state is reported.
%%
Throughout this Letter, 
charge conjugate decays are implied.
%w
The~study is based on 
proton\nobreakdash-proton\,($\proton\proton$) 
collision  data collected
with the~LHCb detector 
at the~Large Hadron Collider\,(LHC)
at CERN 
at centre\nobreakdash-of\nobreakdash-mass 
energies of~7,~8 and~13\tev, 
corresponding to integrated
luminosity of~9\invfb. 
%%
The~LHCb detector~\cite{LHCb-DP-2008-001,LHCb-DP-2014-002} 
is a~single-arm forward spectrometer covering 
the~pseudorapidity
%% \footnote{
%% %% {\color{red}{
%% Pseudorapidity $\eta$ is defined 
%% as $-\log \left( \tan \tfrac{\theta}{2}\right) $,
%% where $\theta$~is a~polar angle of the track relative to the 
%% proton beam line.
%% %%}}
%% }
range \mbox{$2 < \eta < 5$}, 
designed for the~study of 
particles containing 
\bquark\ or \cquark\ quarks and
is further described in Methods.
%% 
Pseudorapidity $\eta$ is defined 
as $-\log \left( \tan \tfrac{\theta}{2}\right) $,
where $\theta$~is a~polar angle of the track relative to
the~proton beam line.
%% 


%% Marco's variant
The~$\Dz\Dz\pip$ final state is reconstructed by 
selecting events with two \Dz~mesons and 
a~positively charged pion all produced 
at the~same $\proton\proton$ 
interaction point.
%% 
Both~\Dz~mesons are reconstructed 
in the~$\Dz\to\Km\pip$~decay channel. 
%% To~subtract non\nobreakdash–\Dz background, 
The~selection criteria are similar to those 
used in Ref.~\cite{LHCb-PAPER-2012-003}.
% 
To~subtract background not originating 
from two \Dz~candidates
an~extended unbinned 
maximum\nobreakdash-likelihood fit to 
the~two\nobreakdash-dimensional distribution of
the~masses of the~two \Dz~candidates 
is performed. 
%% {\color{red}
The corresponding procedure, 
together with the~selection criteria, is described in detail in Methods.
%% }%
To~improve the~$\updelta m$  mass resolution and to make
the~determination insensitive 
to the~precision of the~\Dz~meson mass, 
the~mass of the~$\Dz\Dz\pip$~combinations is
calculated with the~mass of each $\Dz$~meson
constrained to the~known value~\cite{PDG2021}.
%% Fits 
%
The~resulting 
$\Dz\Dz\pip$~mass distribution 
for~selected $\Dz\Dz\pip$~combinations
is shown in Fig.~\ref{fig:DATA_BW0_fit}.
A~narrow peak near 
the~$\Dstarp\Dz$~mass threshold is clearly visible. 
%%


An~extended unbinned maximum\nobreakdash-likelihood 
fit to the~$\Dz\Dz\pip$~mass
distribution is performed using 
a~model consisting of signal and background components.
%%
The~signal component
is described by the~convolution of 
the~detector resolution with 
a~resonant shape,
which is modelled by 
a~relativistic P\nobreakdash-wave 
two\nobreakdash-body Breit\nobreakdash--Wigner function 
modified by a~\mbox{Blatt}\nobreakdash--Weisskopf 
form factor %% ~\cite{Blatt:1952ije}  %% ,VonHippel:1972fg}
with a~meson\nobreakdash-radius parameter of $3.5\gev^{-1}$. 
The~use of 
a~P\nobreakdash--wave resonance 
is motivated by 
the~expected $\mathrm{J^P}=1^+$ quantum 
numbers for the~\Tcc~state.
%%  
A~two\nobreakdash-body decay 
structure \mbox{$\decay{\Tcc}{\PA\PB}$} 
is assumed with $m_{\PA}=2m_{\Dz}$  and $m_{\PB}=m_{\pip}$,
where $m_{\pip}$~stands for 
the~known mass of the~\pip~meson.
Several alternative prescriptions are used for evaluation
of systematic uncertainties.
Despite its simplicity, 
the~model serves well to quantify 
the~existence of the~$\Tcc$ state and to measure 
its  properties, 
such as the~position and the~width
of the~resonance.
A~follow\nobreakdash-up study~\cite{LHCb-PAPER-2021-032}
investigates the~underlying nature of 
the~\Tcc~state,
expanding on 
the~modelling of the~signal shape
and determining its physical properties.
%%
The~detector resolution  
is modelled by the~sum 
of two Gaussian functions 
with a~common mean, 
where the~additional parameters are 
taken from simulation\,(see Methods) with 
corrections applied~\cite{LHCb-PAPER-2020-008,
LHCb-PAPER-2020-009,
LHCb-PAPER-2020-035}. 
The~root mean square of the~resolution 
function is around 400\kevcc. 
A~study of the~$\Dz\pip$~mass distribution 
for  $\Dz\Dz\pip$~combinations 
in the~region above the~$\Dstarz\Dp$~mass threshold 
and below $3.9\gevcc$ shows 
that  approximately $90\%$ of 
all random $\Dz\Dz\pip$~combinations 
contain a~genuine $\Dstarp$~meson.
Based on this observation, the~background component
is parametrised by the~product of  
a~two\nobreakdash-body phase space 
function %% ~\cite{Kallen} 
%% $\Phi_{\Dstarp\Dz}$~\cite{Kallen} 
and  a~positive second\nobreakdash-order polynomial. 
The~resulting function is convolved 
with the~detector resolution.
%%

The~fit results are shown in 
Fig.~\ref{fig:DATA_BW0_fit}, 
and the~parameters of interest, 
namely the~signal yield, $N$, 
the~mass parameter of the Breit\nobreakdash--Wigner
function relative to the~$\Dstarp\Dz$~mass threshold,  
\mbox{$\updelta m_{\mathrm{BW}}
\equiv m_{\mathrm{BW}}-(m_{\Dstarp}+m_{\Dz})$},
and the~width parameter, $\Gamma_{\mathrm{BW}}$,
are listed in Table~\ref{tab:DATA_BW0_fits}. 
%%
The~statistical significance of the~observed 
\mbox{$\decay{\Tcc}{\Dz\Dz\pip}$}~signal is estimated 
using Wilks' theorem %% ~\cite{Wilks:1938dza} 
to be $22$~standard deviations.
%%
The~fit suggests that~the~mass parameter of 
the~Breit\nobreakdash--Wigner shape  
is slightly below 
the~$\Dstarp\Dz$~mass threshold. 
The~statistical significance
of the~hypothesis $\updelta m_{\mathrm{BW}}<0$ is 
estimated to be 4.3~standard deviations.
%%

\begin{figure}[t]
  \includegraphics[width=\textwidth]{Fig1.pdf}
  \caption { \small
 {\bf Distribution of \Dz\Dz\pip~mass}.
 Distribution of \Dz\Dz\pip~mass where 
 the~contribution of the~non\protect\nobreakdash-$\Dz$ 
 background has been statistically subtracted.
 The~result of the~fit 
 with the~two\nobreakdash-component function 
 described in the~text is overlaid.
 %%
 The~$\Dstarp\Dz$ and $\Dstarz\Dp$~thresholds 
 are indicated with the~vertical dashed lines. 
 %%
 The~horizontal bin width is indicated on 
 the~vertical axis legend.
 %%
 Inset shows a~zoomed signal region
 with fine binning scheme,  
 %% 
 %%{\color{red}{
 Uncertainties on the~data points are statistical
 only and represent one standard deviation, 
 calculated as a~sum in quadrature of the~assigned weights from 
 the~background\protect\nobreakdash-subtraction procedure.
 %%}}
 }
  \label{fig:DATA_BW0_fit}
\end{figure}

\begin{table}[bt]
	\centering
	\caption{\small
        %%
        Parameters obtained
	obtained from the~fit to the~$\Dz\Dz\pip$~mass spectrum.
        %%
	Signal yield, $N$, 
	Breit\protect\nobreakdash--Wigner 
	mass relative to 
	$\Dstarp\Dz$~mass threshold, 
	$\updelta m_{\mathrm{BW}}$,
	and width, $\Gamma_{\mathrm{BW}}$,
        are listed.
	%~parameters
	%% obtained from the~fit to the~\Dz\Dz\pip~mass spectrum.
	%%  
	The~uncertainties are statistical only. 
	}
	\label{tab:DATA_BW0_fits}
	\vspace{2mm}
	\begin{tabular*}{0.40\textwidth}
	{@{\hspace{3mm}}l@{\extracolsep{\fill}}l@{\hspace{3mm}}}
	Parameter  & ~~~~Value 
   \\[1mm]
  \hline 
  \\[-2mm]
  %%
   $N$            & $\phantom{-}117\pm16\phantom{0}$ 
   \\     
   $\updelta m_{\mathrm{BW}}$   
 %% &  $-278\pm61\phantom{0}\kevcc$   
   &  $-273\pm61\phantom{0}\kevcc$   
   \\
   $\Gamma_{\mathrm{BW}}$ 
    & $\phantom{-}410\pm165\kev$ 

	\end{tabular*}
	\vspace{3mm}
\end{table}




%%
%% Cross-checks 
%% 
To~validate the~presence of the~signal component, 
several additional cross\nobreakdash-checks are
performed.
The~data are categorised according 
to data\nobreakdash-taking 
periods including the~polarity of the~LHCb
dipole magnet and the~charge 
of the~\Tcc~candidates.
%%
%%In~addition,
% 
Instead of statistically subtracting
the~non\nobreakdash-\Dz~background,
the~mass of 
each \mbox{$\decay{\Dz}{\Km\pip}$}~candidate 
is required to be within a narrow~region around 
the~known mass of the~\Dz~meson~\cite{PDG2021}.
%%
The~results are found to be consistent
among all samples and analysis techniques.
%
Furthermore, dedicated studies are performed 
to ensure that the observed signal  is not caused by
kaon or pion misidentification, 
doubly Cabibbo\nobreakdash-suppressed 
\mbox{$\decay{\Dz}{\Kp\pim}$}~decays
and $\Dz\Dzb$~oscillations,
decays of charm hadrons originating 
from beauty hadrons, 
or artefacts due to the~track reconstruction
creating duplicate tracks.

%% 
%% Systematic uncertainties 
%% 
Systematic uncertainties 
for the~$\updelta m_{\mathrm{BW}}$
and 
$\Gamma_{\mathrm{BW}}$~parameters 
are summarised in Table~\ref{tab:systematic}
and described below. %
%%
The~largest systematic uncertainty 
is related to the~fit model 
and is studied using pseudoexperiments 
with alternative parametrisations 
of the~\Dz\Dz\pip~mass shape.
%%
Several
variations in 
the~fit model are considered: 
changes in the~signal model due 
to the~imperfect knowledge of the~detector resolution, 
an~uncertainty in 
the~correction factor for 
the~resolution 
taken from control channels,
parametrisation of the~background component
and the~additional model parameters 
of the~Breit\nobreakdash--Wigner function.
%
The~model uncertainty related to 
the~assumption of $\mathrm{J^P}=1^+$~quantum 
numbers of the~state 
is estimated and listed separately.
%%
The~results are affected 
by the~overall detector momentum scale, 
which is known to 
a~relative precision of 
$\updelta\upalpha=
3\times10^{-4}$~\cite{LHCb-PAPER-2013-011}. 
The corresponding uncertainty is 
estimated using simulated samples where 
the~momentum-scale is modified by 
factors of $\left(1\pm\updelta\upalpha\right)$.
 %%
In~the reconstruction, 
the~momenta of charged tracks 
are corrected for energy loss 
in the~detector material,  
the amount of which is known 
with a~relative uncertainty
of 10. %% \%~\cite{LHCb-PAPER-2010-001}. 
The~resulting uncertainty 
is assessed by varying 
the~energy loss correction 
by $\pm10\%$.
%%
As the~mass of the~$\Dz\Dz\pip$~combinations is 
calculated with the mass of each $\Dz$~meson 
constrained to the~known value of the~\Dz~mass,
the~$\updelta m_{\mathrm{BW}}$~parameter
is insensitive to the~precision of the~\Dz~mass.
% 
However, the~small uncertainty of 2\kevcc for
the $\Dstarp-\Dz$~mass difference~\cite{PDG2021}
%% ~\cite{Lees:2013zna,
%% Anastassov:2001cw,PDG2021}
directly affects 
the~$\updelta m_{\mathrm{BW}}$~value.
The~corresponding systematic uncertainty is added.


\ifthenelse{\boolean{wordcount}}{}{
\begin{table}[tb]
	\centering
	\caption{\small 
	Systematic uncertainties for 
	the~$\updelta m_{\mathrm{BW}}$ 
	and $\Gamma_{\mathrm{BW}}$~parameters.  
	The~total uncertainty is calculated 
	as the~sum in quadrature of all components 
	except for those related to 
	the~$\mathrm{J^P}$~quantum numbers
	assignment, which are handled separately. 
	}
	\label{tab:systematic}
	\vspace{2mm}
	\begin{tabular*}{0.75\textwidth}{@{\hspace{3mm}}l@{\extracolsep{\fill}}cc@{\hspace{3mm}}}
	%% \multirow{2}{*}{Source}
	Source 
    %% & $\upsigma_{\updelta m_{\mathrm{BW}}}$
    %% & $\upsigma_{\Gamma_{\mathrm{BW}}}$
    & $\upsigma_{\updelta
    m_{\mathrm{BW}}}~\left[\!\kevcc\right]$
    & $\upsigma_{\Gamma_{\mathrm{BW}}}~\left[\!\kev\right]$
    %%\\
    %%  & $\left[\!\kevcc\right]$
    %%  & $\left[\!\kev\right]$
   \\[1.5mm]
  \hline 
  \\[-2mm]
  %% 
  Fit model                         &             &     \\
  ~~Resolution model                & 2   &  \phantom{0}7 \\
  ~~Resolution correction factor    & 1   &  30 \\
  ~~Background model                & 3   &  30 \\ 
  ~~Model parameters                & $<1\phantom{0}\,\,$ & $<1\phantom{0}$ \\ 
  Momentum scale                 &  3 &  ---   \\
  Energy loss corrections        &  1 &  ---  \\
  $\Dstarp-\Dz$ mass difference &  2 & --- 
  \\[1.5mm]
  \hline 
  \\[-2mm]
  Total  & 5 & 43
  \\[1.5mm]
  \hline
  \\[-2mm]
  $\mathrm{J^P}$~quantum numbers     & ${}^{+11}_{-14}$ & ${}^{+18}_{-38}$
   \end{tabular*}
	\vspace{3mm}
\end{table}
}
%%


In summary,  using the~full
dataset corresponding to an~integrated 
luminosity 
of $9\invfb$,
collected by the~\lhcb experiment 
at centre-of-mass energies of 7, 8 and~13\tev
%during the~2011\nobreakdash--2018 period
, 
a~narrow peak is observed 
in the~mass spectrum of $\Dz\Dz\pip$~candidates 
produced promptly in $\proton\proton$~collisions.
%%
The~statistical significance of the peak 
is overwhelming. 
%%
Using the~Breit\nobreakdash--Wigner 
parametrisation, 
the~location of the peak 
relative to the~$\Dstarp\Dz$~mass threshold,
$\updelta m_{\mathrm{BW}}$,
and the~width, $\Gamma_{\mathrm{BW}}$, 
are determined to be 
\ifthenelse{\boolean{wordcount}}{}{
\begin{eqnarray*}
\updelta m_{\mathrm{BW}} 
& = &  
-273\pm \phantom{0}61 
\pm \phantom{0}5\,  {}^{\,+\,11}_{\,-\,14} \kevcc \,,
\\
\Gamma_{\mathrm{BW}} 
& = & 
\phantom{-} 410 \pm 165 \pm  43\,   {}^{\,+\,18}_{\,-\,38}\kev\,,
\end{eqnarray*}
}
where the~first uncertainty is statistical, 
the~second systematic 
and the~third is related 
to the~$\mathrm{J^P}$~quantum numbers  assignment.
The~measured $\updelta m_{\mathrm{BW}}$  
value corresponds 
to a~mass of approximately 3875\mev.
%%
This~is the~narrowest exotic state 
observed to date~\cite{Brambilla:2019esw,
PDG2021}.
%% 
The~minimal quark content 
for this
%% newly
%% observed
state is $\cquark\cquark\uquarkbar\dquarkbar$.
Two~heavy quarks of the~same 
flavour make it manifestly exotic, 
\ie beyond the conventional pattern
of hadron formation found in mesons and baryons.
%%
%% representing a~novel class of hadronic matter formation. 
%%
Moreover, 
a~combination of the~near\nobreakdash-threshold mass,
narrow decay width and 
its appearance in prompt hadroproduction
demonstrates its genuine resonance nature.
%% This is the first such exotic resonance ever 
%% observed.
%%
The~measured mass and width are consistent with 
the~expected values for a~\Tcc~isoscalar 
tetraquark ground state with 
quantum numbers $\mathrm{J}^{\mathrm{P}}=1^+$. %
%% 
The~precision of the~mass measurement 
with respect to the~corresponding threshold 
is superior to those of all other exotic states, 
which will give better understanding of 
the~nature of exotic states. %
%% 
A~dedicated study of the~reaction amplitudes
for the~\mbox{$\decay{\Tcc}{\Dz\Dz\pip}$} and
\mbox{$\decay{\Tcc}{\Dz\Dp\piz(\g)}$}~decays
that uses the~isospin 
symmetry for~the~\mbox{$\decay{\Tcc}{\Dstar\D}$}
transition~\cite{LHCb-PAPER-2021-032}
yields insights on
the~fundamental resonance properties, 
like the~pole position, 
the scattering length and the~effective range.
%% 
The~observation of 
this $\cquark\cquark\uquarkbar\dquarkbar$~tetraquark 
candidate 
close to the~$\Dstarp\Dz$ threshold 
%%
%% {\color{red}{
provides~strong support 
for the~theory approaches and models 
that predict 
%%
%% further supports 
the~existence 
of a~$\bquark\bquark\uquarkbar\dquarkbar$~tetraquark 
%% that is 
stable with respect to the~strong and 
electromagnetic interactions.
%% }}
% 


==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script python listsymbols.py

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash belletwo} & \belletwo & \texttt{\textbackslash besiii} & \besiii & \texttt{\textbackslash cleo} & \cleo \\
\texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero & \texttt{\textbackslash aleph} & \aleph \\
\texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal & \texttt{\textbackslash lthree} & \lthree \\
\texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern & \texttt{\textbackslash lhc} & \lhc \\
\texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron & \texttt{\textbackslash bfactories} & \bfactories \\
\texttt{\textbackslash bfactory} & \bfactory & \texttt{\textbackslash upgradeone} & \upgradeone & \texttt{\textbackslash upgradetwo} & \upgradetwo \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash emp} & \emp & \texttt{\textbackslash epem} & \epem \\
\texttt{\textbackslash muon} & \muon & \texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun \\
\texttt{\textbackslash mupm} & \mupm & \texttt{\textbackslash mump} & \mump & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash taupm} & \taupm & \texttt{\textbackslash taump} & \taump & \texttt{\textbackslash tautau} & \tautau \\
\texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm & \texttt{\textbackslash ellp} & \ellp \\
\texttt{\textbackslash ellpm} & \ellpm & \texttt{\textbackslash ellmp} & \ellmp & \texttt{\textbackslash ellell} & \ellell \\
\texttt{\textbackslash neu} & \neu & \texttt{\textbackslash neub} & \neub & \texttt{\textbackslash neue} & \neue \\
\texttt{\textbackslash neueb} & \neueb & \texttt{\textbackslash neum} & \neum & \texttt{\textbackslash neumb} & \neumb \\
\texttt{\textbackslash neut} & \neut & \texttt{\textbackslash neutb} & \neutb & \texttt{\textbackslash neul} & \neul \\
\texttt{\textbackslash neulb} & \neulb &  \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim & \texttt{\textbackslash pipm} & \pipm \\
\texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson & \texttt{\textbackslash rhoz} & \rhoz \\
\texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom & \texttt{\textbackslash rhopm} & \rhopm \\
\texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon & \texttt{\textbackslash Kbar} & \Kbar \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash Vzero} & \Vzero & \texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz \\
\texttt{\textbackslash Kstarzb} & \Kstarzb & \texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb \\
\texttt{\textbackslash Kstarp} & \Kstarp & \texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm \\
\texttt{\textbackslash Kstarmp} & \Kstarmp & \texttt{\textbackslash KorKbarz} & \KorKbarz & \texttt{\textbackslash etaz} & \etaz \\
\texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz & \texttt{\textbackslash omegaz} & \omegaz \\
\end{tabular*}

\subsubsection{Charmed mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Dbar} & \Dbar & \texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db \\
\texttt{\textbackslash DorDbar} & \DorDbar & \texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb \\
\texttt{\textbackslash Dp} & \Dp & \texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm \\
\texttt{\textbackslash Dmp} & \Dmp & \texttt{\textbackslash DpDm} & \DpDm & \texttt{\textbackslash Dstar} & \Dstar \\
\texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz & \texttt{\textbackslash Dstarzb} & \Dstarzb \\
\texttt{\textbackslash theDstarz} & \theDstarz & \texttt{\textbackslash theDstarzb} & \theDstarzb & \texttt{\textbackslash Dstarp} & \Dstarp \\
\texttt{\textbackslash Dstarm} & \Dstarm & \texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp \\
\texttt{\textbackslash theDstarp} & \theDstarp & \texttt{\textbackslash theDstarm} & \theDstarm & \texttt{\textbackslash theDstarpm} & \theDstarpm \\
\texttt{\textbackslash theDstarmp} & \theDstarmp & \texttt{\textbackslash Ds} & \Ds & \texttt{\textbackslash Dsp} & \Dsp \\
\texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm & \texttt{\textbackslash Dsmp} & \Dsmp \\
\texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp & \texttt{\textbackslash Dssm} & \Dssm \\
\texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp & \texttt{\textbackslash DporDsp} & \DporDsp \\
\texttt{\textbackslash DmorDsm} & \DmorDsm & \texttt{\textbackslash DpmorDspm} & \DpmorDspm &  \\
\end{tabular*}

\subsubsection{Beauty mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash BdorBdbar} & \BdorBdbar \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb & \texttt{\textbackslash BsorBsbar} & \BsorBsbar \\
\texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp & \texttt{\textbackslash Bcm} & \Bcm \\
\texttt{\textbackslash Bcpm} & \Bcpm & \texttt{\textbackslash Bds} & \Bds & \texttt{\textbackslash Bdsb} & \Bdsb \\
\texttt{\textbackslash BdorBs} & \BdorBs & \texttt{\textbackslash BdorBsbar} & \BdorBsbar &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash psires} & \psires & \texttt{\textbackslash chic} & \chic \\
\texttt{\textbackslash chiczero} & \chiczero & \texttt{\textbackslash chicone} & \chicone & \texttt{\textbackslash chictwo} & \chictwo \\
\texttt{\textbackslash chicJ} & \chicJ & \texttt{\textbackslash Upsilonres} & \Upsilonres & \texttt{\textbackslash OneS} & \OneS \\
\texttt{\textbackslash TwoS} & \TwoS & \texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS \\
\texttt{\textbackslash FiveS} & \FiveS & \texttt{\textbackslash chib} & \chib & \texttt{\textbackslash chibzero} & \chibzero \\
\texttt{\textbackslash chibone} & \chibone & \texttt{\textbackslash chibtwo} & \chibtwo & \texttt{\textbackslash chibJ} & \chibJ \\
\texttt{\textbackslash theX} & \theX &  \\
\end{tabular*}

\subsubsection{Light Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Lz} & \Lz & \texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar \\
\texttt{\textbackslash Lambdares} & \Lambdares & \texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares \\
\texttt{\textbackslash Sigmaz} & \Sigmaz & \texttt{\textbackslash Sigmap} & \Sigmap & \texttt{\textbackslash Sigmam} & \Sigmam \\
\texttt{\textbackslash Sigmaresbar} & \Sigmaresbar & \texttt{\textbackslash Sigmabarz} & \Sigmabarz & \texttt{\textbackslash Sigmabarp} & \Sigmabarp \\
\texttt{\textbackslash Sigmabarm} & \Sigmabarm & \texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiz} & \Xiz \\
\texttt{\textbackslash Xim} & \Xim & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Xibarz} & \Xibarz \\
\texttt{\textbackslash Xibarp} & \Xibarp & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Omegam} & \Omegam & \texttt{\textbackslash Omegabarp} & \Omegabarp &  \\
\end{tabular*}

\subsubsection{Charmed Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lc} & \Lc & \texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Xic} & \Xic \\
\texttt{\textbackslash Xicz} & \Xicz & \texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar \\
\texttt{\textbackslash Xicbarz} & \Xicbarz & \texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac \\
\texttt{\textbackslash Omegacbar} & \Omegacbar & \texttt{\textbackslash Xicc} & \Xicc & \texttt{\textbackslash Xiccbar} & \Xiccbar \\
\texttt{\textbackslash Xiccp} & \Xiccp & \texttt{\textbackslash Xiccpp} & \Xiccpp & \texttt{\textbackslash Xiccbarm} & \Xiccbarm \\
\texttt{\textbackslash Xiccbarmm} & \Xiccbarmm & \texttt{\textbackslash Omegacc} & \Omegacc & \texttt{\textbackslash Omegaccbar} & \Omegaccbar \\
\texttt{\textbackslash Omegaccc} & \Omegaccc & \texttt{\textbackslash Omegacccbar} & \Omegacccbar &  \\
\end{tabular*}

\subsubsection{Beauty Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Sigmab} & \Sigmab \\
\texttt{\textbackslash Sigmabp} & \Sigmabp & \texttt{\textbackslash Sigmabz} & \Sigmabz & \texttt{\textbackslash Sigmabm} & \Sigmabm \\
\texttt{\textbackslash Sigmabpm} & \Sigmabpm & \texttt{\textbackslash Sigmabbar} & \Sigmabbar & \texttt{\textbackslash Sigmabbarp} & \Sigmabbarp \\
\texttt{\textbackslash Sigmabbarz} & \Sigmabbarz & \texttt{\textbackslash Sigmabbarm} & \Sigmabbarm & \texttt{\textbackslash Sigmabbarpm} & \Sigmabbarpm \\
\texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz & \texttt{\textbackslash Xibm} & \Xibm \\
\texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz & \texttt{\textbackslash Xibbarp} & \Xibbarp \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BR} & \BR & \texttt{\textbackslash BRvis} & \BRvis \\
\texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to &  \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, \boldmath \CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash T} & \T & \texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar \\
\texttt{\textbackslash Vud} & \Vud & \texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd \\
\texttt{\textbackslash Vus} & \Vus & \texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts \\
\texttt{\textbackslash Vub} & \Vub & \texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb \\
\texttt{\textbackslash Vuds} & \Vuds & \texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds \\
\texttt{\textbackslash Vuss} & \Vuss & \texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss \\
\texttt{\textbackslash Vubs} & \Vubs & \texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\texttt{\textbackslash Cpipi} & \Cpipi & \texttt{\textbackslash Spipi} & \Spipi & \texttt{\textbackslash CKK} & \CKK \\
\texttt{\textbackslash SKK} & \SKK & \texttt{\textbackslash ADGKK} & \ADGKK &  \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash Bsee} & \Bsee & \texttt{\textbackslash Bdee} & \Bdee \\
\texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk &  \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units (these macros add a small space in front)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}   } & \unit{kg}    &  \\
\end{tabular*}

\subsubsection{Energy and momentum }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevgev} & \gevgev \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevc} & \gevc & \texttt{\textbackslash mevcc} & \mevcc \\
\texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcc} & \gevgevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\end{tabular*}

\subsubsection{Distance and area (these macros add a small space)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst & \texttt{\textbackslash lumi} & \lumi \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqvs} & \chisqvs & \texttt{\textbackslash chisqvtx} & \chisqvtx \\
\texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv & \texttt{\textbackslash gsim} & \gsim \\
\texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} & \texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} \\
\texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag & \texttt{\textbackslash PDF} & \PDF \\
\texttt{\textbackslash sPlot} & \sPlot & \texttt{\textbackslash sFit} & \sFit &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash sqsnn} & \sqsnn \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash ptsq} & \ptsq & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt & \texttt{\textbackslash dpp} & \dpp \\
\texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx &  \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash murad} & \murad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig & \texttt{\textbackslash moore} & \moore \\
\texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos & \texttt{\textbackslash powheg} & \powheg \\
\texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos & \texttt{\textbackslash roofit} & \roofit \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice & \texttt{\textbackslash urania} & \urania \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn & \texttt{\textbackslash git} & \git & \texttt{\textbackslash latex} & \latex \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbit} & \kbit & \texttt{\textbackslash kbps} & \kbps & \texttt{\textbackslash kbytes} & \kbytes \\
\texttt{\textbackslash kbyps} & \kbyps & \texttt{\textbackslash mbit} & \mbit & \texttt{\textbackslash mbps} & \mbps \\
\texttt{\textbackslash mbytes} & \mbytes & \texttt{\textbackslash mbyps} & \mbyps & \texttt{\textbackslash gbit} & \gbit \\
\texttt{\textbackslash gbps} & \gbps & \texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbyps} & \gbyps \\
\texttt{\textbackslash tbit} & \tbit & \texttt{\textbackslash tbps} & \tbps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbyps} & \tbyps & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}

\subsubsection{Helpful to align numbers in tables}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash phz} & \phz &  \\
\end{tabular*}



==> refs.tex <==
\ifx\mcitethebibliography\mciteundefinedmacro
\PackageError{LHCb.bst}{mciteplus.sty has not been loaded}
{This bibstyle requires the use of the mciteplus package.}\fi
\providecommand{\href}[2]{#2}
\begin{mcitethebibliography}{100}
\mciteSetBstSublistMode{n}
\mciteSetBstMaxWidthForm{subitem}{\alph{mcitesubitemcount})}
\mciteSetBstSublistLabelBeginEnd{\mcitemaxwidthsubitemform\space}
{\relax}{\relax}

\bibitem{GellMann:1964nj}
M.~Gell-Mann, \ifthenelse{\boolean{articletitles}}{\emph{{A schematic model of
  baryons and mesons}},
  }{}\href{https://doi.org/10.1016/S0031-9163(64)92001-3}{Phys.\ Lett.\
  \textbf{8} (1964) 214}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Zweig:352337}
G.~Zweig, \ifthenelse{\boolean{articletitles}}{\emph{{An SU$_3$ model for
  strong interaction symmetry and its breaking; Version 1}}}{}
  \href{http://cds.cern.ch/record/352337}{CERN-TH-401}, CERN, Geneva,
  1964\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Zweig:570209}
G.~Zweig,  \ifthenelse{\boolean{articletitles}}{\emph{{An SU$_3$ model for
  strong interaction symmetry and its breaking; Version 2}}}{},
  \href{http://cds.cern.ch/record/570209}{\href{http://cds.cern.ch/record/570209}{CERN-TH-412}},
  CERN, 1964\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Jaffe:1976ig}
R.~L. Jaffe, \ifthenelse{\boolean{articletitles}}{\emph{{Multiquark hadrons. I.
  Phenomenology of $\PQ^2\bar{\PQ}^2$~mesons}},
  }{}\href{https://doi.org/10.1103/PhysRevD.15.267}{Phys.\ Rev.\  \textbf{D15}
  (1977) 267}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Jaffe:1976ih}
R.~L. Jaffe, \ifthenelse{\boolean{articletitles}}{\emph{{Multi-quark hadrons.
  2.~Methods}}, }{}\href{https://doi.org/10.1103/PhysRevD.15.281}{Phys.\ Rev.\
  \textbf{D15} (1977) 281}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Rossi:1977cy}
G.~C. Rossi and G.~Veneziano,
  \ifthenelse{\boolean{articletitles}}{\emph{{A~possible description of baryon
  dynamics in dual and gauge theories}},
  }{}\href{https://doi.org/10.1016/0550-3213(77)90178-X}{Nucl.\ Phys.\
  \textbf{B123} (1977) 507}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Jaffe:1977cv}
R.~L. Jaffe, \ifthenelse{\boolean{articletitles}}{\emph{{
  $\PQ^2\bar{\PQ}^2$~resonances in the~baryon\nobreakdash-antibaryon system}},
  }{}\href{https://doi.org/10.1103/PhysRevD.17.1444}{Phys.\ Rev.\  \textbf{D17}
  (1978) 1444}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lipkin:1987sk}
H.~J. Lipkin, \ifthenelse{\boolean{articletitles}}{\emph{{New~possibilities for
  exotic hadrons - anticharmed strange baryons}},
  }{}\href{https://doi.org/10.1016/0370-2693(87)90055-4}{Phys.\ Lett.\
  \textbf{B195} (1987) 484}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Choi:2003ue}
Belle collaboration, S.~K. Choi {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~narrow
  charmoniumlike state in exclusive
  \mbox{$\decay{\B^{\pm}}{\kaon^{\pm}\pip\pim\jpsi}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.91.262001}{Phys.\ Rev.\ Lett.\
  \textbf{91} (2003) 262001},
  \href{http://arxiv.org/abs/hep-ex/0309032}{{\normalfont\ttfamily
  arXiv:hep-ex/0309032}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{PDG2021}
Particle Data Group, P.~A. Zyla {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{\href{http://pdg.lbl.gov/}{Review
  of particle physics}}}, }{}\href{https://doi.org/10.1093/ptep/ptaa104}{Prog.\
  Theor.\ Exp.\ Phys.\  \textbf{2020} (2020) 083C01}, and
  {\href{http://pdglive.lbl.gov/}{2021 update}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Chen:2016qju}
H.-X. Chen, W.~Chen, X.~Liu, and S.-L. Zhu,
  \ifthenelse{\boolean{articletitles}}{\emph{{The hidden\nobreakdash-charm
  pentaquark and tetraquark states}},
  }{}\href{https://doi.org/10.1016/j.physrep.2016.05.004}{Phys.\ Rept.\
  \textbf{639} (2016) 1},
  \href{http://arxiv.org/abs/1601.02092}{{\normalfont\ttfamily
  arXiv:1601.02092}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Esposito:2016noz}
A.~Esposito, A.~Pilloni, and A.~D. Polosa,
  \ifthenelse{\boolean{articletitles}}{\emph{{Multiquark resonances}},
  }{}\href{https://doi.org/10.1016/j.physrep.2016.11.002}{Phys.\ Rept.\
  \textbf{668} (2017) 1},
  \href{http://arxiv.org/abs/1611.07920}{{\normalfont\ttfamily
  arXiv:1611.07920}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ali:2017jda}
A.~Ali, J.~S. Lange, and S.~Stone,
  \ifthenelse{\boolean{articletitles}}{\emph{{Exotics: Heavy pentaquarks and
  tetraquarks}}, }{}\href{https://doi.org/10.1016/j.ppnp.2017.08.003}{Prog.\
  Part.\ Nucl.\ Phys.\  \textbf{97} (2017) 123},
  \href{http://arxiv.org/abs/1706.00610}{{\normalfont\ttfamily
  arXiv:1706.00610}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Hosaka:2016pey}
A.~Hosaka {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Exotic
  hadrons with heavy flavors: \PX, \PY, \PZ, and related states}},
  }{}\href{https://doi.org/10.1093/ptep/ptw045}{PTEP \textbf{2016} (2016)
  062C01}, \href{http://arxiv.org/abs/1603.09229}{{\normalfont\ttfamily
  arXiv:1603.09229}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lebed:2016hpi}
R.~F. Lebed, R.~E. Mitchell, and E.~S. Swanson,
  \ifthenelse{\boolean{articletitles}}{\emph{{Heavy-quark QCD exotica}},
  }{}\href{https://doi.org/10.1016/j.ppnp.2016.11.003}{Prog.\ Part.\ Nucl.\
  Phys.\  \textbf{93} (2017) 143},
  \href{http://arxiv.org/abs/1610.04528}{{\normalfont\ttfamily
  arXiv:1610.04528}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Guo:2017jvc}
F.-K. Guo {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Hadronic
  molecules}}, }{}\href{https://doi.org/10.1103/RevModPhys.90.015004}{Rev.\
  Mod.\ Phys.\  \textbf{90} (2018) 015004},
  \href{http://arxiv.org/abs/1705.00141}{{\normalfont\ttfamily
  arXiv:1705.00141}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Olsen:2017bmm}
S.~L. Olsen, T.~Skwarnicki, and D.~Zieminska,
  \ifthenelse{\boolean{articletitles}}{\emph{{Nonstandard heavy mesons and
  baryons: Experimental evidence}},
  }{}\href{https://doi.org/10.1103/RevModPhys.90.015003}{Rev.\ Mod.\ Phys.\
  \textbf{90} (2018) 015003},
  \href{http://arxiv.org/abs/1708.04012}{{\normalfont\ttfamily
  arXiv:1708.04012}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Brambilla:2019esw}
N.~Brambilla {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{The
  $\PX\PY\PZ$ states: experimental and theoretical status and perspectives}},
  }{}\href{https://doi.org/10.1016/j.physrep.2020.05.001}{Phys.\ Rept.\
  \textbf{873} (2020) 1},
  \href{http://arxiv.org/abs/1907.07583}{{\normalfont\ttfamily
  arXiv:1907.07583}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ali:2019roi}
A.~Ali, L.~Maiani, and A.~D. Polosa, {\em {Multiquark hadrons}},
  \href{https://doi.org/10.1017/9781316761465}{ Cambridge University Press,
  2019}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Richard_2016}
J.-M. Richard, \ifthenelse{\boolean{articletitles}}{\emph{Exotic hadrons:
  Review and perspectives},
  }{}\href{https://doi.org/10.1007/s00601-016-1159-0}{Few-Body Systems
  \textbf{57} (2016) 1185}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Oset:2019upy}
E.~Oset {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Tetra and
  pentaquarks from the molecular perspective}},
  }{}\href{https://doi.org/10.1051/epjconf/201919901003}{EPJ Web Conf.\
  \textbf{199} (2019) 01003}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{MartinezTorres:2020hus}
A.~Martinez~Torres, K.~P. Khemchandani, L.~Roca, and E.~Oset,
  \ifthenelse{\boolean{articletitles}}{\emph{{Few-body systems consisting of
  mesons}}, }{}\href{https://doi.org/10.1007/s00601-020-01568-y}{Few Body
  Syst.\  \textbf{61} (2020) 35},
  \href{http://arxiv.org/abs/2005.14357}{{\normalfont\ttfamily
  arXiv:2005.14357}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Tornqvist:1991ks}
N.~A. Tornqvist, \ifthenelse{\boolean{articletitles}}{\emph{{Possible large
  deuteronlike meson\nobreakdash-meson states bound by pions}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.67.556}{Phys.\ Rev.\ Lett.\
  \textbf{67} (1991) 556}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2017-018}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of the doubly charmed
  baryon \Xiccpp}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.119.112001}{Phys.\ Rev.\ Lett.\
  \textbf{119} (2017) 112001},
  \href{http://arxiv.org/abs/1707.01621}{{\normalfont\ttfamily
  arXiv:1707.01621}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2018-019}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the lifetime of
  the doubly charmed baryon \Xiccpp}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.121.052002}{Phys.\ Rev.\ Lett.\
  \textbf{121} (2018) 052002},
  \href{http://arxiv.org/abs/1806.02744}{{\normalfont\ttfamily
  arXiv:1806.02744}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-011}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of structure in the
  \jpsi-pair mass spectrum}},
  }{}\href{https://doi.org/10.1016/j.scib.2020.08.032}{Science Bulletin
  \textbf{65} (2020) 1983},
  \href{http://arxiv.org/abs/2006.16957}{{\normalfont\ttfamily
  arXiv:2006.16957}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Albuquerque:2020hio}
R.~M. Albuquerque {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Doubly-hidden scalar heavy
  molecules and tetraquarks states from QCD at NLO}},
  }{}\href{https://doi.org/10.1103/PhysRevD.102.094001}{Phys.\ Rev.\
  \textbf{D102} (2020) 094001},
  \href{http://arxiv.org/abs/2008.01569}{{\normalfont\ttfamily
  arXiv:2008.01569}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Dong:2020nwy}
X.-K. Dong {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Coupled-channel interpretation of
  the~LHCb double-$\jpsi$ spectrum and hints of a~new state near
  the~$\jpsi\jpsi$~threshold}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.126.132001}{Phys.\ Rev.\ Lett.\
  \textbf{126} (2021) 132001},
  \href{http://arxiv.org/abs/2009.07795}{{\normalfont\ttfamily
  arXiv:2009.07795}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Bedolla:2019zwg}
M.~A. Bedolla, J.~Ferretti, C.~D. Roberts, and E.~Santopinto,
  \ifthenelse{\boolean{articletitles}}{\emph{{Spectrum of fully-heavy
  tetraquarks from a diquark+antidiquark perspective}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-020-08579-3}{Eur.\ Phys.\ J.\
  \textbf{C80} (2020) 1004},
  \href{http://arxiv.org/abs/1911.00960}{{\normalfont\ttfamily
  arXiv:1911.00960}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Karliner:2020dta}
M.~Karliner and J.~L. Rosner,
  \ifthenelse{\boolean{articletitles}}{\emph{{Interpretation of structure in
  the~di-$\jpsi$~spectrum}},
  }{}\href{https://doi.org/10.1103/PhysRevD.102.114039}{Phys.\ Rev.\
  \textbf{D102} (2020) 114039},
  \href{http://arxiv.org/abs/2009.04429}{{\normalfont\ttfamily
  arXiv:2009.04429}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lu:2020cns}
Q.-F. L\"u, D.-Y. Chen, and Y.-B. Dong,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of fully heavy tetraquarks
  $\PQ\PQ {\bar{\PQ}} {\bar{\PQ}}$ in an extended relativized quark model}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-020-08454-1}{Eur.\ Phys.\ J.\
  \textbf{C80} (2020) 871},
  \href{http://arxiv.org/abs/2006.14445}{{\normalfont\ttfamily
  arXiv:2006.14445}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Giron:2020wpx}
J.~F. Giron and R.~F. Lebed, \ifthenelse{\boolean{articletitles}}{\emph{{Simple
  spectrum of $\cquark\cquarkbar\cquark\cquarkbar$ states in the dynamical
  diquark model}}, }{}\href{https://doi.org/10.1103/PhysRevD.102.074003}{Phys.\
  Rev.\  \textbf{D102} (2020) 074003},
  \href{http://arxiv.org/abs/2008.01631}{{\normalfont\ttfamily
  arXiv:2008.01631}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-024}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Model-independent study of
  structure in \mbox{$\decay{\Bp}{\Dp \Dm \Kp}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.125.242001}{Phys.\ Rev.\ Lett.\
  \textbf{125} (2020) 242001},
  \href{http://arxiv.org/abs/2009.00025}{{\normalfont\ttfamily
  arXiv:2009.00025}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-025}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Amplitude analysis of
  the~\mbox{$\decay{\Bp}{\Dp \Dm \Kp}$}~decay}},
  }{}\href{https://doi.org/10.1103/PhysRevD.102.112003}{Phys.\ Rev.\
  \textbf{D102} (2020) 112003},
  \href{http://arxiv.org/abs/2009.00026}{{\normalfont\ttfamily
  arXiv:2009.00026}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ablikim:2013mio}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~charged
  charmoniumlike structure in \mbox{$\decay{\epem}{\pip\pim\jpsi}$} at
  \mbox{$\sqs=4.26\gev$} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.110.252001}{Phys.\ Rev.\ Lett.\
  \textbf{110} (2013) 252001},
  \href{http://arxiv.org/abs/1303.5949}{{\normalfont\ttfamily
  arXiv:1303.5949}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Belle:2013yex}
Belle collaboration, Z.~Q. Liu {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of
  \mbox{$\decay{\epem}{\pip\pim\jpsi}$} and observation of a~charged
  charmoniumlike state at Belle}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.110.252002}{Phys.\ Rev.\ Lett.\
  \textbf{110} (2013) 252002}, Erratum
  \href{https://doi.org/10.1103/PhysRevLett.111.019901}{ibid.\   \textbf{111}
  (2013) 019901}, \href{http://arxiv.org/abs/1304.0121}{{\normalfont\ttfamily
  arXiv:1304.0121}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{BESIII:2013qmu}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~charged
  \mbox{$(\D\Dstarb)^\pm$} mass peak in \mbox{$\decay{\epem}{\pion \D\Dstarb}$}
  at~\mbox{$\sqs =4.26\gev$}}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.112.022001}{Phys.\ Rev.\ Lett.\
  \textbf{112} (2014) 022001},
  \href{http://arxiv.org/abs/1310.1163}{{\normalfont\ttfamily
  arXiv:1310.1163}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{BESIII:2015cld}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of
  $\Z_{\cquark}(3900)^{0}$ in \mbox{$\decay{\epem}{\piz\piz\jpsi}$}}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.115.112003}{Phys.\ Rev.\ Lett.\
  \textbf{115} (2015) 112003},
  \href{http://arxiv.org/abs/1506.06018}{{\normalfont\ttfamily
  arXiv:1506.06018}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{BESIII:2015ntl}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~neutral
  structure near the~\mbox{$\D\Dstarb$}~mass threshold in \mbox{$\decay{\epem}{
  (\D\Dstarb)^0\piz}$} at~\mbox{$\sqs=4.226$} and~$4.257\gev$ }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.115.222002}{Phys.\ Rev.\ Lett.\
  \textbf{115} (2015) 222002},
  \href{http://arxiv.org/abs/1509.05620}{{\normalfont\ttfamily
  arXiv:1509.05620}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{BESIII:2013ouc}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~charged
  charmoniumlike structure \mbox{$\Z_{\cquark}(4020)$} and search for
  the~\mbox{$\Z_{\cquark}(3900)$} in
  \mbox{$\decay{\epem}{\pip\pim\Ph_{\cquark}}$} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.111.242001}{Phys.\ Rev.\ Lett.\
  \textbf{111} (2013) 242001},
  \href{http://arxiv.org/abs/1309.1896}{{\normalfont\ttfamily
  arXiv:1309.1896}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{BESIII:2013mhi}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~charged
  charmoniumlike structure in
  \mbox{$\decay{\epem}{\left(\Dstar\Dstarb\right)^{\pm}\pion^{\mp}}$}
  at~\mbox{$\sqs=4.26\gev$} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.112.132001}{Phys.\ Rev.\ Lett.\
  \textbf{112} (2014) 132001},
  \href{http://arxiv.org/abs/1308.2760}{{\normalfont\ttfamily
  arXiv:1308.2760}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Belle:2008qeq}
Belle collaboration, R.~Mizuk {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of two
  resonance\nobreakdash-like structures in the~\mbox{$\pip\chicone$}~mass
  distribution in exclusive \mbox{$\decay{\Bdb}{\Km\pip\chicone}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevD.78.072004}{Phys.\ Rev.\
  \textbf{D78} (2008) 072004},
  \href{http://arxiv.org/abs/0806.4098}{{\normalfont\ttfamily
  arXiv:0806.4098}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHcb-PAPER-2018-034}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for
  a~\mbox{$\Peta_\cquark(1\PS) \pim$}~resonance in
  \mbox{\decay{\Bz}{\Peta_\cquark(1\PS)\Kp\pim}}~decays}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-018-6447-z}{Eur.\ Phys.\ J.\
  \textbf{C78} (2018) 1019},
  \href{http://arxiv.org/abs/1809.07416}{{\normalfont\ttfamily
  arXiv:1809.07416}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Chilikin:2014bkk}
Belle collaboration, K.~Chilikin {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~new charged
  charmoniumlike state in \mbox{$\decay{\Bdb}{\jpsi\Km\pip}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevD.90.112009}{Phys.\ Rev.\
  \textbf{D90} (2014) 112009},
  \href{http://arxiv.org/abs/1408.6457}{{\normalfont\ttfamily
  arXiv:1408.6457}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Choi:2007wga}
Belle collaboration, S.~K. Choi {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~resonancelike
  structure in the~\mbox{$\Ppi^\pm\Ppsi^\prime$}~mass distribution in exclusive
  \mbox{$\decay{\B}{\kaon\Ppi^{\pm}\Ppsi^{\prime}}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.100.142001}{Phys.\ Rev.\ Lett.\
  \textbf{100} (2008) 142001},
  \href{http://arxiv.org/abs/0708.1790}{{\normalfont\ttfamily
  arXiv:0708.1790}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Chilikin:2013tch}
Belle collaboration, K.~Chilikin {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Experimental constraints on the
  spin and parity of the~\mbox{$\Z\mathrm{(4430)}^+$}}},
  }{}\href{https://doi.org/10.1103/PhysRevD.88.074026}{Phys.\ Rev.\
  \textbf{D88} (2013) 074026},
  \href{http://arxiv.org/abs/1306.4894}{{\normalfont\ttfamily
  arXiv:1306.4894}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2014-014}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of the~resonant
  character of the~$\Z(4430)^-$~state}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.112.222002}{Phys.\ Rev.\ Lett.\
  \textbf{112} (2014) 222002},
  \href{http://arxiv.org/abs/1404.1903}{{\normalfont\ttfamily
  arXiv:1404.1903}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2015-038}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Model-independent confirmation of
  the $Z(4430)^-$ state}},
  }{}\href{https://doi.org/10.1103/PhysRevD.92.112009}{Phys.\ Rev.\
  \textbf{D92} (2015) 112009},
  \href{http://arxiv.org/abs/1510.01951}{{\normalfont\ttfamily
  arXiv:1510.01951}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ablikim_2021}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of
  a~near\nobreakdash-threshold structure in the~\Kp recoil\nobreakdash-mass
  spectra in \mbox{$\decay{\epem}{\Kp\left(\Dsm \Dstarz +
  \D^{*-}_{\squark}\Dz\right) } $} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.126.102001}{Phys.\ Rev.\ Lett.\
  \textbf{126} (2021) 102001},
  \href{http://arxiv.org/abs/2011.07855}{{\normalfont\ttfamily
  arXiv:2011.07855}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-044}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of new resonances
  decaying to $\jpsi\Kp$ and $\jpsi\Pphi$}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.127.082001}{Phys.\ Rev.\ Lett.\
  \textbf{127} (2020) 082001},
  \href{http://arxiv.org/abs/2103.01803}{{\normalfont\ttfamily
  arXiv:2103.01803}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Aaltonen:2009tz}
CDF collaboration, T.~Aaltonen {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for a~narrow
  near\nobreakdash-threshold structure in the~$\jpsi\Pphi$~mass spectrum in
  \mbox{$\decay{\Bu}{\jpsi\Pphi\Kp}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.102.242002}{Phys.\ Rev.\ Lett.\
  \textbf{102} (2009) 242002},
  \href{http://arxiv.org/abs/0903.2229}{{\normalfont\ttfamily
  arXiv:0903.2229}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Abazov:2013xda}
D0 collaboration, V.~M. Abazov {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Search for the~$\PX(4140)$~state
  in $\decay{\Bu}{\jpsi\Pphi\Kp}$~decays with the D0 Detector}},
  }{}\href{https://doi.org/10.1103/PhysRevD.89.012004}{Phys.\ Rev.\
  \textbf{D89} (2014) 012004},
  \href{http://arxiv.org/abs/1309.6580}{{\normalfont\ttfamily
  arXiv:1309.6580}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Chatrchyan:2013dma}
CMS collaboration, S.~Chatrchyan {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~peaking
  structure in the~$\jpsi\Pphi$~mass spectrum from
  $\decay{\Bu}{\jpsi\Pphi\Kp}$~decays}},
  }{}\href{https://doi.org/10.1016/j.physletb.2014.05.055}{Phys.\ Lett.\
  \textbf{B734} (2014) 261},
  \href{http://arxiv.org/abs/1309.6920}{{\normalfont\ttfamily
  arXiv:1309.6920}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2016-018}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of exotic
  $\jpsi\Pphi$ structures from amplitude analysis of
  \mbox{\decay{\Bp}{\jpsi\Pphi\Kp}} decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.118.022003}{Phys.\ Rev.\ Lett.\
  \textbf{118} (2017) 022003},
  \href{http://arxiv.org/abs/1606.07895}{{\normalfont\ttfamily
  arXiv:1606.07895}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-035}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of \mbox{$\decay{\Bs}{\jpsi
  \pip \pim \Kp \Km}$}~decays}},
  }{}\href{https://doi.org/10.1007/JHEP02(2021)024}{JHEP \textbf{02} (2021)
  024}, \href{http://arxiv.org/abs/2011.01867}{{\normalfont\ttfamily
  arXiv:2011.01867}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Belle:2011aa}
Belle collaboration, A.~Bondar {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of two charged
  bottomonium\nobreakdash-like resonances in $\PUpsilon(5\PS)$~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.108.122001}{Phys.\ Rev.\ Lett.\
  \textbf{108} (2012) 122001},
  \href{http://arxiv.org/abs/1110.2251}{{\normalfont\ttfamily
  arXiv:1110.2251}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2019-014}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a narrow
  pentaquark state, $\PP_\cquark(4312)^+$, and of two-peak structure of
  the~$\PP_\cquark(4450)^+$}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.122.222001}{Phys.\ Rev.\ Lett.\
  \textbf{122} (2019) 222001},
  \href{http://arxiv.org/abs/1904.03947}{{\normalfont\ttfamily
  arXiv:1904.03947}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2015-029}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of $\jpsi\proton$
  resonances consistent with pentaquark states in
  \mbox{\decay{\Lb}{\jpsi\proton\Km}} decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.115.072001}{Phys.\ Rev.\ Lett.\
  \textbf{115} (2015) 072001},
  \href{http://arxiv.org/abs/1507.03414}{{\normalfont\ttfamily
  arXiv:1507.03414}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2021-018}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for a~new structure in
  the~$\jpsi\proton$ and $\jpsi\antiproton$~systems
  in~\mbox{$\decay{\Bs}{\jpsi\proton\antiproton}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.128.062001}{Phys.\ Rev.\ Lett.\
  \textbf{128} (2021) 062001},
  \href{http://arxiv.org/abs/2108.04720}{{\normalfont\ttfamily
  arXiv:2108.04720}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-039}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence of a $\jpsi\Lz$
  structure and observation of excited $\Xim$ states in
  the~\mbox{$\decay{\Xibm}{\jpsi \Lz \Km}$}~decay}},
  }{}\href{https://doi.org/10.1016/j.scib.2021.02.030}{Science Bulletin
  \textbf{66} (2021) 1278},
  \href{http://arxiv.org/abs/2012.10380}{{\normalfont\ttfamily
  arXiv:2012.10380}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ader:1981db}
J.~P. Ader, J.~M. Richard, and P.~Taxil,
  \ifthenelse{\boolean{articletitles}}{\emph{{Do narrow heavy multiquark states
  exist?}}, }{}\href{https://doi.org/10.1103/PhysRevD.25.2370}{Phys.\ Rev.\
  \textbf{D25} (1982) 2370}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ballot:1983iv}
J.~l. Ballot and J.~M. Richard,
  \ifthenelse{\boolean{articletitles}}{\emph{{Four quark states in additive
  potentials}}, }{}\href{https://doi.org/10.1016/0370-2693(83)90991-7}{Phys.\
  Lett.\  \textbf{B123} (1983) 449}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Zouzou:1986qh}
S.~Zouzou, B.~Silvestre-Brac, C.~Gignoux, and J.~M. Richard,
  \ifthenelse{\boolean{articletitles}}{\emph{{Four quark bound states}},
  }{}\href{https://doi.org/10.1007/BF01557611}{Z.\ Phys.\  \textbf{C30} (1986)
  457}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lipkin:1986dw}
H.~J. Lipkin, \ifthenelse{\boolean{articletitles}}{\emph{{A~model-independent
  approach to multiquark bound states}},
  }{}\href{https://doi.org/10.1016/0370-2693(86)90843-9}{Phys.\ Lett.\
  \textbf{B172} (1986) 242}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Heller:1986bt}
L.~Heller and J.~A. Tjon, \ifthenelse{\boolean{articletitles}}{\emph{{On
  the~existence of stable dimesons}},
  }{}\href{https://doi.org/10.1103/PhysRevD.35.969}{Phys.\ Rev.\  \textbf{D35}
  (1987) 969}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Manohar:1992nd}
A.~V. Manohar and M.~B. Wise,
  \ifthenelse{\boolean{articletitles}}{\emph{{Exotic
  $\PQ\PQ\bar{\Pq}\bar{\Pq}$~states in QCD}},
  }{}\href{https://doi.org/10.1016/0550-3213(93)90614-U}{Nucl.\ Phys.\
  \textbf{B399} (1993) 17},
  \href{http://arxiv.org/abs/hep-ph/9212236}{{\normalfont\ttfamily
  arXiv:hep-ph/9212236}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Carlson:1987hh}
J.~Carlson, L.~Heller, and J.~A. Tjon,
  \ifthenelse{\boolean{articletitles}}{\emph{{Stability of dimesons}},
  }{}\href{https://doi.org/10.1103/PhysRevD.37.744}{Phys.\ Rev.\  \textbf{D37}
  (1988) 744}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{SilvestreBrac:1993ss}
B.~Silvestre-Brac and C.~Semay,
  \ifthenelse{\boolean{articletitles}}{\emph{{Systematics of \mbox{$L = 0$}
  \mbox{$\quark^2\quarkbar^2$}~systems}},
  }{}\href{https://doi.org/10.1007/BF01565058}{Z.\ Phys.\  \textbf{C57} (1993)
  273}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Semay:1994ht}
C.~Semay and B.~Silvestre-Brac,
  \ifthenelse{\boolean{articletitles}}{\emph{{Diquonia and potential models}},
  }{}\href{https://doi.org/10.1007/BF01413104}{Z.\ Phys.\  \textbf{C61} (1994)
  271}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Moinester:1995fk}
M.~A. Moinester, \ifthenelse{\boolean{articletitles}}{\emph{{How to search for
  doubly charmed baryons and tetraquarks}},
  }{}\href{https://doi.org/10.1007/s002180050123}{Z.\ ~Phys.\  \textbf{A355}
  (1996) 349}, \href{http://arxiv.org/abs/hep-ph/9506405}{{\normalfont\ttfamily
  arXiv:hep-ph/9506405}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Pepin:1996id}
S.~Pepin, F.~Stancu, M.~Genovese, and J.~M. Richard,
  \ifthenelse{\boolean{articletitles}}{\emph{{Tetraquarks with color blind
  forces in chiral quark models}},
  }{}\href{https://doi.org/10.1016/S0370-2693(96)01597-3}{Phys.\ Lett.\
  \textbf{B393} (1997) 119},
  \href{http://arxiv.org/abs/hep-ph/9609348}{{\normalfont\ttfamily
  arXiv:hep-ph/9609348}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{GELMAN2003296}
B.~A. Gelman and S.~Nussinov, \ifthenelse{\boolean{articletitles}}{\emph{Does
  a~narrow tetraquark $\cquark\cquark\uquarkbar\dquarkbar$~state exist?},
  }{}\href{https://doi.org/https://doi.org/10.1016/S0370-2693(02)03069-1}{Phys.\
  Lett.\  \textbf{B551} (2003) 296}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Vijande:2003ki}
J.~Vijande, F.~Fernandez, A.~Valcarce, and B.~Silvestre-Brac,
  \ifthenelse{\boolean{articletitles}}{\emph{{Tetraquarks in a chiral
  constituent quark model}},
  }{}\href{https://doi.org/10.1140/epja/i2003-10128-9}{Eur.\ Phys.\ J.\
  \textbf{A19} (2004) 383},
  \href{http://arxiv.org/abs/hep-ph/0310007}{{\normalfont\ttfamily
  arXiv:hep-ph/0310007}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Janc:2004qn}
D.~Janc and M.~Rosina, \ifthenelse{\boolean{articletitles}}{\emph{{The
  $\PT_{\cquark\cquark} = \D\Dstar$ molecular state}},
  }{}\href{https://doi.org/10.1007/s00601-004-0068-9}{Few Body Syst.\
  \textbf{35} (2004) 175},
  \href{http://arxiv.org/abs/hep-ph/0405208}{{\normalfont\ttfamily
  arXiv:hep-ph/0405208}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Navarra:2007yw}
F.~S. Navarra, M.~Nielsen, and S.~H. Lee,
  \ifthenelse{\boolean{articletitles}}{\emph{{QCD sum rules study of
  \mbox{$\PQ\PQ-\uquarkbar\dquarkbar$}~mesons}},
  }{}\href{https://doi.org/10.1016/j.physletb.2007.04.010}{Phys.\ Lett.\
  \textbf{B649} (2007) 166},
  \href{http://arxiv.org/abs/hep-ph/0703071}{{\normalfont\ttfamily
  arXiv:hep-ph/0703071}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Vijande}
J.~Vijande, E.~Weissman, A.~Valcarce, and N.~Barnea,
  \ifthenelse{\boolean{articletitles}}{\emph{Are there compact heavy four-quark
  bound states?}, }{}\href{https://doi.org/10.1103/PhysRevD.76.094027}{Phys.\
  Rev.\  \textbf{D76} (2007) 094027},
  \href{http://arxiv.org/abs/0710.2516}{{\normalfont\ttfamily
  arXiv:0710.2516}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ebert:2007rn}
D.~Ebert, R.~N. Faustov, V.~O. Galkin, and W.~Lucha,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of tetraquarks with two
  heavy quarks in the relativistic quark model}},
  }{}\href{https://doi.org/10.1103/PhysRevD.76.114015}{Phys.\ Rev.\
  \textbf{D76} (2007) 114015},
  \href{http://arxiv.org/abs/0706.3853}{{\normalfont\ttfamily
  arXiv:0706.3853}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lee:2009rt}
S.~H. Lee and S.~Yasui, \ifthenelse{\boolean{articletitles}}{\emph{{Stable
  multiquark states with heavy quarks in a diquark model}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-009-1140-x}{Eur.\ Phys.\ J.\
  \textbf{C64} (2009) 283},
  \href{http://arxiv.org/abs/0901.2977}{{\normalfont\ttfamily
  arXiv:0901.2977}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Yang2009}
Y.~Yang, C.~Deng, J.~Ping, and T.~Goldman,
  \ifthenelse{\boolean{articletitles}}{\emph{{\PS-wave
  $\mathrm{QQ}\quarkbar\quarkbar$ state in the~constituent quark model}},
  }{}\href{https://doi.org/10.1103/PhysRevD.80.114023}{Phys.\ Rev.\
  \textbf{D80} (2009) 114023}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Li:2012ss}
N.~Li, Z.-F. Sun, X.~Liu, and S.-L. Zhu,
  \ifthenelse{\boolean{articletitles}}{\emph{{Coupled\nobreakdash-channel
  analysis of the~possible \mbox{$\D^{(*)}\D^{(*)}$},
  \mbox{$\Bbar^{(*)}\Bbar^{(*)}$} and \mbox{$\D^{(*)}\Bbar^{(*)}$}~molecular
  states}}, }{}\href{https://doi.org/10.1103/PhysRevD.88.114008}{Phys.\ Rev.\
  \textbf{D88} (2013) 114008},
  \href{http://arxiv.org/abs/1211.5007}{{\normalfont\ttfamily
  arXiv:1211.5007}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Feng:2013kea}
G.-Q. Feng, X.-H. Guo, and B.-S. Zou,
  \ifthenelse{\boolean{articletitles}}{\emph{{$\mathrm{QQ}^{\prime} \uquarkbar
  \dquarkbar$ bound state in the Bethe-Salpeter equation approach}},
  }{}\href{http://arxiv.org/abs/1309.7813}{{\normalfont\ttfamily
  arXiv:1309.7813}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Luo:2017eub}
S.-Q. Luo {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Exotic
  tetraquark states with the $\Pq\Pq\bar{\PQ}\bar{\PQ}$ configuration}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-017-5297-4}{Eur.\ Phys.\ J.\
  \textbf{C77} (2017) 709},
  \href{http://arxiv.org/abs/1707.01180}{{\normalfont\ttfamily
  arXiv:1707.01180}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Karliner:2017qjm}
M.~Karliner and J.~L. Rosner,
  \ifthenelse{\boolean{articletitles}}{\emph{{Discovery of doubly-charmed
  $\Xi_{\cquark\cquark}$ baryon implies a~stable \mbox{$\bquark\bquark
  \uquarkbar \dquarkbar$}~tetraquark}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.119.202001}{Phys.\ Rev.\ Lett.\
  \textbf{119} (2017) 202001},
  \href{http://arxiv.org/abs/1707.07666}{{\normalfont\ttfamily
  arXiv:1707.07666}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Eichten:2017ffp}
E.~J. Eichten and C.~Quigg,
  \ifthenelse{\boolean{articletitles}}{\emph{{Heavy-quark symmetry implies
  stable heavy tetraquark mesons $\PQ_i\PQ_j \bar \Pq_k \bar \Pq_l$}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.119.202002}{Phys.\ Rev.\ Lett.\
  \textbf{119} (2017) 202002},
  \href{http://arxiv.org/abs/1707.09575}{{\normalfont\ttfamily
  arXiv:1707.09575}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Wang:2017uld}
Z.-G. Wang, \ifthenelse{\boolean{articletitles}}{\emph{{Analysis of
  the~axialvector doubly heavy tetraquark states with QCD sum rules}},
  }{}\href{https://doi.org/10.5506/APhysPolB.49.1781}{Acta Phys.\ Polon.\
  \textbf{B49} (2018) 1781},
  \href{http://arxiv.org/abs/1708.04545}{{\normalfont\ttfamily
  arXiv:1708.04545}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Park:2018wjk}
W.~Park, S.~Noh, and S.~H. Lee,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of the~doubly heavy
  tetraquarks in a~constituent quark model}},
  }{}\href{https://doi.org/10.1016/j.nuclphysa.2018.12.019}{Acta Phys.\ Polon.\
   \textbf{B50} (2019) 1151},
  \href{http://arxiv.org/abs/1809.05257}{{\normalfont\ttfamily
  arXiv:1809.05257}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Junnarkar:2018twb}
P.~Junnarkar, N.~Mathur, and M.~Padmanath,
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of doubly heavy tetraquarks
  in lattice QCD}}, }{}\href{https://doi.org/10.1103/PhysRevD.99.034507}{Phys.\
  Rev.\  \textbf{D99} (2019) 034507},
  \href{http://arxiv.org/abs/1810.12285}{{\normalfont\ttfamily
  arXiv:1810.12285}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Deng:2018kly}
C.~Deng, H.~Chen, and J.~Ping,
  \ifthenelse{\boolean{articletitles}}{\emph{{Systematical investigation on the
  stability of doubly heavy tetraquark states}},
  }{}\href{https://doi.org/10.1140/epja/s10050-019-00012-y}{Eur.\ Phys.\ J.\
  \textbf{A56} (2020) 9},
  \href{http://arxiv.org/abs/1811.06462}{{\normalfont\ttfamily
  arXiv:1811.06462}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Liu:2019stu}
M.-Z. Liu {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Heavy\nobreakdash-quark spin and
  flavor symmetry partners of the~\mbox{$\PX(3872)$}~revisited: What can we
  learn from the~one boson exchange model?}},
  }{}\href{https://doi.org/10.1103/PhysRevD.99.094018}{Phys.\ Rev.\
  \textbf{D99} (2019) 094018},
  \href{http://arxiv.org/abs/1902.03044}{{\normalfont\ttfamily
  arXiv:1902.03044}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Maiani:2019lpu}
L.~Maiani, A.~D. Polosa, and V.~Riquer,
  \ifthenelse{\boolean{articletitles}}{\emph{{Hydrogen bond of QCD in doubly
  heavy baryons and tetraquarks}},
  }{}\href{https://doi.org/10.1103/PhysRevD.100.074002}{Phys.\ Rev.\
  \textbf{D100} (2019) 074002},
  \href{http://arxiv.org/abs/1908.03244}{{\normalfont\ttfamily
  arXiv:1908.03244}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Yang:2019itm}
G.~Yang, J.~Ping, and J.~Segovia,
  \ifthenelse{\boolean{articletitles}}{\emph{{Doubly-heavy tetraquarks}},
  }{}\href{https://doi.org/10.1103/PhysRevD.101.014001}{Phys.\ Rev.\
  \textbf{D101} (2020) 014001},
  \href{http://arxiv.org/abs/1911.00215}{{\normalfont\ttfamily
  arXiv:1911.00215}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Tan:2020ldi}
Y.~Tan, W.~Lu, and J.~Ping,
  \ifthenelse{\boolean{articletitles}}{\emph{{$\PQ\PQ\bar{\Pq}\bar{\Pq}$ in
  a~chiral constituent quark model}},
  }{}\href{https://doi.org/10.1140/epjp/s13360-020-00741-w}{Eur.\ Phys.\ J.\
  Plus \textbf{135} (2020) 716},
  \href{http://arxiv.org/abs/2004.02106}{{\normalfont\ttfamily
  arXiv:2004.02106}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lu:2020rog}
Q.-F. L\"u, D.-Y. Chen, and Y.-B. Dong,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of doubly heavy
  tetraquarks $\PT_{\PQ\PQ^\prime}$ in a relativized quark model}},
  }{}\href{https://doi.org/10.1103/PhysRevD.102.034012}{Phys.\ Rev.\
  \textbf{D102} (2020) 034012},
  \href{http://arxiv.org/abs/2006.08087}{{\normalfont\ttfamily
  arXiv:2006.08087}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Braaten:2020nwp}
E.~Braaten, L.-P. He, and A.~Mohapatra,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of doubly heavy
  tetraquarks with error bars}},
  }{}\href{https://doi.org/10.1103/PhysRevD.103.016001}{Phys.\ Rev.\
  \textbf{D103} (2021) 016001},
  \href{http://arxiv.org/abs/2006.08650}{{\normalfont\ttfamily
  arXiv:2006.08650}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Gao:2020ogo}
D.~Gao {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Masses of
  doubly heavy tetraquark states with isospin = $\frac{1}{2}$ and $1$ and
  spin\nobreakdash-parity $1^{+\pm}$}},
  }{}\href{http://arxiv.org/abs/2007.15213}{{\normalfont\ttfamily
  arXiv:2007.15213}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Cheng:2020wxa}
J.-B. Cheng {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Double-heavy tetraquark states
  with heavy diquark-antiquark symmetry}},
  }{}\href{https://doi.org/10.1088/1674-1137/abde2f}{Chin.\ Phys.\
  \textbf{C45} (2021) 043102},
  \href{http://arxiv.org/abs/2008.00737}{{\normalfont\ttfamily
  arXiv:2008.00737}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Noh:2021lqs}
S.~Noh, W.~Park, and S.~H. Lee,
  \ifthenelse{\boolean{articletitles}}{\emph{{The~doubly\nobreakdash-heavy
  tetraquarks, $\Pq\Pq^{\prime}\bar{\PQ}\bar{\PQ}^{\prime}$, in a~constituent
  quark model with a~complete set of harmonic oscillator bases}},
  }{}\href{https://doi.org/10.1103/PhysRevD.103.114009}{Phys.\ Rev.\
  \textbf{D103} (2021) 114009},
  \href{http://arxiv.org/abs/2102.09614}{{\normalfont\ttfamily
  arXiv:2102.09614}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Faustov:2021hjs}
R.~N. Faustov, V.~O. Galkin, and E.~M. Savchenko,
  \ifthenelse{\boolean{articletitles}}{\emph{{Heavy tetraquarks in
  the~relativistic quark model}},
  }{}\href{https://doi.org/10.3390/universe7040094}{Universe \textbf{7} (2021)
  94}, \href{http://arxiv.org/abs/2103.01763}{{\normalfont\ttfamily
  arXiv:2103.01763}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2021-031}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of an~exotic narrow
  doubly charmed tetraquark}},
  }{}\href{http://arxiv.org/abs/2109.01038}{{\normalfont\ttfamily
  arXiv:2109.01038}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2008-001}
LHCb collaboration, A.~A. Alves~Jr.\ {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{The \lhcb detector at the LHC}},
  }{}\href{https://doi.org/10.1088/1748-0221/3/08/S08005}{JINST \textbf{3}
  (2008) S08005}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2014-002}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{LHCb detector performance}},
  }{}\href{https://doi.org/10.1142/S0217751X15300227}{Int.\ J.\ Mod.\ Phys.\
  \textbf{A30} (2015) 1530022},
  \href{http://arxiv.org/abs/1412.6352}{{\normalfont\ttfamily
  arXiv:1412.6352}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2012-003}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of double charm
  production involving open charm in \proton\proton collisions at
  \mbox{$\sqs=$7\tev}}}, }{}\href{https://doi.org/10.1007/JHEP06(2012)141}{JHEP
  \textbf{06} (2012) 141}, Addendum
  \href{https://doi.org/10.1007/JHEP03(2014)108}{ibid.\   \textbf{03} (2014)
  108}, \href{http://arxiv.org/abs/1205.0975}{{\normalfont\ttfamily
  arXiv:1205.0975}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2013-062}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of associated
  production of a \Z boson with a \D meson in the forward region}},
  }{}\href{https://doi.org/10.1007/JHEP04(2014)091}{JHEP \textbf{04} (2014)
  091}, \href{http://arxiv.org/abs/1401.3245}{{\normalfont\ttfamily
  arXiv:1401.3245}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2015-046}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Production of associated
  \Upsilonres and open charm hadrons in \proton\proton collisions at $\sqs = $7
  and 8\tev via double parton scattering}},
  }{}\href{https://doi.org/10.1007/JHEP07(2016)052}{JHEP \textbf{07} (2016)
  052}, \href{http://arxiv.org/abs/1510.05949}{{\normalfont\ttfamily
  arXiv:1510.05949}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2019-005}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Near-threshold \D\Db spectroscopy
  and observation of a new charmonium state}},
  }{}\href{https://doi.org/10.1007/JHEP07(2019)035}{JHEP \textbf{07} (2019)
  035}, \href{http://arxiv.org/abs/1903.12240}{{\normalfont\ttfamily
  arXiv:1903.12240}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Blatt:1952ije}
J.~M. Blatt and V.~F. Weisskopf, {\em {Theoretical nuclear physics}},
  \href{https://doi.org/10.1007/978-1-4612-9959-2}{ Springer, New York,
  1952}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{VonHippel:1972fg}
F.~von Hippel and C.~Quigg,
  \ifthenelse{\boolean{articletitles}}{\emph{{Centrifugal-barrier effects in
  resonance partial decay widths, shapes, and production amplitudes}},
  }{}\href{https://doi.org/10.1103/PhysRevD.5.624}{Phys.\ Rev.\  \textbf{D5}
  (1972) 624}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Hanhart:2007yq}
C.~Hanhart, Y.~S. Kalashnikova, A.~E. Kudryavtsev, and A.~V. Nefediev,
  \ifthenelse{\boolean{articletitles}}{\emph{{Reconciling the~$\PX(3872)$ with
  the~near\nobreakdash-threshold enhancement in the~$\Dz\Dstarzb$~final
  state}}, }{}\href{https://doi.org/10.1103/PhysRevD.76.034007}{Phys.\ Rev.\
  \textbf{D76} (2007) 034007},
  \href{http://arxiv.org/abs/0704.0605}{{\normalfont\ttfamily
  arXiv:0704.0605}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Braaten:2007dw}
E.~Braaten and M.~Lu, \ifthenelse{\boolean{articletitles}}{\emph{{Line shapes
  of the~$\PX(3872)$}},
  }{}\href{https://doi.org/10.1103/PhysRevD.76.094028}{Phys.\ Rev.\
  \textbf{D76} (2007) 094028},
  \href{http://arxiv.org/abs/0709.2697}{{\normalfont\ttfamily
  arXiv:0709.2697}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Stapleton:2009ey}
E.~Braaten and J.~Stapleton,
  \ifthenelse{\boolean{articletitles}}{\emph{{Analysis of $\jpsi\pip\pim$ and
  $\Dz\Dzb\piz$~decays of the~$\PX(3872)$}},
  }{}\href{https://doi.org/10.1103/PhysRevD.81.014019}{Phys.\ Rev.\
  \textbf{D81} (2010) 014019},
  \href{http://arxiv.org/abs/0907.3167}{{\normalfont\ttfamily
  arXiv:0907.3167}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Kalashnikova:2009gt}
Y.~S. Kalashnikova and A.~V. Nefediev,
  \ifthenelse{\boolean{articletitles}}{\emph{{Nature of~$\PX(3872)$ from
  data}}, }{}\href{https://doi.org/10.1103/PhysRevD.80.074004}{Phys.\ Rev.\
  \textbf{D80} (2009) 074004},
  \href{http://arxiv.org/abs/0907.4901}{{\normalfont\ttfamily
  arXiv:0907.4901}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Artoisenet:2010va}
P.~Artoisenet, E.~Braaten, and D.~Kang,
  \ifthenelse{\boolean{articletitles}}{\emph{{Using line shapes to discriminate
  between binding mechanisms for the~$\PX(3872)$}},
  }{}\href{https://doi.org/10.1103/PhysRevD.82.014013}{Phys.\ Rev.\
  \textbf{D82} (2010) 014013},
  \href{http://arxiv.org/abs/1005.2167}{{\normalfont\ttfamily
  arXiv:1005.2167}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Hanhart:2010wh}
C.~Hanhart, Y.~S. Kalashnikova, and A.~V. Nefediev,
  \ifthenelse{\boolean{articletitles}}{\emph{{Lineshapes for composite
  particles with unstable constituents}},
  }{}\href{https://doi.org/10.1103/PhysRevD.81.094028}{Phys.\ Rev.\
  \textbf{D81} (2010) 094028},
  \href{http://arxiv.org/abs/1002.4097}{{\normalfont\ttfamily
  arXiv:1002.4097}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Hanhart:2011jz}
C.~Hanhart, Y.~S. Kalashnikova, and A.~V. Nefediev,
  \ifthenelse{\boolean{articletitles}}{\emph{{Interplay of quark and meson
  degrees of freedom in a near-threshold resonance: multi-channel case}},
  }{}\href{https://doi.org/10.1140/epja/i2011-11101-9}{Eur.\ Phys.\ J.\
  \textbf{A47} (2011) 101},
  \href{http://arxiv.org/abs/1106.1185}{{\normalfont\ttfamily
  arXiv:1106.1185}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Hanhart:2015cua}
C.~Hanhart {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Practical
  parametrization for line shapes of near\nobreakdash-threshold states}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.115.202001}{Phys.\ Rev.\ Lett.\
  \textbf{115} (2015) 202001},
  \href{http://arxiv.org/abs/1507.00382}{{\normalfont\ttfamily
  arXiv:1507.00382}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Guo:2016bjq}
F.-K. Guo {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Interplay
  of quark and meson degrees of freedom in near\nobreakdash-threshold states:
  A~practical parametrization for line shapes}},
  }{}\href{https://doi.org/10.1103/PhysRevD.93.074031}{Phys.\ Rev.\
  \textbf{D93} (2016) 074031},
  \href{http://arxiv.org/abs/1602.00940}{{\normalfont\ttfamily
  arXiv:1602.00940}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Hanhart:2016eyl}
C.~Hanhart {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{A
  practical parametrisation of line shapes of near\nobreakdash-threshold
  resonances}}, }{}\href{https://doi.org/10.1088/1742-6596/675/2/022016}{J.\
  Phys.\ Conf.\ Ser.\  \textbf{675} (2016) 022016}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Guo:2017jpg}
F.~K. Guo {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Phenomenology of near-threshold
  states: A~practical parametrisation for the line shapes}},
  }{}\href{https://doi.org/10.1051/epjconf/201713706020}{EPJ Web Conf.\
  \textbf{137} (2017) 06020}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Mikhasenko:2019vhk}
M.~Mikhasenko {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Three\nobreakdash-body
  scattering: ladders and resonances}},
  }{}\href{https://doi.org/10.1007/JHEP08(2019)080}{JHEP \textbf{08} (2019)
  080}, \href{http://arxiv.org/abs/1904.11894}{{\normalfont\ttfamily
  arXiv:1904.11894}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Pasquier:1968zz}
R.~Pasquier and J.~Y. Pasquier,
  \ifthenelse{\boolean{articletitles}}{\emph{{Khuri\nobreakdash-Treiman\nobreakdash-type
  equations for three\nobreakdash-body Decay and Production Processes}},
  }{}\href{https://doi.org/10.1103/PhysRev.170.1294}{Phys.\ Rev.\  \textbf{170}
  (1968) 1294}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Aitchison:1979fj}
I.~J.~R. Aitchison and J.~J. Brehm,
  \ifthenelse{\boolean{articletitles}}{\emph{{ARE THERE IMPORTANT UNITARITY
  CORRECTIONS TO THE ISOBAR MODEL?}},
  }{}\href{https://doi.org/10.1016/0370-2693(79)90056-X}{Phys.\ Lett.\ B
  \textbf{84} (1979) 349}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-008}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of the line shape of the
  $\chicone(3872)$ state}},
  }{}\href{https://doi.org/10.1103/PhysRevD.102.092005}{Phys.\ Rev.\
  \textbf{D102} (2020) 092005},
  \href{http://arxiv.org/abs/2005.13419}{{\normalfont\ttfamily
  arXiv:2005.13419}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-009}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of the $\psires_2(3823)$
  and $\chicone(3872)$ states in \mbox{$\decay{\Bp}{\left(\jpsi
  \pip\pim\right)\Kp}$} decays}},
  }{}\href{https://doi.org/10.1007/JHEP08(2020)123}{JHEP \textbf{08} (2020)
  123}, \href{http://arxiv.org/abs/2005.13422}{{\normalfont\ttfamily
  arXiv:2005.13422}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Kallen}
G.~K{\"{a}}ll{\'{e}}n, {\em {Elementary particle physics}},
  Addison\nobreakdash-Wesley, Reading, Massachusetts, 1964\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Flatte:1976xu}
S.~M. Flatt\'e, \ifthenelse{\boolean{articletitles}}{\emph{{Coupled-channel
  analysis of the~$\Ppi\Peta$ and $\kaon\Kb$~systems near
  $\kaon\Kb$~threshold}},
  }{}\href{https://doi.org/10.1016/0370-2693(76)90654-7}{Phys.\ Lett.\
  \textbf{B63} (1976) 224}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Baru:2004xg}
V.~Baru {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Flatt\'e-like
  distributions and the~\mbox{$a_0(980)/f_0(980)$}~mesons}},
  }{}\href{https://doi.org/10.1140/epja/i2004-10105-x}{Eur.\ Phys.\ J.\
  \textbf{A23} (2005) 523},
  \href{http://arxiv.org/abs/nucl-th/0410099}{{\normalfont\ttfamily
  arXiv:nucl-th/0410099}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Santos:2013gra}
D.~Mart{\'\i}nez~Santos and F.~Dupertuis,
  \ifthenelse{\boolean{articletitles}}{\emph{{Mass distributions marginalized
  over per-event errors}},
  }{}\href{https://doi.org/10.1016/j.nima.2014.06.081}{Nucl.\ Instrum.\ Meth.\
  \textbf{A764} (2014) 150},
  \href{http://arxiv.org/abs/1312.5000}{{\normalfont\ttfamily
  arXiv:1312.5000}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Skwarnicki:1986xj}
T.~Skwarnicki, {\em {A study of the~radiative cascade transitions between
  the~$\PUpsilon^{\prime}$ and $\PUpsilon$~resonances}}, PhD thesis, Institute
  of Nuclear Physics, Krakow, 1986,
  {\href{http://inspirehep.net/record/230779/}{DESY-F31-86-02}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2011-013}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of \jpsi-pair
  production in \proton\proton collisions at \mbox{$\sqs=$7\tev}}},
  }{}\href{https://doi.org/10.1016/j.physletb.2011.12.015}{Phys.\ Lett.\
  \textbf{B707} (2012) 52},
  \href{http://arxiv.org/abs/1109.0963}{{\normalfont\ttfamily
  arXiv:1109.0963}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Student}
{Student~(W.\ \,S.\ ~Gosset)},
  \ifthenelse{\boolean{articletitles}}{\emph{{The~probable error of a~mean}},
  }{}\href{https://doi.org/10.1093/biomet/6.1.1}{Biometrika \textbf{6} (1908)
  1}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Jackman}
S.~Jackman, {\em Bayesian analysis for the social sciences}, John Wiley \&
  Sons, Inc., Hoboken, New Jersey, USA, 2009\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{JohnsonSU1}
N.~L. Johnson, \ifthenelse{\boolean{articletitles}}{\emph{Systems of frequency
  curves generated by methods of translation},
  }{}\href{https://doi.org/10.1093/biomet/36.1-2.149}{Biometrika \textbf{36}
  (1949) 149}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{JohnsonSU2}
N.~L. Johnson, \ifthenelse{\boolean{articletitles}}{\emph{{Bivariate
  distributions based on simplie translation systems}},
  }{}\href{https://doi.org/10.1093/biomet/36.3-4.297}{Biometrika \textbf{36}
  (1949) 297}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Bukin}
\babar collaboration, J.~P. Lees {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Branching fraction measurements
  of the~color\nobreakdash-suppressed decays \Bzb to $\D^{(*)0}\piz$,
  $\D^{(*)0}\Peta$, $\D^{(*)0}\Pomega$, and $\D^{(*)0}\Peta^{\prime}$ and
  measurement of the~polarization in the~decay
  \mbox{$\decay{\Bzb}{\Dstarz\Pomega}$} }},
  }{}\href{https://doi.org/10.1103/PhysRevD.84.112007}{Phys.\ Rev.\
  \textbf{D84} (2011) 112007}, Erratum
  \href{https://doi.org/10.1103/PhysRevD.87.039901}{ibid.\   \textbf{D87}
  (2013) 039901(E)},
  \href{http://arxiv.org/abs/1107.5751}{{\normalfont\ttfamily
  arXiv:1107.5751}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2017-036}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{$\Pchi_{\cquark1}$ and
  $\Pchi_{\cquark2}$ resonance parameters with the~decays
  \mbox{\decay{\Pchi_{\cquark1,\cquark2}}{\jpsi\mumu}}}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.119.221801}{Phys.\ Rev.\ Lett.\
  \textbf{119} (2017) 221801},
  \href{http://arxiv.org/abs/1709.04247}{{\normalfont\ttfamily
  arXiv:1709.04247}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2019-045}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a new baryon state
  in the $\Lb\pip\pim$ mass spectrum}},
  }{}\href{https://doi.org/10.1007/JHEP06(2020)136}{JHEP \textbf{06} (2020)
  136}, \href{http://arxiv.org/abs/2002.05112}{{\normalfont\ttfamily
  arXiv:2002.05112}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2021-023}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Updated search for $\Bc$~decays
  to two open charm mesons}},
  }{}\href{https://doi.org/10.1007/JHEP12(2021)117}{JHEP \textbf{12} (2021)
  117}, \href{http://arxiv.org/abs/2109.00488}{{\normalfont\ttfamily
  arXiv:2109.00488}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Byckling}
E.~Byckling and K.~Kajantie, {\em Particle kinematics}, John Wiley \& Sons
  Inc., New York, 1973\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lees:2013zna}
BaBar collaboration, J.~P. Lees {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the~$\D^*(2010)^+$
  meson width and the~\mbox{$\D^*(2010)^+ - \Dz$}~mass difference}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.111.111801}{Phys.\ Rev.\ Lett.\
  \textbf{111} (2013) 111801},
  \href{http://arxiv.org/abs/1304.5657}{{\normalfont\ttfamily
  arXiv:1304.5657}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Guo:2019qcn}
F.-K. Guo, \ifthenelse{\boolean{articletitles}}{\emph{{Novel method for
  precisely measuring the~$\PX(3872)$~mass}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.122.202002}{Phys.\ Rev.\ Lett.\
  \textbf{122} (2019) 202002},
  \href{http://arxiv.org/abs/1902.11221}{{\normalfont\ttfamily
  arXiv:1902.11221}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2012-048}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Measurements of the \Lb, \Xibm,
  and \Omegab baryon masses}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.110.182001}{Phys.\ Rev.\ Lett.\
  \textbf{110} (2013) 182001},
  \href{http://arxiv.org/abs/1302.1072}{{\normalfont\ttfamily
  arXiv:1302.1072}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2013-011}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Precision measurement of \D meson
  mass differences}}, }{}\href{https://doi.org/10.1007/JHEP06(2013)065}{JHEP
  \textbf{06} (2013) 065},
  \href{http://arxiv.org/abs/1304.6865}{{\normalfont\ttfamily
  arXiv:1304.6865}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Bethe}
H.~A. Bethe, \ifthenelse{\boolean{articletitles}}{\emph{{Zur Theorie des
  Durchgangs schneller Korpuskularstrahlen durch Materie}},
  }{}\href{https://doi.org/10.1002/andp.19303970303}{Annalen der Physik
  \textbf{397} (1930) 325}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{BLOCH}
F.~Bloch, \ifthenelse{\boolean{articletitles}}{\emph{{Zur Bremsung rasch
  bewegter Teilchen beim Durchgang durch Materie}},
  }{}\href{https://doi.org/https://doi.org/10.1002/andp.19334080303}{Annalen
  der Physik \textbf{408} (1933) 285}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2010-001}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Prompt \KS production in
  \proton\proton collisions at $\sqs=$0.9\tev}},
  }{}\href{https://doi.org/10.1016/j.physletb.2010.08.055}{Phys.\ Lett.\
  \textbf{B693} (2010) 69},
  \href{http://arxiv.org/abs/1008.3105}{{\normalfont\ttfamily
  arXiv:1008.3105}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Anastassov:2001cw}
CLEO collaboration, A.~Anastassov {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{First measurement of
  $\Gamma(\Dstarp)$ and precision measurement of \mbox{$m_{\Dstarp}-m_{\Dz}$}
  }}, }{}\href{https://doi.org/10.1103/PhysRevD.65.032003}{Phys.\ Rev.\
  \textbf{D65} (2002) 032003},
  \href{http://arxiv.org/abs/hep-ex/0108043}{{\normalfont\ttfamily
  arXiv:hep-ex/0108043}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Wilks:1938dza}
S.~S. Wilks, \ifthenelse{\boolean{articletitles}}{\emph{{The large-sample
  distribution of the likelihood ratio for testing composite hypotheses}},
  }{}\href{https://doi.org/10.1214/aoms/1177732360}{Ann.\ Math.\ Stat.\
  \textbf{9} (1938) 60}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{DelFabbro:2004ta}
A.~Del~Fabbro, D.~Janc, M.~Rosina, and D.~Treleani,
  \ifthenelse{\boolean{articletitles}}{\emph{{Production and detection of
  doubly charmed tetraquarks}},
  }{}\href{https://doi.org/10.1103/PhysRevD.71.014008}{Phys.\ Rev.\
  \textbf{D71} (2005) 014008},
  \href{http://arxiv.org/abs/hep-ph/0408258}{{\normalfont\ttfamily
  arXiv:hep-ph/0408258}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Bethe:1949yr}
H.~A. Bethe, \ifthenelse{\boolean{articletitles}}{\emph{{Theory of the
  effective range in nuclear scattering}},
  }{}\href{https://doi.org/10.1103/PhysRev.76.38}{Phys.\ Rev.\  \textbf{76}
  (1949) 38}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Balakrishnan:1997xyz}
N.~Balakrishnan, V.~Kharchenko, R.~C. Forrey, and A.~Dalgarno,
  \ifthenelse{\boolean{articletitles}}{\emph{Complex scattering lengths in
  multi\nobreakdash-channel atom\nobreakdash-molecule collisions},
  }{}\href{https://doi.org/10.1016/S0009-2614(97)01052-X}{Chemical Physics
  Letters \textbf{280} (1997) 5}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Weinberg:1965zz}
S.~Weinberg, \ifthenelse{\boolean{articletitles}}{\emph{{Evidence that
  the~deuteron is not an~elementary particle}},
  }{}\href{https://doi.org/10.1103/PhysRev.137.B672}{Phys.\ Rev.\  \textbf{137}
  (1965) B672}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Matuschek:2020gqe}
I.~Matuschek, V.~Baru, F.-K. Guo, and C.~Hanhart,
  \ifthenelse{\boolean{articletitles}}{\emph{{On the nature of near-threshold
  bound and virtual states}},
  }{}\href{https://doi.org/10.1140/epja/s10050-021-00413-y}{Eur.\ Phys.\ J.\
  \textbf{A57} (2021) 101},
  \href{http://arxiv.org/abs/2007.05329}{{\normalfont\ttfamily
  arXiv:2007.05329}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-023}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Modification of $\chicone(3872)$
  and $\psitwos$ production in $\proton\proton$~collisions at $\sqrt{s}=
  8\tev$}}, }{}\href{https://doi.org/10.1103/PhysRevLett.126.092001}{Phys.\
  Rev.\ Lett.\  \textbf{126} (2021) 092001},
  \href{http://arxiv.org/abs/2009.06619}{{\normalfont\ttfamily
  arXiv:2009.06619}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{DPSBOOK}
I.~Belyaev and D.~Savrina, \ifthenelse{\boolean{articletitles}}{\emph{{Study of
  double parton scattering processes with heavy quarks}}, }{} in {\em {Multiple
  parton interactions at the LHC}} (P.~Bartalini and J.~R. Gaunt, eds.).
\newblock World Scientific, Singapore, 2018.
\newblock \href{http://arxiv.org/abs/1711.10877}{{\normalfont\ttfamily
  arXiv:1711.10877}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2012-003}
M.~Adinolfi {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Performance of the \lhcb RICH
  detector at the LHC}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-013-2431-9}{Eur.\ Phys.\ J.\
  \textbf{C73} (2013) 2431},
  \href{http://arxiv.org/abs/1211.6759}{{\normalfont\ttfamily
  arXiv:1211.6759}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Sjostrand:2007gs}
T.~Sj\"{o}strand, S.~Mrenna, and P.~Skands,
  \ifthenelse{\boolean{articletitles}}{\emph{{A brief introduction to
  {\sc{PYTHIA\,8.1}}}},
  }{}\href{https://doi.org/10.1016/j.cpc.2008.01.036}{Comput.\ Phys.\ Commun.\
  \textbf{178} (2008) 852},
  \href{http://arxiv.org/abs/0710.3820}{{\normalfont\ttfamily
  arXiv:0710.3820}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PROC-2010-056}
I.~Belyaev {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Handling
  of the~generation of primary events in {\sc{Gauss}}, the~LHCb simulation
  framework}}, }{}\href{https://doi.org/10.1088/1742-6596/331/3/032047}{J.\
  Phys.\ Conf.\ Ser.\  \textbf{331} (2011) 032047}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lange:2001uf}
D.~J. Lange, \ifthenelse{\boolean{articletitles}}{\emph{{The {\sc{EvtGen}}
  particle decay simulation package}},
  }{}\href{https://doi.org/10.1016/S0168-9002(01)00089-4}{Nucl.\ Instrum.\
  Meth.\  \textbf{A462} (2001) 152}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{davidson2015photos}
N.~Davidson, T.~Przedzinski, and Z.~Was,
  \ifthenelse{\boolean{articletitles}}{\emph{{{\sc{PHOTOS}} interface in C++:
  Technical and physics documentation}},
  }{}\href{https://doi.org/https://doi.org/10.1016/j.cpc.2015.09.013}{Comp.\
  Phys.\ Comm.\  \textbf{199} (2016) 86},
  \href{http://arxiv.org/abs/1011.0937}{{\normalfont\ttfamily
  arXiv:1011.0937}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Allison:2006ve}
Geant4 collaboration, J.~Allison {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{{\sc{Geant4}} developments and
  applications}}, }{}\href{https://doi.org/10.1109/TNS.2006.869826}{IEEE
  Trans.\ Nucl.\ Sci.\  \textbf{53} (2006) 270}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Agostinelli:2002hh}
Geant4 collaboration, S.~Agostinelli {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{{\sc{Geant4}}: A~simulation
  toolkit}}, }{}\href{https://doi.org/10.1016/S0168-9002(03)01368-8}{Nucl.\
  Instrum.\ Meth.\  \textbf{A506} (2003) 250}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PROC-2011-006}
M.~Clemencic {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{The
  \lhcb simulation application, {\sc{Gauss}}: Design, evolution and
  experience}}, }{}\href{https://doi.org/10.1088/1742-6596/331/3/032023}{J.\
  Phys.\ Conf.\ Ser.\  \textbf{331} (2011) 032023}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Hulsbergen:2005pu}
W.~D. Hulsbergen, \ifthenelse{\boolean{articletitles}}{\emph{{Decay chain
  fitting with a Kalman filter}},
  }{}\href{https://doi.org/10.1016/j.nima.2005.06.078}{Nucl.\ Instrum.\ Meth.\
  \textbf{A552} (2005) 566},
  \href{http://arxiv.org/abs/physics/0503191}{{\normalfont\ttfamily
  arXiv:physics/0503191}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Pivk:2004ty}
M.~Pivk and F.~R. Le~Diberder,
  \ifthenelse{\boolean{articletitles}}{\emph{{sPlot: A statistical tool to
  unfold data distributions}},
  }{}\href{https://doi.org/10.1016/j.nima.2005.08.106}{Nucl.\ Instrum.\ Meth.\
  \textbf{A555} (2005) 356},
  \href{http://arxiv.org/abs/physics/0402083}{{\normalfont\ttfamily
  arXiv:physics/0402083}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Rosner:1980bd}
J.~L. Rosner, \ifthenelse{\boolean{articletitles}}{\emph{{Quark models}},
  }{}\href{https://doi.org/10.1007/978-1-4684-3938-0_1}{NATO Sci.\ Ser.\ B
  \textbf{66} (1981) 1}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Gasiorowicz:1981jz}
S.~Gasiorowicz and J.~L. Rosner,
  \ifthenelse{\boolean{articletitles}}{\emph{{Hadron spectra and quarks}},
  }{}\href{https://doi.org/10.1119/1.12597}{Am.\ J.\ Phys.\  \textbf{49} (1981)
  954}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Rosner_2013}
J.~L. Rosner, \ifthenelse{\boolean{articletitles}}{\emph{{Hadronic and
  radiative $\Dstar$ widths}},
  }{}\href{https://doi.org/10.1103/physrevd.88.034034}{Phys.\ Rev.\
  \textbf{D88} (2013) 034034},
  \href{http://arxiv.org/abs/1307.2550}{{\normalfont\ttfamily
  arXiv:1307.2550}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Peskin:1995ev}
M.~E. Peskin and D.~V. Schroeder, {\em {An introduction to quantum field
  theory}}, Addison-Wesley, Reading, USA, 1995\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Gribov:2009zz}
V.~N. Gribov, {\em {Strong interactions of hadrons at high energies: Gribov
  lectures on Theoretical Physics}}, Cambridge University Press, 2012\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Martin:102663}
A.~D. Martin and T.~D. Spearman, {\em {Elementary-particle theory}},
  North-Holland, Amsterdam, 1970\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Eden:1966dnq}
R.~J. Eden, P.~V. Landshoff, D.~I. Olive, and J.~C. Polkinghorne, {\em {The
  analytic S-matrix}}, Cambridge Univ. Press, Cambridge, 1966\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Aitchison:1972ay}
I.~J.~R. Aitchison, \ifthenelse{\boolean{articletitles}}{\emph{{K-matrix
  formalism for overlapping resonances}},
  }{}\href{https://doi.org/10.1016/0375-9474(72)90305-3}{Nucl.\ Phys.\
  \textbf{A189} (1972) 417}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Mikhasenko:2018bzm}
JPAC collaboration, M.~Mikhasenko {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Pole position of
  the~$\Pa_1(1260)$ from $\Ptau$-decay}},
  }{}\href{https://doi.org/10.1103/PhysRevD.98.096021}{Phys.\ Rev.\
  \textbf{D98} (2018) 096021},
  \href{http://arxiv.org/abs/1810.00016}{{\normalfont\ttfamily
  arXiv:1810.00016}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Karliner:2019lau}
M.~Karliner and J.~L. Rosner,
  \ifthenelse{\boolean{articletitles}}{\emph{{Status of isospin splittings in
  mesons and baryons}},
  }{}\href{https://doi.org/10.1103/PhysRevD.100.073006}{Phys.\ Rev.\
  \textbf{D100} (2019) 073006},
  \href{http://arxiv.org/abs/1906.07799}{{\normalfont\ttfamily
  arXiv:1906.07799}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\end{mcitethebibliography}


==> refs_main.tex <==

\ifx\mcitethebibliography\mciteundefinedmacro
\PackageError{LHCb.bst}{mciteplus.sty has not been loaded}
{This bibstyle requires the use of the mciteplus package.}\fi
\providecommand{\href}[2]{#2}
\begin{mcitethebibliography}{100}
\mciteSetBstSublistMode{n}
\mciteSetBstMaxWidthForm{subitem}{\alph{mcitesubitemcount})}
\mciteSetBstSublistLabelBeginEnd{\mcitemaxwidthsubitemform\space}
{\relax}{\relax}


\bibitem{GellMann:1964nj}
M.~Gell-Mann, \ifthenelse{\boolean{articletitles}}{\emph{{A~schematic model of
  baryons and mesons}},
  }{}\href{https://doi.org/10.1016/S0031-9163(64)92001-3}{Phys.\ Lett.\
  \textbf{8} 214--215} (1964)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Zweig:352337}
G.~Zweig, \ifthenelse{\boolean{articletitles}}{\emph{{An SU$_3$ model for
  strong interaction symmetry and its breaking; Version 1,}}, }{} Tech. Rep.
  \href{http://cds.cern.ch/record/352337}{CERN-TH-401}, CERN, Geneva,
  1964\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Zweig:570209}
G.~Zweig, \ifthenelse{\boolean{articletitles}}{\emph{{An SU$_3$ model for
  strong interaction symmetry and its breaking; Version 2,}}, }{} Tech. Rep.
  \href{http://cds.cern.ch/record/570209}{CERN-TH-412}, CERN, Geneva,
  1964\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Jaffe:1976ig}
R.~L. Jaffe, \ifthenelse{\boolean{articletitles}}{\emph{{Multiquark hadrons. I.
  Phenomenology of $\PQ^2\bar{\PQ}^2$~mesons}},
  }{}\href{https://doi.org/10.1103/PhysRevD.15.267}{Phys.\ Rev.\  \textbf{D15}
  267--280} (1977)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Jaffe:1976ih}
R.~L. Jaffe, \ifthenelse{\boolean{articletitles}}{\emph{{Multi-quark hadrons.
  2.~Methods}}, }{}\href{https://doi.org/10.1103/PhysRevD.15.281}{Phys.\ Rev.\
  \textbf{D15} 281--289} (1977)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Rossi:1977cy}
G.~C. Rossi and G.~Veneziano,
  \ifthenelse{\boolean{articletitles}}{\emph{{A~possible description of baryon
  dynamics in dual and gauge theories}},
  }{}\href{https://doi.org/10.1016/0550-3213(77)90178-X}{Nucl.\ Phys.\
  \textbf{B123} 507--545} (1977)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Jaffe:1977cv}
R.~L. Jaffe, \ifthenelse{\boolean{articletitles}}{\emph{{
  $\PQ^2\bar{\PQ}^2$~resonances in the~baryon\nobreakdash-antibaryon system}},
  }{}\href{https://doi.org/10.1103/PhysRevD.17.1444}{Phys.\ Rev.\  \textbf{D17}
  1444--1458} (1978)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lipkin:1987sk}
H.~J. Lipkin, \ifthenelse{\boolean{articletitles}}{\emph{{New~possibilities for
  exotic hadrons - anticharmed strange baryons}},
  }{}\href{https://doi.org/10.1016/0370-2693(87)90055-4}{Phys.\ Lett.\
  \textbf{B195} 484--488} (1987)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Choi:2003ue}
Belle collaboration, S.~K. Choi {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~narrow
  charmoniumlike state in exclusive
  \mbox{$\decay{\B^{\pm}}{\kaon^{\pm}\pip\pim\jpsi}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.91.262001}{Phys.\ Rev.\ Lett.\
  \textbf{91} 262001} (2003)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Choi:2007wga}
Belle collaboration, S.~K. Choi {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~resonancelike
  structure in the~\mbox{$\Ppi^\pm\Ppsi^\prime$}~mass distribution in exclusive
  \mbox{$\decay{\B}{\kaon\Ppi^{\pm}\Ppsi^{\prime}}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.100.142001}{Phys.\ Rev.\ Lett.\
  \textbf{100} 142001} (2008)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Belle:2008qeq}
Belle collaboration, R.~Mizuk {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of two
  resonance\nobreakdash-like structures in the~\mbox{$\pip\chicone$}~mass
  distribution in exclusive \mbox{$\decay{\Bdb}{\Km\pip\chicone}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevD.78.072004}{Phys.\ Rev.\
  \textbf{D78} 072004} (2008)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Aaltonen:2009tz}
CDF collaboration, T.~Aaltonen {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for a~narrow
  near\nobreakdash-threshold structure in the~$\jpsi\Pphi$~mass spectrum in
  \mbox{$\decay{\Bu}{\jpsi\Pphi\Kp}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.102.242002}{Phys.\ Rev.\ Lett.\
  \textbf{102} 242002} (2009)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Belle:2011aa}
Belle collaboration, A.~Bondar {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of two charged
  bottomonium\nobreakdash-like resonances in $\PUpsilon(5\PS)$~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.108.122001}{Phys.\ Rev.\ Lett.\
  \textbf{108} 122001} (2012)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ablikim:2013mio}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~charged
  charmoniumlike structure in \mbox{$\decay{\epem}{\pip\pim\jpsi}$} at
  \mbox{$\sqs=4.26\gev$} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.110.252001}{Phys.\ Rev.\ Lett.\
  \textbf{110} 252001} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{BESIII:2013ouc}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~charged
  charmoniumlike structure \mbox{$\Z_{\cquark}(4020)$} and search for
  the~\mbox{$Z_{\cquark}(3900)$} in
  \mbox{$\decay{\epem}{\pip\pim\Ph_{\cquark}}$} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.111.242001}{Phys.\ Rev.\ Lett.\
  \textbf{111} 242001} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{BESIII:2013mhi}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~charged
  charmoniumlike structure in
  \mbox{$\decay{\epem}{\left(\Dstar\Dstarb\right)^{\pm}\pion^{\mp}}$}
  at~\mbox{$\sqs=4.26\gev$} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.112.132001}{Phys.\ Rev.\ Lett.\
  \textbf{112} 132001} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Abazov:2013xda}
D0 collaboration, V.~M. Abazov {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Search for the~$\PX(4140)$~state
  in \mbox{$\decay{\Bu}{\jpsi\Pphi\Kp}$}~decays with the D0 Detector}},
  }{}\href{https://doi.org/10.1103/PhysRevD.89.012004}{Phys.\ Rev.\
  \textbf{D89} 012004} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Chatrchyan:2013dma}
CMS collaboration, S.~Chatrchyan {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~peaking
  structure in the~$\jpsi\Pphi$~mass spectrum from
  $\decay{\Bu}{\jpsi\Pphi\Kp}$~decays}},
  }{}\href{https://doi.org/10.1016/j.physletb.2014.05.055}{Phys.\ Lett.\
  \textbf{B734} 261--281} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Chilikin:2013tch}
Belle collaboration, K.~Chilikin {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Experimental constraints on the
  spin and parity of the~\mbox{$\Z\mathrm{(4430)}^+$}}},
  }{}\href{https://doi.org/10.1103/PhysRevD.88.074026}{Phys.\ Rev.\
  \textbf{D88} 074026} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Belle:2013yex}
Belle collaboration, Z.~Q. Liu {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of
  \mbox{$\decay{\epem}{\pip\pim\jpsi}$} and observation of a~charged
  charmoniumlike state at Belle}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.110.252002}{Phys.\ Rev.\ Lett.\
  \textbf{110} 252002} (2013), Erratum
  \href{https://doi.org/10.1103/PhysRevLett.111.019901}{ibid.\   \textbf{111}
  019901} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Chilikin:2014bkk}
Belle collaboration, K.~Chilikin {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~new charged
  charmoniumlike state in \mbox{$\decay{\Bdb}{\jpsi\Km\pip}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevD.90.112009}{Phys.\ Rev.\
  \textbf{D90} 112009} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2014-014}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of the resonant
  character of the~\mbox{$\PZ(4430)^-$}~state}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.112.222002}{Phys.\ Rev.\ Lett.\
  \textbf{112} 222002} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2015-029}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of $\jpsi\proton$
  resonances consistent with pentaquark states in
  \mbox{\decay{\Lb}{\jpsi\proton\Km}} decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.115.072001}{Phys.\ Rev.\ Lett.\
  \textbf{115} 072001} (2015)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2015-038}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Model-independent confirmation of
  the~\mbox{$\Z(4430)^-$}~state}},
  }{}\href{https://doi.org/10.1103/PhysRevD.92.112009}{Phys.\ Rev.\
  \textbf{D92} 112009} (2015)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2016-018}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of exotic
  $\jpsi\Pphi$~structures from amplitude analysis of
  \mbox{\decay{\Bp}{\jpsi\Pphi\Kp}} decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.118.022003}{Phys.\ Rev.\ Lett.\
  \textbf{118} 022003} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2016-019}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Amplitude analysis of
  \mbox{\decay{\Bp}{\jpsi\Pphi\Kp}} decays}},
  }{}\href{https://doi.org/10.1103/PhysRevD.95.012002}{Phys.\ Rev.\
  \textbf{D95} 012002} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2018-034}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for
  a~\mbox{$\Peta_\cquark(1\PS) \pim$}~resonance in
  \mbox{\decay{\Bz}{\Peta_\cquark(1\PS) \Kp\pim}} decays}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-018-6447-z}{Eur.\ Phys.\ J.\
  \textbf{C78} 1019} (2018)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2019-014}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~narrow
  pentaquark state, $\PP_\cquark(4312)^+$, and of two-peak structure of
  the~$\PP_\cquark(4450)^+$}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.122.222001}{Phys.\ Rev.\ Lett.\
  \textbf{122} 222001} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-011}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of structure in the
  \jpsi-pair mass spectrum}},
  }{}\href{https://doi.org/10.1016/j.scib.2020.08.032}{Science Bulletin
  \textbf{65} 1983--1993} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-024}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Model\nobreakdash-independent
  study of structure in \mbox{$\decay{\Bp}{\Dp \Dm \Kp}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.125.242001}{Phys.\ Rev.\ Lett.\
  \textbf{125} 242001} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-025}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Amplitude analysis of
  the~\mbox{$\decay{\Bp}{\Dp \Dm \Kp}$}~decay}},
  }{}\href{https://doi.org/10.1103/PhysRevD.102.112003}{Phys.\ Rev.\
  \textbf{D102} 112003} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-035}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of \mbox{$\decay{\Bs}{\jpsi
  \pip \pim \Kp \Km}$}~decays}},
  }{}\href{https://doi.org/10.1007/JHEP02(2021)024}{JHEP \textbf{02} 024}
  (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-039}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence of a $\jpsi\Lz$
  structure and observation of excited $\Xim$ states in the $\Xibm \rightarrow
  \jpsi \Lz \Km$ decay}},
  }{}\href{https://doi.org/10.1016/j.scib.2021.02.030}{Science Bulletin
  \textbf{66} 1278--1287} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-044}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of new resonances
  decaying into \mbox{$\jpsi\Kp$} and \mbox{$\jpsi\Pphi$}}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.127.082001}{Phys.\ Rev.\ Lett.\
  \textbf{127} 082001} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ablikim_2021}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of
  a~near\nobreakdash-threshold structure in the~\Kp recoil\nobreakdash-mass
  spectra in \mbox{$\decay{\epem}{\Kp\left(\Dsm \Dstarz +
  \D^{*-}_{\squark}\Dz\right) } $} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.126.102001}{Phys.\ Rev.\ Lett.\
  \textbf{126} 102001} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2021-018}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for a~new structure in
  the~$\jpsi\proton$ and $\jpsi\antiproton$~systems
  in~\mbox{$\decay{\Bs}{\jpsi\proton\antiproton}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.128.062001}{Phys.\ Rev.\ Lett.\
  \textbf{128} 062001} (2022)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Brambilla:2019esw}
N.~Brambilla {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{The
  $\PX\PY\PZ$~states: experimental and theoretical status and perspectives}},
  }{}\href{https://doi.org/10.1016/j.physrep.2020.05.001}{Phys.\ Rept.\
  \textbf{873} 1--154} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{PDG2021}
Particle Data Group, P.~A. Zyla {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{\href{http://pdg.lbl.gov/}{Review
  of particle physics}}}, }{}\href{https://doi.org/10.1093/ptep/ptaa104}{Prog.\
  Theor.\ Exp.\ Phys.\  \textbf{2020} 083C01} (2020), and
  {\href{http://pdglive.lbl.gov/}{2021 update
  {\tt{http:/pdglive.lbl.gov}}}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Oset:2019upy}
E.~Oset {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Tetra and
  pentaquarks from the molecular perspective}},
  }{}\href{https://doi.org/10.1051/epjconf/201919901003}{EPJ Web Conf.\
  \textbf{199} 01003} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Richard_2016}
J.-M. Richard, \ifthenelse{\boolean{articletitles}}{\emph{Exotic hadrons:
  Review and perspectives},
  }{}\href{https://doi.org/10.1007/s00601-016-1159-0}{Few-Body Systems
  \textbf{57} 1185--1212} (2016)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Guo:2017jvc}
F.-K. Guo {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Hadronic
  molecules}}, }{}\href{https://doi.org/10.1103/RevModPhys.90.015004}{Rev.\
  Mod.\ Phys.\  \textbf{90} 015004} (2018)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{MartinezTorres:2020hus}
A.~Martinez~Torres, K.~P. Khemchandani, L.~Roca, and E.~Oset,
  \ifthenelse{\boolean{articletitles}}{\emph{{Few-body systems consisting of
  mesons}}, }{}\href{https://doi.org/10.1007/s00601-020-01568-y}{Few Body
  Syst.\  \textbf{61} 35} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ali:2019roi}
A.~Ali, L.~Maiani, and A.~D. Polosa, {\em {Multiquark Hadrons}},
  \href{https://doi.org/10.1017/9781316761465}{ Cambridge University Press,
  2019}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ader:1981db}
J.~P. Ader, J.-M. Richard, and P.~Taxil,
  \ifthenelse{\boolean{articletitles}}{\emph{{Do narrow heavy multiquark states
  exist?}}, }{}\href{https://doi.org/10.1103/PhysRevD.25.2370}{Phys.\ Rev.\
  \textbf{D25} 2370--2382} (1982)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ballot:1983iv}
J.~l. Ballot and J.~M. Richard,
  \ifthenelse{\boolean{articletitles}}{\emph{{Four quark states in additive
  potentials}}, }{}\href{https://doi.org/10.1016/0370-2693(83)90991-7}{Phys.\
  Lett.\  \textbf{B123} 449--451} (1983)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Zouzou:1986qh}
S.~Zouzou, B.~Silvestre-Brac, C.~Gignoux, and J.~M. Richard,
  \ifthenelse{\boolean{articletitles}}{\emph{{Four quark bound states}},
  }{}\href{https://doi.org/10.1007/BF01557611}{Z.\ Phys.\  \textbf{C30}
  457--468} (1986)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lipkin:1986dw}
H.~J. Lipkin, \ifthenelse{\boolean{articletitles}}{\emph{{A~model-independent
  approach to multiquark bound states}},
  }{}\href{https://doi.org/10.1016/0370-2693(86)90843-9}{Phys.\ Lett.\
  \textbf{B172} 242--247} (1986)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Heller:1986bt}
L.~Heller and J.~A. Tjon, \ifthenelse{\boolean{articletitles}}{\emph{{On
  the~existence of stable dimesons}},
  }{}\href{https://doi.org/10.1103/PhysRevD.35.969}{Phys.\ Rev.\  \textbf{D35}
  969--974} (1987)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Manohar:1992nd}
A.~V. Manohar and M.~B. Wise,
  \ifthenelse{\boolean{articletitles}}{\emph{{Exotic
  $\PQ\PQ\bar{\Pq}\bar{\Pq}$~states in QCD}},
  }{}\href{https://doi.org/10.1016/0550-3213(93)90614-U}{Nucl.\ Phys.\
  \textbf{B399} 17--33} (1993)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2017-018}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of the~doubly charmed
  baryon \Xiccpp}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.119.112001}{Phys.\ Rev.\ Lett.\
  \textbf{119} 112001} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2018-026}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{First observation of the~doubly
  charmed baryon decay \mbox{\decay{\Xiccpp}{\Xires_c^+\pip}}}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.121.162002}{Phys.\ Rev.\ Lett.\
  \textbf{121} 162002} (2018)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2019-037}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Precision measurement of the
  $\Xiccpp$ mass}}, }{}\href{https://doi.org/10.1007/JHEP02(2020)049}{JHEP
  \textbf{02} 049} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Karliner:2017qjm}
M.~Karliner and J.~L. Rosner,
  \ifthenelse{\boolean{articletitles}}{\emph{{Discovery of doubly-charmed
  $\Xi_{\cquark\cquark}$ baryon implies a~stable \mbox{$\bquark\bquark
  \uquarkbar \dquarkbar$}~tetraquark}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.119.202001}{Phys.\ Rev.\ Lett.\
  \textbf{119} 202001} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Carlson:1987hh}
J.~Carlson, L.~Heller, and J.~A. Tjon,
  \ifthenelse{\boolean{articletitles}}{\emph{{Stability of dimesons}},
  }{}\href{https://doi.org/10.1103/PhysRevD.37.744}{Phys.\ Rev.\  \textbf{D37}
  744--753} (1988)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{SilvestreBrac:1993ss}
B.~Silvestre-Brac and C.~Semay,
  \ifthenelse{\boolean{articletitles}}{\emph{{Systematics of \mbox{$L = 0$}
  \mbox{$\quark^2\quarkbar^2$}~systems}},
  }{}\href{https://doi.org/10.1007/BF01565058}{Z.\ Phys.\  \textbf{C57}
  273--282} (1993)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Semay:1994ht}
C.~Semay and B.~Silvestre-Brac,
  \ifthenelse{\boolean{articletitles}}{\emph{{Diquonia and potential models}},
  }{}\href{https://doi.org/10.1007/BF01413104}{Z.\ Phys.\  \textbf{C61}
  271--275} (1994)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Moinester:1995fk}
M.~A. Moinester, \ifthenelse{\boolean{articletitles}}{\emph{{How to search for
  doubly charmed baryons and tetraquarks}},
  }{}\href{https://doi.org/10.1007/s002180050123}{Z.\ Phys.\  \textbf{A355}
  349--362} (1996)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Pepin:1996id}
S.~Pepin, F.~Stancu, M.~Genovese, and J.-M. Richard,
  \ifthenelse{\boolean{articletitles}}{\emph{{Tetraquarks with color blind
  forces in chiral quark models}},
  }{}\href{https://doi.org/10.1016/S0370-2693(96)01597-3}{Phys.\ Lett.\
  \textbf{B393} 119--123} (1997)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{GELMAN2003296}
B.~A. Gelman and S.~Nussinov, \ifthenelse{\boolean{articletitles}}{\emph{{Does
  a~narrow tetraquark $\cquark\cquark\uquarkbar\dquarkbar$~state exist?}},
  }{}\href{https://doi.org/10.1016/S0370-2693(02)03069-1}{Phys.\ Lett.\
  \textbf{B551} 296--304} (2003)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Vijande:2003ki}
J.~Vijande, F.~Fernandez, A.~Valcarce, and B.~Silvestre-Brac,
  \ifthenelse{\boolean{articletitles}}{\emph{{Tetraquarks in a chiral
  constituent quark model}},
  }{}\href{https://doi.org/10.1140/epja/i2003-10128-9}{Eur.\ Phys.\ J.\
  \textbf{A19} 383--389} (2004)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Janc:2004qn}
D.~Janc and M.~Rosina, \ifthenelse{\boolean{articletitles}}{\emph{{The
  $\PT_{\cquark\cquark} = \D\Dstar$ molecular state}},
  }{}\href{https://doi.org/10.1007/s00601-004-0068-9}{Few Body Syst.\
  \textbf{35} 175--196} (2004)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Navarra:2007yw}
F.~S. Navarra, M.~Nielsen, and S.~H. Lee,
  \ifthenelse{\boolean{articletitles}}{\emph{{QCD sum rules study of
  \mbox{$\PQ\PQ-\uquarkbar\dquarkbar$}~mesons}},
  }{}\href{https://doi.org/10.1016/j.physletb.2007.04.010}{Phys.\ Lett.\
  \textbf{B649} 166--172} (2007)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Vijande}
J.~Vijande, E.~Weissman, A.~Valcarce, and N.~Barnea,
  \ifthenelse{\boolean{articletitles}}{\emph{{Are there compact heavy
  four-quark bound states?}},
  }{}\href{https://doi.org/10.1103/PhysRevD.76.094027}{Phys.\ Rev.\
  \textbf{D76} 094027} (2007)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ebert:2007rn}
D.~Ebert, R.~N. Faustov, V.~O. Galkin, and W.~Lucha,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of tetraquarks with two
  heavy quarks in the~relativistic quark model}},
  }{}\href{https://doi.org/10.1103/PhysRevD.76.114015}{Phys.\ Rev.\
  \textbf{D76} 114015} (2007)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lee:2009rt}
S.~H. Lee and S.~Yasui, \ifthenelse{\boolean{articletitles}}{\emph{{Stable
  multiquark states with heavy quarks in a diquark model}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-009-1140-x}{Eur.\ Phys.\ J.\
  \textbf{C64} 283--295} (2009)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Yang2009}
Y.~Yang, C.~Deng, J.~Ping, and T.~Goldman,
  \ifthenelse{\boolean{articletitles}}{\emph{$\mathrm{S}$-wave
  $\mathrm{QQ}\quarkbar\quarkbar$ state in the~constituent quark model},
  }{}\href{https://doi.org/10.1103/PhysRevD.80.114023}{Phys.\ Rev.\
  \textbf{D80} 114023} (2009)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Li:2012ss}
N.~Li, Z.-F. Sun, X.~Liu, and S.-L. Zhu,
  \ifthenelse{\boolean{articletitles}}{\emph{{Coupled\nobreakdash-channel
  analysis of the~possible \mbox{$\D^{(*)}\D^{(*)}$},
  \mbox{$\Bbar^{(*)}\Bbar^{(*)}$} and \mbox{$\D^{(*)}\Bbar^{(*)}$}~molecular
  states}}, }{}\href{https://doi.org/10.1103/PhysRevD.88.114008}{Phys.\ Rev.\ D
  \textbf{88} 114008} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Feng:2013kea}
G.-Q. Feng, X.-H. Guo, and B.-S. Zou,
  \ifthenelse{\boolean{articletitles}}{\emph{{$\mathrm{QQ}^{\prime} \uquarkbar
  \dquarkbar$ bound state in the Bethe-Salpeter equation approach}},
  }{}\href{http://arxiv.org/abs/1309.7813}{{\normalfont\ttfamily
  arXiv:1309.7813}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Luo:2017eub}
S.-Q. Luo {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Exotic
  tetraquark states with the $\Pq\Pq\bar{\PQ}\bar{\PQ}$ configuration}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-017-5297-4}{Eur.\ Phys.\ J.\
  \textbf{C77} 709} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Eichten:2017ffp}
E.~J. Eichten and C.~Quigg,
  \ifthenelse{\boolean{articletitles}}{\emph{{Heavy-quark symmetry implies
  stable heavy tetraquark mesons $\PQ_i\PQ_j \bar \Pq_k \bar \Pq_l$}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.119.202002}{Phys.\ Rev.\ Lett.\
  \textbf{119} 202002} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Wang:2017uld}
Z.-G. Wang, \ifthenelse{\boolean{articletitles}}{\emph{{Analysis of
  the~axialvector doubly heavy tetraquark states with QCD sum rules}},
  }{}\href{https://doi.org/10.5506/APhysPolB.49.1781}{Acta Phys.\ Polon.\
  \textbf{B49} 1781--1800} (2018)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Park:2018wjk}
W.~Park, S.~Noh, and S.~H. Lee,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of the~doubly heavy
  tetraquarks in a~constituent quark model}},
  }{}\href{https://doi.org/10.1016/j.nuclphysa.2018.12.019}{Acta Phys.\ Polon.\
   \textbf{B50} 1151--1157} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Junnarkar:2018twb}
P.~Junnarkar, N.~Mathur, and M.~Padmanath,
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of doubly heavy tetraquarks
  in Lattice QCD}}, }{}\href{https://doi.org/10.1103/PhysRevD.99.034507}{Phys.\
  Rev.\  \textbf{D99} 034507} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Deng:2018kly}
C.~Deng, H.~Chen, and J.~Ping,
  \ifthenelse{\boolean{articletitles}}{\emph{{Systematical investigation on the
  stability of doubly heavy tetraquark states}},
  }{}\href{https://doi.org/10.1140/epja/s10050-019-00012-y}{Eur.\ Phys.\ J.\
  \textbf{A56} 9} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Liu:2019stu}
M.-Z. Liu {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Heavy\nobreakdash-quark spin and
  flavor symmetry partners of the~\mbox{$\PX(3872)$}~revisited: What can we
  learn from the~one boson exchange model?}},
  }{}\href{https://doi.org/10.1103/PhysRevD.99.094018}{Phys.\ Rev.\
  \textbf{D99} 094018} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Maiani:2019lpu}
L.~Maiani, A.~D. Polosa, and V.~Riquer,
  \ifthenelse{\boolean{articletitles}}{\emph{{Hydrogen bond of QCD in doubly
  heavy baryons and tetraquarks}},
  }{}\href{https://doi.org/10.1103/PhysRevD.100.074002}{Phys.\ Rev.\
  \textbf{D100} 074002} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Yang:2019itm}
G.~Yang, J.~Ping, and J.~Segovia,
  \ifthenelse{\boolean{articletitles}}{\emph{{Doubly-heavy tetraquarks}},
  }{}\href{https://doi.org/10.1103/PhysRevD.101.014001}{Phys.\ Rev.\
  \textbf{D101} 014001} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Tan:2020ldi}
Y.~Tan, W.~Lu, and J.~Ping,
  \ifthenelse{\boolean{articletitles}}{\emph{{$\PQ\PQ\bar{\Pq}\bar{\Pq}$ in
  a~chiral constituent quark model}},
  }{}\href{https://doi.org/10.1140/epjp/s13360-020-00741-w}{Eur.\ Phys.\ J.\
  Plus \textbf{135} 716} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lu:2020rog}
Q.-F. L\"u, D.-Y. Chen, and Y.-B. Dong,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of doubly heavy
  tetraquarks $\PT_{\PQ\PQ^\prime}$ in a relativized quark model}},
  }{}\href{https://doi.org/10.1103/PhysRevD.102.034012}{Phys.\ Rev.\
  \textbf{D102} 034012} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Braaten:2020nwp}
E.~Braaten, L.-P. He, and A.~Mohapatra,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of doubly heavy
  tetraquarks with error bars}},
  }{}\href{https://doi.org/10.1103/PhysRevD.103.016001}{Phys.\ Rev.\
  \textbf{D103} 016001} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Gao:2020ogo}
D.~Gao {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Masses of
  doubly heavy tetraquark states with isospin = $\frac{1}{2}$ and $1$ and
  spin\nobreakdash-parity~$1^{+\pm}$}},
  }{}\href{http://arxiv.org/abs/2007.15213}{{\normalfont\ttfamily
  arXiv:2007.15213}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Cheng:2020wxa}
J.-B. Cheng {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Double-heavy tetraquark states
  with heavy diquark\nobreakdash-antiquark symmetry}},
  }{}\href{https://doi.org/10.1088/1674-1137/abde2f}{Chin.\ Phys.\ C
  \textbf{45} 043102} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Noh:2021lqs}
S.~Noh, W.~Park, and S.~H. Lee,
  \ifthenelse{\boolean{articletitles}}{\emph{Doubly heavy tetraquarks,
  ${\Pq}{\Pq}^{\prime}\bar{\PQ}\bar{\PQ}^{\prime}$, in a~nonrelativistic quark
  model with a~complete set of harmonic oscillator bases},
  }{}\href{https://doi.org/10.1103/physrevd.103.114009}{Phys.\ Rev.\
  \textbf{D103} 114009} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Faustov:2021hjs}
R.~N. Faustov, V.~O. Galkin, and E.~M. Savchenko,
  \ifthenelse{\boolean{articletitles}}{\emph{{Heavy tetraquarks in
  the~relativistic quark model}},
  }{}\href{https://doi.org/10.3390/universe7040094}{Universe \textbf{7} 94}
  (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ikeda:2013vwa}
Y.~Ikeda {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Charmed
  tetraquarks $\PT_{\cquark\cquark}$ and $\PT_{\cquark\squark}$ from dynamical
  lattice QCD simulations}},
  }{}\href{https://doi.org/10.1016/j.physletb.2014.01.002}{Phys.\ Lett.\
  \textbf{B729} 85--90} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Cheung:2017tnt}
Hadron Spectrum collaboration, G.~K.~C. Cheung, C.~E. Thomas, J.~J. Dudek, and
  R.~G. Edwards, \ifthenelse{\boolean{articletitles}}{\emph{{Tetraquark
  operators in lattice QCD and exotic flavour states in the charm sector}},
  }{}\href{https://doi.org/10.1007/JHEP11(2017)033}{JHEP \textbf{11} 033}
  (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Francis:2018jyb}
A.~Francis, R.~J. Hudspith, R.~Lewis, and K.~Maltman,
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for charm-bottom
  tetraquarks and the mass dependence of heavy-light tetraquark states from
  lattice QCD}}, }{}\href{https://doi.org/10.1103/PhysRevD.99.054505}{Phys.\
  Rev.\  \textbf{D99} 054505} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2008-001}
LHCb collaboration, A.~A. Alves~Jr.\ {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{The \lhcb detector at the LHC}},
  }{}\href{https://doi.org/10.1088/1748-0221/3/08/S08005}{JINST \textbf{3}
  S08005} (2008)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2014-002}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{LHCb detector performance}},
  }{}\href{https://doi.org/10.1142/S0217751X15300227}{Int.\ J.\ Mod.\ Phys.\
  \textbf{A30} 1530022} (2015)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2012-003}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of double charm
  production involving open charm in \proton\proton collisions at
  \mbox{$\sqs=$7\tev}}}, }{}\href{https://doi.org/10.1007/JHEP06(2012)141}{JHEP
  \textbf{06} 141} (2012), Addendum
  \href{https://doi.org/10.1007/JHEP03(2014)108}{ibid.\   \textbf{03} 108}
  (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2021-032}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of a~doubly charmed
  tetraquark state}},
  }{}\href{http://arxiv.org/abs/2109.01056}{{\normalfont\ttfamily
  arXiv:2109.01056}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-008}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of the~line shape of
  the~$\chicone(3872)$~state}},
  }{}\href{https://doi.org/10.1103/PhysRevD.102.092005}{Phys.\ Rev.\
  \textbf{D102} 092005} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-009}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of the $\psires_2(3823)$
  and $\chicone(3872)$~states in \mbox{$\decay{\Bu}{ \left(
  \jpsi\pip\pim\right)\Kp}$}~decays}},
  }{}\href{https://doi.org/10.1007/JHEP08(2020)123}{JHEP \textbf{08} 123}
  (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2013-011}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Precision measurement of \D meson
  mass differences}}, }{}\href{https://doi.org/10.1007/JHEP06(2013)065}{JHEP
  \textbf{06} 065} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\end{mcitethebibliography}


==> refs_methods.tex <==
\ifx\mcitethebibliography\mciteundefinedmacro
\PackageError{LHCb.bst}{mciteplus.sty has not been loaded}
{This bibstyle requires the use of the mciteplus package.}\fi
\providecommand{\href}[2]{#2}
\begin{mcitethebibliography}{100}
\mciteSetBstSublistMode{n}
\mciteSetBstMaxWidthForm{subitem}{\alph{mcitesubitemcount})}
\mciteSetBstSublistLabelBeginEnd{\mcitemaxwidthsubitemform\space}
{\relax}{\relax}

\bibitem{LHCb-DP-2012-003}
M.~Adinolfi {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Performance of the \lhcb RICH
  detector at the LHC}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-013-2431-9}{Eur.\ Phys.\ J.\
  \textbf{C73} 2431} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PROC-2010-056}
I.~Belyaev {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Handling
  of the generation of primary events in {\sc{Gauss}}, the LHCb simulation
  framework}}, }{}\href{https://doi.org/10.1088/1742-6596/331/3/032047}{J.\
  Phys.\ Conf.\ Ser.\  \textbf{331} 032047} (2011)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lange:2001uf}
D.~J. Lange, \ifthenelse{\boolean{articletitles}}{\emph{{The~{\sc{EvtGen}}
  particle decay simulation package}},
  }{}\href{https://doi.org/10.1016/S0168-9002(01)00089-4}{Nucl.\ Instrum.\
  Meth.\  \textbf{A462} 152--155} (2001)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PROC-2011-006}
M.~Clemencic {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{The
  \lhcb simulation application, {\sc{Gauss}}: Design, evolution and
  experience}}, }{}\href{https://doi.org/10.1088/1742-6596/331/3/032023}{J.\
  Phys.\ Conf.\ Ser.\  \textbf{331} 032023} (2011)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Hulsbergen:2005pu}
W.~D. Hulsbergen, \ifthenelse{\boolean{articletitles}}{\emph{{Decay chain
  fitting with a Kalman filter}},
  }{}\href{https://doi.org/10.1016/j.nima.2005.06.078}{Nucl.\ Instrum.\ Meth.\
  \textbf{A552} 566--575} (2005)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Pivk:2004ty}
M.~Pivk and F.~R. Le~Diberder,
  \ifthenelse{\boolean{articletitles}}{\emph{{sPlot: A statistical tool to
  unfold data distributions}},
  }{}\href{https://doi.org/10.1016/j.nima.2005.08.106}{Nucl.\ Instrum.\ Meth.\
  \textbf{A555} 356--369} (2005)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\end{mcitethebibliography}


==> selection.tex <==
\subsection*{Event selection}\label{sec:selection}


%The~\Dz, \Dp and \Dstarp~mesons are reconstructed in decay channels \mbox{$\decay{\Dz}{\Km\pip}$}, \mbox{$\decay{\Dp}{\Km\pip\pip}$} and  \mbox{$\decay{\Dstarp}{\Dz\pip}$} correspondingly.
%% The~selection  of~\Dp~and~\Dz~mesons largely follows 
%% the~one used in  
%% Refs.~\cite{LHCb-PAPER-2012-003,LHCb-PAPER-2013-062,LHCb-PAPER-2015-046,LHCb-PAPER-2019-005}
%% and is shortly summarized in this  section.
%%
The~$\Dz\Dz$, $\Dz\Dp$ and $\Dz\Dz\pip$ final states 
are reconstructed using the
\mbox{$\decay{\Dz}{\Km\pip}$} and 
\mbox{$\decay{\Dp}{\Km\pip\pip}$}~decay channels. 
The~selection criteria are similar to those used in 
Refs.\mbox{\cite{LHCb-PAPER-2012-003,
LHCb-PAPER-2013-062,
LHCb-PAPER-2015-046,
LHCb-PAPER-2019-005}}. 
Kaons and pions are selected from well\nobreakdash-reconstructed tracks
within the acceptance of the~spectrometer that are identified using information from
the~ring-imaging Cherenkov detectors.
%%
The~kaon and pion candidates that have transverse momenta larger than $250\mevc$ 
and are inconsistent with being produced at a~$\proton\proton$~interaction 
vertex are combined together to form $\Dz$ and $\Dp$ candidates, 
referred to as \D~hereafter. The~resulting $\D$ candidates are required to have 
good vertex quality,
mass within $\pm 65\mevcc$ and $\pm 50\mevcc$ 
of the~known \Dz and \Dp masses~\cite{PDG2021}, respectively, 
transverse momentum larger than $1\gevc$, 
decay time larger than $100\mum/c$ and 
a~momentum  direction that is consistent 
with the~vector from the~primary to~secondary vertex. 
Selected \Dz and \Dp~candidates 
consistent with originating 
from a~common primary vertex 
are combined to 
form $\Dz\Dz$ and $\Dz\Dp$ candidates. 
The~resulting $\Dz\Dz$ candidates are
combined with a~pion to form $\Dz\Dz\pip$~candidates.
For~those, at~least one out of the two $\Dz\pip$ 
combinations is required to have good vertex quality and mass 
not exceeding the known $\Dstarp$ mass by more than $155\mevcc$.
%%
For~each $\Dz\Dz$, $\Dz\Dp$ and $\Dz\Dz\pip$ candidate 
a~kinematic fit~\cite{Hulsbergen:2005pu} is performed.
This~fit 
constrains the mass of the $\D$ candidates to their known values and 
requires both $\D$ mesons, 
and a~pion in the case of $\Dz\Dz\pip$,
to originate from the~same primary vertex.
%%  
A~requirement is applied to the~quality
of this fit to further suppress combinatorial background 
and reduce 
the~background from $\D$~candidates produced 
in two independent $\proton\proton$~interactions or 
in the~decays of beauty hadrons~\cite{LHCb-PAPER-2012-003}.
%%
To~suppress background from kaon and pion candidates reconstructed from 
one common track, all track pairs of the~same charge are required to have 
an opening angle inconsistent with being zero 
and the mass of the~combination must be inconsistent with the~sum 
of the masses of the~two constituents.
%
For cross-checks additional final states 
$\Dp\Dp$, $\Dp\Dz\pip$,
$\Dz\Dzb$, $\Dz\Dm$ and $\Dzb\Dz\pip$ are 
reconstructed, selected and treated in the~same way.

\subsection*{Non\nobreakdash-\D background subtraction}
Two-dimensional distributions 
of the~mass of one \D~candidate versus
the~mass of the other \D~candidate from selected $\Dz\Dz\pip$, 
$\Dz\Dz$ and $\Dz\Dp$~combinations
are shown in Extended Data Fig.~\ref{fig:DATA_2D}.
These distributions illustrate the relatively
small combinatorial background levels due to fake \D~candidates. 
This background is subtracted 
using the~\sPlot technique~\cite{Pivk:2004ty}, which is based on 
an~extended unbinned  
maximum\nobreakdash-likelihood  fit to 
these~two\nobreakdash-dimensional distributions with the function described in Ref.~\cite{LHCb-PAPER-2012-003}.
%%
\begin{comment}
with  a~four\nobreakdash-component 
function from Ref.~\cite{LHCb-PAPER-2012-003}.
\begin{eqnarray*}
  f(x, y )  & \propto &  N_{\D\D} {S}_x(x) {S}_y(y)  \\
  &   +     &  N_{\D\&\mathrm{b}} {S}_x(x) {B}_y(y)            \\
  &   +     &  N_{\mathrm{b}\&\D} {B}_x(x) {S}_y(y)            \\
  &   +     &  N_{\mathrm{b\&b}}  {B}_{2D}(x,y),
\end{eqnarray*}
where $N_{{\D\&\D}}$ is  
the~number of genuine $\D_{1}\D_{2}$ pairs,
$N_{\mathrm{\D\&b(b\&\D)}}$ is 
the~number of combinations of 
$\D_{1(2)}$~mesons with combinatorial 
background, $N_{\mathrm{b\&b}}$ is 
the~number of pure background pairs
and $x(y)$ is the combined mass of $\D$ daughters: 
$m_{\Km\pip}$ for $\Dz$ and $m_{\Km\pip\pip}$ for $\Dp$.
%%
\end{comment} 
%%
This~function consists of four components:
\begin{itemize}
    \item a component corresponding 
    to genuine $\D_1\D_2$~pairs and described 
    as a~product of two~signal functions, 
    each parameterised with 
    a~modified Novosibirsk function~\cite{Bukin};
    \item two components corresponding
    to combinations of 
    one of the \D~mesons
    %$\D_{1,2}$~mesons
    with combinatorial background  
    and described as products
    of the~signal functions and 
    background function in turn  
    parameterised with a~product 
    of an~exponential function 
    and a~positive first\nobreakdash-order 
    polynomial; 
    \item a component corresponding to pure background 
    pairs and described by a~product of exponential functions
    and a~positive two\nobreakdash-dimensional 
    non\nobreakdash-factorisable second\nobreakdash-order 
    polynomial function.
\end{itemize}
%%
Based on the~results of the~fit,  
each candidate is assigned 
a~positive weight for being signal\nobreakdash-like or
a~negative weight for being background\nobreakdash-like, 
with the~masses of the~two \Dz~candidates 
as discriminating variables. 
%% 
The~$\Dz\Dz\pip$ mass distributions for each of 
the~subtracted background components 
are presented in Extended Data Fig.~\ref{fig:SIDEBANDS}, 
where fit results 
with background\nobreakdash-only 
functions $B^{\prime}_{10}$, 
defined in Eq.~\eqref{eq:background_ext}
are overlaid. 


==> summary.tex <==
\section*{Summary}


The~exotic narrow tetraquark state \Tcc~observed in Ref.~\cite{LHCb-PAPER-2021-031}~is studied 
using a dataset
corresponding to an integrated luminosity of $9\invfb$,
collected by the~\lhcb experiment 
in $\proton\proton$~collisions
at centre-of-mass energies of 7, 8 and 13\tev.
%during the~2011--2018 period. 
%%
The~observed~$\Dz\pip$~mass distribution 
%from the~signal \mbox{$\decay{\Tcc}{\Dz\Dz\pip}$}~decays 
indicates that 
the~$\decay{\Tcc}{\Dz\Dz\pip}$~decay proceeds via an~intermediate 
off\nobreakdash-shell $\Dstarp$~meson.
Together with the~proximity of the~state 
to the~\Dstar\Dz~mass threshold 
this favours the~spin\nobreakdash-parity 
quantum numbers $\mathrm{J^P}$ to be~$1^+$. 
Narrow  near\nobreakdash-threshold structures are observed
in the~$\Dz\Dz$ and $\Dz\Dp$~mass spectra 
 with high significance.
They are found to be consistent 
with originating from off\nobreakdash-shell 
\mbox{$\decay{\Tcc}{\Dstar\D}$}~decays 
followed by the~\mbox{$\decay{\Dstar}{\D\Ppi}$} and 
\mbox{$\decay{\Dstar}{\D\g}$}~decays.
No signal is observed in the~$\Dp\Dz\pip$~mass spectrum,
and no structure is observed in the~$\Dp\Dp$~mass spectrum. 
These non-observations 
provide a~strong argument in favour 
of the~isoscalar  nature for the~observed state, 
supporting its interpretation as  
the~isoscalar $\mathrm{J^P}=1^+$ 
$\cquark\cquark
\uquarkbar\dquarkbar$\nobreakdash-tetraquark ground state.  
%%
Under this hypothesis 
%% 
the~mass of the~\Tcc~state, 
relative to the~$\Dstarp\Dz$~mass
threshold, is determined  
using a~unitarised three\nobreakdash-body Breit\nobreakdash--Wigner amplitude model 
\ifthenelse{\boolean{wordcount}}{}{
\begin{equation*}
 %% \updelta m_{\mathrm{U}} = -363 \pm 40 ^{\,+\,9}_{\,-\,6} \kevcc\,,
    \updelta m_{\mathrm{U}} = -359 \pm 40 ^{\,+\,9}_{\,-\,6} \kevcc\,,
\end{equation*}
}
where the~first uncertainty is statistic and 
the~second systematic.
The~lower limit on the~absolute value of 
the~coupling constant of the~$\Tcc$~state
to the~$\Dstar\D$~system is 
\ifthenelse{\boolean{wordcount}}{}{
\begin{equation*} 
     \left| g \right| > 
%% 5.07\,(4.26)\gev~\mathrm{at}~90\,(95)\,\%\ \mathrm{CL}\,.
   5.1\,(4.3)\gev~\mathrm{at}~90\,(95)\,\%\ \mathrm{CL}\,.
\end{equation*}
}
%% With assumption of molecular nature of 
%% the~\Tcc~state
From the~low\nobreakdash-energy limit of the~amplitude,  
the~estimates for the~scattering length $a$,
effective range $r$, and the~compositness, $Z$, are obtained 
%%
\ifthenelse{\boolean{wordcount}}{}{
%%\begingroup
%%\allowdisplaybreaks
\begin{eqnarray*}
    a & = & \Bigl[ -\left(7.16 \pm 0.51\right) 
    + i\left(1.85 \pm 0.28 \right) \Bigr] \fm\,,\\
    % a             &  = &  \Bigl( -\left( 7.16\pm 0.51 \right)  + i \left( 1.85 \pm 0.28 \right) \Bigr)\fm             \,,  \\ 
    -r            &  < & 
    11.9\,(16.9)\fm~\text{at}~90\,(95)\%\,\mathrm{CL}     \,,  \\
    Z            &  < &  
    0.52\,(0.58)~\text{at}~90\,(95)\%\,\mathrm{CL}  \,.
\end{eqnarray*}%%\endgroup
}
%%
%% \noindent
The~characteristic size calculated from 
the~binding energy is $R_{\Delta E} = 7.49 \pm 0.42\fm$.
This~value is consistent with the~estimation from 
the~scattering length, $R_a = 7.16 \pm 0.51\fm$.
%
Both $R_{\Delta E}$  and $R_{a}$ correspond to
a~spatial extension 
significantly exceeding 
the~typical scale for  heavy\nobreakdash-flavour hadrons.
%%

The~amplitude pole is found to be located 
on the~second Riemann sheet with respect to 
the~$\Dz\Dz\pip$ threshold, at
$\hat{s}=m_{\mathrm{pole}}-\tfrac{i}{2}\Gamma_{\mathrm{pole}}$, 
where 
\ifthenelse{\boolean{wordcount}}{}{
%%\begingroup
%%\allowdisplaybreaks
\begin{eqnarray*}
    \updelta m_{\mathrm{pole}} 
     & = & 
 %% -364 \pm 40  ^{\,+\,5\phantom{0}}_{\,-\,0} \kevcc \,, \\ 
    -360 \pm 40  ^{\,+\,4\phantom{0}}_{\,-\,0} \kevcc \,, \\ 
    \Gamma_{\mathrm{pole}}              & = &  
     \phantom{-0}48 \pm \phantom{0}2 ^{\,+\,0}_{\,-\,14}\kev \,,
\end{eqnarray*} 
%%\endgroup
}
where the~first uncertainty  
accounts for statistical
and systematic uncertainties for
the~$\updelta m_{\mathrm{U}}$~parameters, 
and the~second is due to 
the~unknown value of 
the~$\left|g\right|$~parameter.
%%
The pole position, scattering 
length, effective range and compositeness 
%% reveals 
form a~complete set 
of experimental observables
related to the~\mbox{$\decay{\Tcc}{\Dz\Dz\pip}$}
reaction 
amplitude,
which is vital for inferring
the~nature of the~\Tcc~tetraquark.


Unlike the~prompt production 
of the~$\chicone(3872)$~state,
no suppression of the~\Tcc~state production
at high track multiplicities
is observed
relative to 
the~low\nobreakdash-mass $\Dz\Dzb$~pairs. 
The~observed similarity 
with the~multiplicity distribution for 
the~low\nobreakdash-mass $\Dz\Dz$~production process, 
that is presumably 
double-parton-scattering dominated, 
is unexpected.
%% 
In~the~future with a~larger dataset and
including other decay modes, 
\eg\mbox{$\decay{\Dz}
{\Km\pip\pip\pim}$}, detailed studies 
of  the~properties of this~new state and its 
production mechanisms
could  be possible. 


